Seeking Stability by being Lazy and Shallow

Designing a language feature often requires a choice between several, similarly expressive possibilities. Given that user studies are generally impractical, we propose using stability as a way of making such decisions. Stability is a measure of whether the meaning of a program alters under small, seemingly innocuous changes in the code. Directly motivated by a need to pin down a feature in GHC/Haskell, we apply this notion of stability to analyse four approaches to the instantiation of polymorphic types, concluding that the most stable approach is lazy (instantiate a polytype only when absolutely necessary) and shallow (instantiate only top-level type variables, not variables that appear after explicit arguments).

==> tex/examples/Ex1.tex <==
%if style == newcode
\begin{code}
module Ex1 where
\end{code}
%endif


==> tex/figures/AltSyntax.tex <==
%if style == newcode
\begin{code}
module AltSyntax where
\end{code}
%endif

\[
\begin{array}{@@{\hspace{0mm}}c@@{\hspace{0mm}}}
  % Expressions
  \Mytabular{
    \syntaxLine{[[ee]]}
               {::=}
               { [[ h args ]] \mid [[ \ x . ee ]] }
               {Expression}
    \\
    \syntaxLine{}
               {\mid}
               { [[ let edecl in ee ]] }
               {}
    \\
    \syntaxLine{[[h]]}
               {::=}
               { [[ x ]] \mid [[ K ]] \mid [[ ee : s ]] \mid [[ ee ]] }
               {Application head}
    \\
    \syntaxLine{[[arg]]}
               {::=}
               { [[ ee ]] }
               {Application argument}
  }
\end{array}
\]


==> tex/figures/AltTyping.tex <==
%if style == newcode
\begin{code}
module AltTyping where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[H]{$[[ G |-H h => s ~> ef ]]$}{Head Type Synthesis}{Var, Con, Ann, Inf}
\drules[ETm]{$[[ G |-E ee => ne ~> ef ]]$}{Term Type Synthesis}{InfAbs, InfApp, InfLet}
\drules[ETm]{$[[ G |-E ee <= s ~> ef ]]$}{Term Type Checking}{CheckAbs, CheckLet, CheckInf}


==> tex/figures/AltTypingAF.tex <==
%if style == newcode
\begin{code}
module AltTyping where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[H]{$[[ G |-H h => s ~> ef ]]$}{Head Type Synthesis}{Var, Con, Ann, Undef, Seq, Inf}
\drules[Tm]{$[[ G |-E ee => ne ~> ef ]]$}{Term Type Synthesis}{InfAbs, InfTyAbs, InfApp, InfLet, InfTrue, InfFalse}
\drules[Tm]{$[[ G |-E ee <= s ~> ef ]]$}{Term Type Scheme Checking}{CheckAbs, CheckTyAbs, CheckLet, CheckInf}


==> tex/figures/AltTypingB.tex <==
%if style == newcode
\begin{code}
module AltTypingB where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[Arg]{$[[ G |-A args <= s => s' ~> fargs ]]$}{Argument Type Checking}{Empty, App, Inst}


==> tex/figures/AltTypingBF.tex <==
%if style == newcode
\begin{code}
module AltTypingB where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[Arg]{$[[ G |-A args <= s => s' ~> fargs ]]$}{Argument Type Checking}{Empty, App, Inst}


==> tex/figures/DeclTyping.tex <==
%if style == newcode
\begin{code}
module DeclTyping where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[Decl]{$[[ G |-E edecl => G' ~> x : s = ef ]]$}{Declaration Checking}{NoAnnSingle, NoAnnMulti, Ann}


==> tex/figures/FEval.tex <==
%if style == newcode
\begin{code}
module FEval where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[FMatch]{$[[ match ( fps1 -> ef1 ; ef2 : s2 ) |~> fps2 -> ef1' ]]$}{Core Pattern Matching}{Var, Con}
\drules[FEval]{$[[ ef1 |~> ef2 ]]$}{Core Evaluation}{App, AppAbs, Seq, SeqVal, CaseEmpty, CaseMatch, TyAbs, TyApp, TyAppAbs, Undef, TyAbsCase}
\drules[FEvalBigStep]{$[[ ef |~>* fval ]]$}{Big Step Evaluation}{Step, Done}



==> tex/figures/FSyntax.tex <==
%if style == newcode
\begin{code}
module FSyntax where
\end{code}
%endif

\[
\begin{array}{@@{\hspace{0mm}}c@@{\hspace{0mm}}}
  \Mytabular{
    \syntaxLine{[[ef]]}
               {::=}
               { [[ x ]] \mid [[ K ]] \mid [[ ef1 ef2 ]] \mid [[ \ x : s . ef ]] \mid [[ ef s ]] \mid [[ /\ a . ef ]] }
               {Expression}
    \\
    \syntaxLine{}
               {\mid}
               { [[ undefined ]] \mid [[ seq ]] }
               {}
    \\
    \syntaxLine{}
               {\mid}
               { [[ case </ fpsi : fpsigs -> efi // i /> ]] \mid [[ true ]] \mid [[ false ]] }
               {}
    \\
    \syntaxLine{[[fval]]}
               {::=}
               { [[ \ x : s . ef ]] \mid [[ /\ a . fval ]] \mid [[ K efs ]] }
               {Value}
    \\
    \syntaxLine{}
               {\mid}
               { [[ case </ fpsi : fpsigs -> efi // i /> ]] }
               {}
    \\
    \syntaxLine{[[ewf]]}
               {::=}
               { [[ [] ]] \mid [[ \ x : s . ewf ]] \mid [[ ewf s ]] \mid [[ /\ a . ewf ]] \mid [[ \ ef1 . ef2 ]] }
               {Expr. Wrapper}
    \\
    \syntaxLine{[[fctx]]}
               {::=}
               { [[ [] ]] \mid [[ \ x : s . fctx ]] \mid [[ fctx ef ]] \mid [[ ef fctx ]] }
               {Context}
    \\
    \syntaxLine{}
               {\mid}
               { [[ /\ a . fctx ]] \mid [[ fctx s ]] }
               {}
    \\
    \syntaxLine{[[farg]]}
               {::=}
               { [[ ef ]] \mid [[ s ]] }
               {Argument}
    \\
    \syntaxLine{[[fp]]}
               {::=}
               { [[ x : s ]] \mid [[ @ a ]] \mid [[ K fps ]] }
               {Pattern}
    \\
    \syntaxLine{[[fpsig]]}
               {::=}
               { [[ s ]] \mid [[ @ a ]] }
               {Arg. descriptor}
  }
\end{array}
\]


==> tex/figures/FTypingA.tex <==
%if style == newcode
\begin{code}
module FTypingA where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[InstT]{$[[ G |- s inst _ d r ~> ewf ]]$}{Type Instantiation}{SInst, SForall, SInfForall, Mono, Function, Forall, InfForall}
\drules[SkolT]{$[[ G |- s skol _ d r ; G' ~> ewf ]]$}{Type Skolemisation}{SInst, SForall, SInfForall, Mono, Function, Forall, InfForall}


==> tex/figures/FTypingB.tex <==
%if style == newcode
\begin{code}
module FTypingB where
\end{code}
%endif

\drules[PatWrap]{$[[ wrap ( ps ; ee1 ~ ee2 ) ]]$}{Pattern Wrapping}{Empty, Var, TyVar}


==> tex/figures/FTypingC.tex <==
%if style == newcode
\begin{code}
module FTypingC where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[FTm]{$[[ G |- ef : s ]]$}{System F Term Typing}{Var, Con, App, Abs, TyApp, TyAbs, Undef, True, False, Seq, Case}
\drules[FPat]{$[[ G |-P fps : fpsigs ; Del ]]$}{System F Pattern Typing}{Empty, Var, TyVar, Con}
\drules[FCtx]{$[[ fctx : G1 ; s1 |-> G2 ; s2 ]]$}{System F Context Typing}{Hole, Abs, AppR, AppL, TyAbs, TyApp, Case}


==> tex/figures/FlavourDepthTable.tex <==
%if style == newcode
\begin{code}
module FlavourDepthTable where
\end{code}
%endif

\begin{tabular}{l||c||c||c||c||}
Depth & \fpa & \fpb & \fpc & \fpd \\ \hline
$ \shallow $ & \py & \py & \py & \py \\
$ \deep $    & \py & \py & \pn & \py
\end{tabular}


==> tex/figures/FlavourEagernessTable.tex <==
%if style == newcode
\begin{code}
module FlavourEagernessTable where
\end{code}
%endif

\begin{tabular}{l||c||c||c||c||}
Eagerness & \fpa & \fpb & \fpc & \fpd \\ \hline
$ \eager $ & \py & \pn & \py & \pn \\
$ \lazy $  & \pn & \py & \py & \py
\end{tabular}


==> tex/figures/FundDefTable.tex <==
%if style == newcode
\begin{code}
module FunDefTable where
\end{code}
%endif

\begin{tabular}{l|l|}
 & Definition \\ \hline
\fpa & Time sensitive instantiation \\
\fpb & Type preserving \\
\fpc & Semantics preserving \\
\fpd & Uniformity
\end{tabular}


==> tex/figures/FundTable.tex <==
%if style == newcode
\begin{code}
module FundTable where
\end{code}
%endif

\begin{tabular}{l||p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}}
  Properties & \rot{Signature Property} & \rot{Prenex Preservation} &
  \rot{Let Inlining Property} & \rot{Let Extracting Property} & \rot{Synonym Property} &
  \rot{Pattern Property} & \rot{Implicit Parameters} & \rot{Undefined Example} \\ \hline
  \fpa &      &      &      &      &      &      & \pry & \pry \\
  \fpb & \pry & \prn & \pry & \pry & \pry &      &      &      \\
  \fpc &      &      &      &      &      &      & \pry & \pry \\
  \fpd &      &      &      &      &      & \pry &      &
\end{tabular}


==> tex/figures/InstSkol.tex <==
%if style == newcode
\begin{code}
module InstSkol where
\end{code}
%endif

%% \drules[EBndr]{$[[ ebinders _ d ( s ) = as ; r ]]$}{Binders}{ShallowInst, ShallowForall, ShallowInfForall, DeepMono, DeepFunction, DeepForall, DeepInfForall}
%% \begin{tabular*}{\textwidth}{@@{}l@@{\hspace{.1\textwidth}}r@@{}}
%% \begin{minipage}{.45\textwidth}
\drules[Inst]{$[[ G |- s inst _ d r ]]$}{Type instantiation}{Inst}
%% \end{minipage}
%% &
%% \begin{minipage}{.45\textwidth}
\drules[Skol]{$[[ G |- s skol _ d r ; G' ]]$}{Type skolemisation}{Skol}
%% \end{minipage}
%% \end{tabular*}
\drules[Type]{$[[ type ( psigs ; s ~ s' ) ]]$}{Telescope Type Construction}{Empty, Var, TyVar}


==> tex/figures/LabSyntax.tex <==
%if style == newcode
\begin{code}
module LabSyntax where
\end{code}
%endif

\[
\begin{array}{@@{\hspace{0mm}}c@@{\hspace{0mm}}}
  % Types
  \Mytabular{
    \syntaxLine{[[s]]}
               {::=}
               { \ldots \mid [[ forall ls . s ]] }
               {type scheme}
  }
  \\\\
  % Expressions
  \Mytabular{
    \syntaxLine{[[arg]]}
               {::=}
               { \ldots \mid [[ @ ( l = t ) ]] }
               {Application argument}
  }
  \\\\
  % Contexts
  \Mytabular{
    \syntaxLine{[[G]]}
               {::=}
               { \ldots \mid [[ G , l ]] }
               {Context}
  }
\end{array}
\]


==> tex/figures/ModSyntax.tex <==
%if style == newcode
\begin{code}
module ModSyntax where
\end{code}
%endif

\begin{tabular}{cc}
\begin{minipage}{.45\textwidth}
\[
  % Types
  \Mytabular{
    \syntaxLine{[[s]]}
               {::=}
               { \ldots \mid [[ forall ias . s ]] }
               {Type scheme}
    \\
    \syntaxLine{[[psig]]}
               {::=}
               { \ldots \mid [[ @ a ]] }
               {Arg. descriptor}
  }
\]
\end{minipage}
&
\begin{minipage}{.45\textwidth}
\[
  % Expressions
  \Mytabular{
    \syntaxLine{[[ee]]}
               {::=}
               { \ldots \mid [[ /\ a . ee ]] }
               {Expression}
    \\
    \syntaxLine{[[p]]}
               {::=}
               { \ldots \mid [[ @ s ]] }
               {Pattern}
    \\
    \syntaxLine{[[arg]]}
               {::=}
               { \ldots \mid [[ @ s ]] }
               {Application argument}
  }
\]
\end{minipage}
\end{tabular}


==> tex/figures/ModTypingB.tex <==
%if style == newcode
\begin{code}
module ModTypingB where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[Arg]{$[[ G |-A args <= s => s' ~> fargs ]]$}{Argument Type Checking}{TyApp, InfInst}


==> tex/figures/ModTypingBF.tex <==
%if style == newcode
\begin{code}
module ModTypingB where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[Arg]{$[[ G |-A args <= s => s' ~> fargs ]]$}{Argument Type Checking}{Empty, App, Inst, TyApp, InfInst}


==> tex/figures/ModTypingC.tex <==
%if style == newcode
\begin{code}
module ModTypingC where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[Decl]{$[[ G |-E edecl => G' ~> x : s = ef ]]$}{Declaration Checking}{NoAnnSingle, NoAnnMulti, Ann}


==> tex/figures/ModTypingCF.tex <==
%if style == newcode
\begin{code}
module ModTypingC where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[Decl]{$[[ G |-E edecl => G' ~> x : s = ef ]]$}{Declaration Checking}{NoAnnSingle, NoAnnMulti, Ann}


==> tex/figures/ModTypingD.tex <==
%if style == newcode
\begin{code}
module ModTypingD where
\end{code}
%endif

\drules[Bndr]{$[[ ebinders _ d ( s ) = as ; r ]]$}{Binders}{ShallowInst, ShallowForall, ShallowInfForall, DeepMono, DeepFunction, DeepForall, DeepInfForall}


==> tex/figures/ModTypingE.tex <==
%if style == newcode
\begin{code}
module ModTypingE where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[Pat]{$[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$}{Pattern Synthesis}{InfTyVar, InfCon}

\drules[Pat]{$[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$}{Pattern Checking}{CheckTyVar, CheckCon, CheckForall, CheckInfForall}


==> tex/figures/ModTypingEF.tex <==
%if style == newcode
\begin{code}
module ModTypingE where
\end{code}
%endif

\renewcommand\elab[1]{#1}

\drules[Pat]{$[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$}{Pattern Synthesis}{InfEmpty, InfVar, InfCon, InfTyVar}
\drules[Pat]{$[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$}{Pattern Checking}{CheckEmpty, CheckVar, CheckCon, CheckForall, CheckTyVar, CheckInfForall}


==> tex/figures/ModTypingF.tex <==
%if style == newcode
\begin{code}
module ModTypingF where
\end{code}
%endif




==> tex/figures/ModTypingG.tex <==
%if style == newcode
\begin{code}
module ModTypingE where
\end{code}
%endif

\renewcommand\elab[1]{}

\begin{tabular*}{\textwidth}{@@{}l@@{\hspace{.1\textwidth}}r@@{}}
\begin{minipage}{.45\textwidth}
\drules[Tm]{$[[ G |-E ee => ne ~> ef ]]$}{Term Type Synthesis}{InfTyAbs}
\drules[Type]{$[[ type ( psigs ; s ~ s' ) ]]$}{Telescope Construction}{TyVar}
\end{minipage}
&
\begin{minipage}{.45\textwidth}
\drules[Tm]{$[[ G |-E ee <= s ~> ef ]]$}{Term Type Checking}{CheckTyAbs, CheckAbs}
\end{minipage}
\end{tabular*}


==> tex/figures/Numargs.tex <==
%if style == newcode
\begin{code}
module Numargs where
\end{code}
%endif

\drules[Numargs]{$[[ numargs ( s ) = m ]]$}{Explicit Argument Counting}{TyVar, Con, Arrow, Forall, InfForall}


==> tex/figures/PatternTyping.tex <==
%if style == newcode
\begin{code}
module PatternTyping where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[Pat]{$[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$}{Pattern Synthesis}{InfEmpty, InfVar, InfCon, InfTyVar}
\drules[Pat]{$[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$}{Pattern Checking}{CheckEmpty, CheckVar, CheckCon, CheckForall, CheckTyVar, CheckInfForall}


==> tex/figures/PropTable.tex <==
%if style == newcode
\begin{code}
module PropTable where
\end{code}
%endif

%% \begin{tabular}{l||c||c||c||c||c||c||c||c||}
%% Preservation of & \multicolumn{4}{c||}{Types} & \multicolumn{4}{c||}{D} \\
%%  & \multicolumn{2}{c||}{$ \eager $} & \multicolumn{2}{c||}{$ \lazy $} & \multicolumn{2}{c||}{$ \eager $} & \multicolumn{2}{c||}{$ \lazy $} \\
%% Transformations & $ \shallow $ & $ \deep $ & $ \shallow $ & $ \deep $ & $ \shallow $ & $ \deep $ & $ \shallow $ & $ \deep $ \\ \hline
%% 1. Let inlining      & \pn & \pn & \py & \py & \py & \py & \py & \py \\
%% 2. Type signatures   & \pn & \pn & \py & \py & \py & \py & \py & \py \\
%% 3. Undefined         & \py & \py & \py & \py & \py & \pn & \pn & \pn \\
%% 4. Pattern inlining  & \pn & \pn & \py & \py & \py & \py & \py & \py \\
%% 5. Implicit inlining & \py & \py & \py & \py & \py & \pn & \pn & \pn
%% \end{tabular}

\begin{tabular}{l||lll||l||c||c||c||c||}
\multicolumn{2}{c}{} & & & & \multicolumn{2}{c||}{$ \eager $} & \multicolumn{2}{c||}{$ \lazy $} \\

Sim. & \multicolumn{3}{l||}{Property\hspace{\stretch{1}}Phase} & App. & $ \shallow $ & $ \deep $ & $ \shallow $ & $ \deep $ \\ \hline

1 & \ref{prop:let_inlining}       & Let inl.         & \comptime & \ref{app:prop1}  & \py & \py & \py & \py \\
  & \ref{prop:let_extraction}     & Let extr.        & \comptime & \ref{app:prop1}  & \pn & \pn & \py & \py \\
  & \ref{prop:let_inlining_dyn}   &                  & \runtime  & \ref{app:prop2}  & \py & \pn & \py & \pn \\
2 & \ref{prop:signature_type}     & Signature prop   & \comptime &                  & \pn & \pn & \pn & \pn \\
  & \ref{prop:signature_type_single} & \restr        &           & \ref{app:prop5}  & \pn & \pn & \py & \py \\
  & \ref{prop:signature_dyn}      &                  & \runtime  & \ref{app:prop5}  & \py & \pn & \py & \pn \\
3 & \ref{prop:type_sig}           & Type sign.       & \runtime  & \ref{app:prop5}  & \py & \pn & \py & \pn \\
4 & \ref{prop:pat_inlining_typ}   & Pattern inl.     & \comptime & \ref{app:prop8}  & \pn & \pn & \py & \py \\
  & \ref{prop:pat_inlining_dyn}   &                  & \runtime  & \ref{app:prop8}  & \py & \pn & \py & \py \\
  & \ref{prop:pat_extraction_typ} & Pattern extr.    & \comptime & \ref{app:prop8}  & \pn & \pn & \py & \py \\
5 & \ref{prop:single_multi}       & Single/multi     & \comptime & \ref{app:prop11} & \py & \py & \pn & \pn \\
6 & \ref{prop:eta}                & $\eta$-expansion & \comptime &                  & \pn & \pn & \pn & \pn \\
  & \ref{prop:eta_restr}          & \restr           &           & \ref{app:prop12} & \pn & \py & \pn & \pn \\
\end{tabular}


==> tex/figures/RelationTable.tex <==
%if style == newcode
\begin{code}
module RelationTable where
\end{code}
%endif

\begin{tabular}{@@{}l@@{\;\;}l@@{\;\;}l@@{}}
Fig. \ref{fig:TermTyping} & $[[ G |-E ee => ne ~> ef ]]$ & Synthesise type $[[ne]]$ for $[[ee]]$ \\
Fig. \ref{fig:TermTyping} & $[[ G |-E ee <= s ~> ef ]]$ & Check $[[ee]]$ against type $[[s]]$ \\
Fig. \ref{fig:TermTyping} & $[[ G |-H h => s ~> ef ]]$ & Synthesise type $[[s]]$ for head $[[h]]$ \\
Fig. \ref{fig:TermTyping} & $[[ G |-A args <= s => s' ~> fargs ]]$ & Check $[[args]]$ against $[[s]]$, \\
& & resulting in type $[[s']]$ \\
Fig. \ref{fig:DeclTyping} & $[[ G |-E edecl => G' ~> x : s = ef ]]$ & Extend context with a decl. \\
Fig. \ref{fig:PatternTyping} & $[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$ & Synthesise types $[[psigs]]$ for  \\
& & patterns $[[ps]]$, binding context $[[Del]]$ \\
Fig. \ref{fig:PatternTyping} & $[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$ & Check $[[ps]]$ against $[[s]]$, with  \\
& & residual type $[[s']]$, binding $[[Del]]$ \\
Fig. \ref{fig:InstSkol} & $[[ G |- s inst _ d r ~> ewf ]]$ & Instantiate $[[s]]$ to $[[r]]$ \\
Fig. \ref{fig:InstSkol} & $[[ G |- s skol _ d r ; G' ~> ewf ]]$ & Skolemise $[[s]]$ to $[[r]]$, binding $[[G']]$ \\
App. \ref{app:addrel} & $[[ ebinders _ d ( s ) = as ; r ]]$ & Extract type var.~binders $[[as]]$
\\
& & and residual $[[r]]$ from $[[s]]$ \\
App. \ref{app:addrel} & $[[ wrap ( ps ; ee1 ~ ee2 ) ]]$ & Bind patterns $[[ps]]$ in $[[ee1]]$ to get $[[ee2]]$
\end{tabular}



==> tex/figures/Syntax.tex <==
%if style == newcode
\begin{code}
module Syntax where
\end{code}
%endif

\begin{minipage}{0.5 \textwidth}
  \[
  \Mytabular{ 
    % Types
    \syntaxLine{[[d]]}
               {::=}
               { [[ S ]] \mid [[ D ]] }
               {Depth}%
    \\
    \syntaxLine{[[ep]]}
               {::=}
               { [[ E ]] \mid [[ L ]] }
               {Eagerness}%
    \\[1ex]
    \syntaxLine{[[t]]}
               {::=}
               { [[ a ]] \mid [[ t1 -> t2 ]] \mid [[ T ts ]] }
               {Monotype}%
    \\
    \syntaxLine{[[r]]}
               {::=}
               { [[ t ]] \mid [[ s -> qd ]] }
               {Instantiated type}%
    \\
    \syntaxLine{[[s]]}
               {::=}
               { [[ r ]] \mid [[ forall as . s ]] \mid [[ forall ias . s ]] \mid [[ s1 -> s2 ]] }
               {Type scheme}%
    \\
    \syntaxLine{[[qd]]}
               {::=}
               { [[ r ]] \quad ( [[ d = D ]] ) }
               {Instantiated result}%
    \\
    \syntaxLine{}
               {\mid}
               { [[ s ]] \quad ( [[ d = S ]] ) }
               {}
    \\
    \syntaxLine{[[ne]]}
               {::=}
               { [[ r ]] \quad ( [[ ep = E ]] ) }
               {Synthesised type}%
    \\
    \syntaxLine{}
               {\mid}
               { [[ s ]] \quad ( [[ ep = L ]] ) }
               {}
  }
  \]
\end{minipage}%
\begin{minipage}{0.5 \textwidth}
  \[
  \Mytabular{ 
    % Expressions
    \syntaxLine{[[ee]]}
               {::=}
               { [[ h args ]] \mid [[ \ x . ee ]] \mid [[ /\ a . ee ]] \mid [[ let edecl in ee ]] }
               {Expression}%
    \\
    \syntaxLine{[[h]]}
               {::=}
               { [[ x ]] \mid [[ K ]] \mid [[ ee : s ]] \mid [[ ee ]] }
               {Application head}%
    \\
    \syntaxLine{[[arg]]}
               {::=}
               { [[ ee ]] \mid [[ @ s ]] }
               {Application argument}%
    \\
    \syntaxLine{[[edecl]]}
               {::=}
               { [[ x : s ; </ x psi = eei // i /> ]] \mid [[ </ x psi = eei // i /> ]] }
               {Declaration}%
    \\
    \syntaxLine{[[p]]}
               {::=}
               { [[ x ]] \mid [[ K ps ]] \mid [[ @ s ]] }
               {Pattern}%
  \\[1ex]
  % Context
    \syntaxLine{[[Sig]]}
               {::=}
               { [[ empty ]] \mid [[ Sig , T as ]] \mid [[ Sig , K : as ; ss ; T ]] }
               {Static context}%
    \\
    \syntaxLine{[[G]] , [[Del]]}
               {::=}
               { [[ Sig ]] \mid [[ G , x : s ]] \mid [[ G , a ]] }
               {Context}%
    \\
    \syntaxLine{[[psig]]}
               {::=}
               { [[ t ]] \mid [[ @ a ]] }
               {Arg. descriptor}%
  }%
  \]%
\end{minipage}


==> tex/figures/TermTyping.tex <==
%if style == newcode
\begin{code}
module TermTyping where
\end{code}
%endif

\renewcommand\elab[1]{}

\drules[H]{$[[ G |-H h => s ~> ef ]]$}{Head Type Synthesis}{Var, Con, Ann, Inf}
\drules[Tm]{$[[ G |-E ee => ne ~> ef ]]$}{Term Type Synthesis}{InfAbs, InfApp, InfLet, InfTyAbs}
\drules[Tm]{$[[ G |-E ee <= s ~> ef ]]$}{Term Type Checking}{CheckAbs, CheckLet, CheckInf, CheckTyAbs}
\drules[Arg]{$[[ G |-A args <= s => s' ~> fargs ]]$}{Argument Type Checking}{Empty, App, Inst, TyApp, InfInst}


==> tex/sections/AdditionalRel.tex <==
%if style == newcode
\begin{code}
module AdditionalRel where
\end{code}
%endif

\section{Type System Details}
\label{app:addrel}

  \input{tex/figures/ModTypingD.mng}

  \input{tex/figures/FTypingB.mng}

In addition to including the figures above, this
appendix describes our treatment of $[[let]]$-declarations
and patterns:

\paragraph{Let Binders}
A $[[let]]$-expression $[[ let edecl in ee ]]$
(\rref{ETm-InfLet} and \rref{ETm-CheckLet}) defines a single
variable, with or without a type signature.
The declaration typing judgement (Figure~\ref{fig:DeclTyping}) produces
a new context $[[G']]$, extended with the binding from this declaration.

\Rref{Decl-NoAnnSingle,Decl-NoAnnMulti} 
distinguish between a single equation without a type signature
and multiple equations. In the former case, we synthesise the types
of the patterns using the $[[|-P]]$ judgement and then the type of
the right-hand side. We assemble the complete type with $[[type]]$,
and then generalise. The multiple-equation case is broadly similar,
synthesising types for the patterns (note that each equation must
yield the \emph{same} types $[[psigs]]$) and then synthesising types
for the right-hand side. These types are then instantiated (only
necessary under \instL{lazy} instantiation---eager instantiation would
have already done this step).
This additional instantiation step is the only difference between
the single-equation case and the multiple-equation case.
The reason is that \rref{Decl-NoAnnMulti} needs to construct a single type
that subsumes the types of every branch.
Following GHC, we simplify this process by first instantiating the types.
% Indeed, this difference is the only
% reason we have separated out the single-equation case, to be able
% to define synonyms of variables with higher-rank or non-prenex types.

\Rref{Decl-Ann} checks a declaration with a type signature. It
works by first checking the patterns $[[psi]]$ on the left
of the equals sign against the provided type $[[s]]$. The right-hand sides $[[eei]]$
are then checked against the remaining type $[[si']]$.
%% The pattern type checking relation $[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$ (see
%% Figure~\ref{fig:STmd}) checks the list of patters $[[ps]]$ under type scheme
%% $[[s]]$, and produces the remaining type $[[s']]$ and the typing context
%% extension $[[Del]]$.

\paragraph{Patterns}
The pattern synthesis relation $[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$
and checking relation $[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$ are presented in
Figure~\ref{fig:PatternTyping}. As the full type is not yet available,
synthesis produces argument descriptors $[[psigs]]$ and a typing context
extension $[[Del]]$.
When checking patterns, the type to check against $[[s]]$ is available, and the
relation produces a residual type $[[s']]$, along with the typing context
extension $[[Del]]$.

Typing a variable pattern works similarly to expressions.
Under inference (\rref{Pat-InfVar}) we construct a monotype and place it in
the context. When checking a variable (\rref{Pat-CheckVar}), its type $[[s1]]$
is extracted from the known function type and placed in the context.
Type abstraction $[[ @ a ]]$ in both synthesis and checking mode
(\rref{Pat-InfTyVar} and \rref{Pat-CheckTyVar} respectively) produces a
type argument descriptor $[[ @ a ]]$ and extends the typing environment.

Typing data constructor patterns (\rref{Pat-InfCon} and \rref{Pat-CheckCon}),
works by looking up the type $[[forall as0 . ss0 -> T as0]]$ of
the constructor $[[K]]$ in the typing context, and checking the applied
patterns $[[ps]]$ against the instantiated type, and an extended context\footnote{Extending
the context for later patterns
is not used in this system, but it would be required for extensions like view
patterns.}.
The remaining type should be the
result type for the constructor, meaning that the constructor always needs to be
fully applied.
Note that full type schemes $[[ss1]]$ are allowed in patterns, where they
are used to instantiate the variables \([[as0]]\)
(possibly extended with guessed monotypes \([[ts0]]\), if there are not enough $[[ss1]]$).
Consider, for example, $[[ f (Just @ Int {,} x ) = x + 1 ]]$,
where the $[[ @ Int ]]$ refines the type of $[[Just]]$, which in turn assigns
$[[ x ]]$ the type $[[ Int ]]$. Note that pattern checking allows skolemising
bound type variables (\rref{Pat-CheckInfForall}), but only when the patterns
are not empty in order not to lose syntax-directedness of the rules.
The same holds for \rref{Pat-CheckForall}, which only applies when no
other rules match.


==> tex/sections/Background.tex <==
%if style == newcode
\begin{code}
module Background where

import Type.Reflection ( Typeable, TypeRep )

\end{code}
%endif

\section{Background}
\label{sec:background}

This section describes instantiation in GHC today and sets our
baseline understanding for the remainder of the paper.

%% The concept of stability is important in languages that have a mix of implicit
%% and explicit features---a very common combination, appearing in Coq, Agda, Idris,
%% modern Haskell, C++, Java, C\#, Scala, F\#, and Rust, among others.
%%  This section walks through how a mixing of implicit
%% and explicit features in Haskell\footnote{Our work
%% is tested with GHC~8.10.1, and we use ``Haskell'' to refer to the language accepted by GHC.},
%% Idris\footnote{\raggedright We work with Idris 2, as available from \url{https://github.com/idris-lang/Idris2},
%% at commit \textsf{a7d5a9a7fdfbc3e7ee8995a07b90e6a454209cd8}.}, and Agda\footnote{We work with Agda~2.6.0.1.} 
%% causes instability. We use these languages to show how the issues we 
%% describe are likely going to arise in any language mixing implicit and explicit
%% features---and how stability is a worthwhile metric in examining these features---not
%% to critique these languages in particular. This section considers the instantiation
%% features in these languages; see Appendix~\ref{sec:idris-agda-haskell} for discussion
%% of other sources of instability in these languages.

%% Many of the key terms in this line of work have subtly different meanings
%% throughout the existing literature. We pin down terminology here.

%% \paragraph{Polymorphism} A function exhibits polymorphism when it can be
%% used at multiple different concrete types. We consider two forms of
%% polymorphism: \emph{Parametric polymorphism} describes a function that
%% treats all types identically---the choice of type is irrelevant at runtime.
%% The |const| function from the introduction is parametrically polymorphic.
%% \emph{Ad-hoc polymorphism} describes a function with different
%% behavior for different types. A function like |+| that works over different
%% numeric types would have ad-hoc polymorphism. Many functional languages
%% use type classes~\cite{wadler-blott} to implement ad-hoc polymorphism; other
%% languages use operator overloading or object-oriented class-based polymorphism
%% to accomplish similar goals.

%% \paragraph{Generalization} Some languages---notably, those derived from the
%% Hindley-Milner type system---perform generalization. If a programmer writes
%% a function that could work over multiple types, the type system assigns a
%% polymorphic (general) type to that function, instead of a specific type
%% that works over only one argument type. For example, if we define |id x = x|
%% in Haskell, we get the type |id :: forall a. a -> a|, not the type |id :: Int -> Int|.

%% \paragraph{Type signatures} Languages may require that all defined variables
%% have a type signature, declaring in advance the type of that variable. These
%% include both C-like languages (though recent innovations such as $\keyword{auto}$
%% in C++ and $\keyword{var}$ in Java blur this distinction) and many dependently
%% typed languages, such as Agda or Idris. Languages derived from Hindley-Milner,
%% including Haskell and ML, generally support but do not require type signatures,
%% instead using type inference to assign types to variables. Some languages support
%% \emph{partial type signatures}~\cite{partial-type-signatures}, where there is a
%% mix of known and unknown information. For example, Haskell allows us to declare
%% %
%% \begin{code}
%% not :: _ -> Bool
%% not  True   =  False
%% not  False  =  True
%% \end{code}
%% %
%% and the type for |not| is inferred to be |Bool -> Bool|. This uses a recent---and
%% somewhat exotic---feature in GHC. However, partial
%% type signatures exist beyond this one Haskell extension. For example, Idris allows
%% %
%% \begin{spec}
%% len : (a : _) -> List a -> Int
%% len _  []         =  0
%% len a  (_ :: xs)  =  1 + len a xs
%% \end{spec}
%% %
%% Here, the interpreter can figure out that the type of |a| is really |Type|, but
%% that is not specified by the user. Clever uses of this feature can lead Idris
%% to perform generalization, even though the language requires type signatures. See \pref{sec:idris-generalization}
%% for an example. \rae{Check with Idris 2.}

%% \paragraph{Bidirectional type checking}
%% In order to support advanced type system features, many languages support
%% \emph{bidirectional type checking}~\cite{?}, where the type checker uses type annotations
%% to direct how to interpret the annotated expressions. \rae{More here}

%% \rae{I've stopped updating this section, thinking that this is better to revisit when 
%% we have a better idea of what will be needed by the final paper.}

%% \subsection{Type Signatures}

%% Writing type signatures is always a good idea as they serve as both a sanity
%% check and as machine-checked documentation.
%% However, as the compiler can often infer the type automatically, most languages
%% do not require programmers to explicitly write type signatures.
%% Indeed, the compiler can use a bidirectional type system, which
%% can both check user-written type annotations and infer missing types.

%% In order to achieve this, the type system has to be able to instantiate
%% polymorphic types, as well as generalise types. The former means that the
%% compiler can fill in either a concrete type, or a unification variable (to be
%% instantiated later on) for a type variable. The latter means that unsolved
%% unification variables can be abstracted over in a \texttt{forall} binder.
%% Section~\ref{sec:inst} discusses different options regarding where and how this
%% instantiation may happen.
%% Note both this abstraction and instantiation happens implicitly.

% \subsection{Explicit Instantiation}

%% All three of our example languages
%% feature explicit instantiation of implicit arguments, allowing the programmer to manually
%% instantiate a polymorphic type, for example.
%% Explicit instantiation broadly comes in two flavours: ordered or
%% named parameters.

\subsection{Instantiation in GHC}

Visible type application and variable specificity are fixed attributes of the
designs we are considering.

\paragraph{Visible type application}
Since GHC~8.0, Haskell has supported visible instantiation of type variables,
based on the order in which those variables occur~\cite{visible-type-application}.
Given |const :: forall a b. a -> b -> a|, we can write |const @Int @Bool|, which instantiates
the type variables, giving us an expression of type |Int -> Bool -> Int|. If a user wants
to visibly instantiate a later type parameter (say, |b|) without choosing an earlier one,
they can write |at _| to skip a parameter. The expression |const (at _) @Bool| has type
|alpha -> Bool -> alpha|, for any type |alpha|. %% Ordered parameters have two
%% advantages: they are concise and do not leak the choice of variable names from
%% the library to its client.

%% %format <= = "\Leftarrow"
%% % \gertjan{Reviewer 3 finds <= hard to parse, and would prefer to just write `leftarrow`}
%% Haskell's treatment of instantiation is unstable even without reference to other features
%% described below, because Haskell type signatures do not need to explicitly quantify their
%% variables. For example, we can declare |const| with |const :: a -> b -> a|, with no
%% |forall a b|, and we can still write |const @Int @Bool| to instantiate the function.
%% The policy is to quantify the variables according to their left-to-right occurrence
%% in the type (ignoring duplicate occurrences). This means, though, that if we define
%% |type b <= a = a -> b| (the lexeme |<-| is reserved) and then write |const :: (b -> a) <= a|,
%% we now require all clients of |const| to also reverse the order of their type instantiations.
%% As a conscientious library author, we could choose to explicitly include |forall a b| to
%% keep the old variable ordering, but it would be easy to think that the use of a type synonym
%% in a type signature is a purely internal matter and that no special care need be taken.

%% \subsection{Idris}
%% Idris, on the other hand, supports named parameters.
%% If we define |const : {a, b : Type} -> a -> b -> a| (this syntax is the Idris
%% equivalent of the Haskell type |forall a b. a -> b -> a|), then we can write |const {b = Bool}|
%% to instantiate only the second type parameter or |const {a = Int} {b = Bool}| to instantiate
%% both. Order does not matter; |const {b = Bool} {a = Int}| works as well as the previous example.
%% Named parameters may be easier to read than ordered parameters and are robust to the addition
%% of new type variables.

%% Idris's approach suffers from an instability inherent with named parameters.
%% Unlike Haskell, the order of quantified variables does
%% not matter. Yet now, the choice of \emph{names} of the parameters naturally \emph{does} matter.
%% Thus |const : c -> d -> c| (taking advantage of the possibility of omitting explicit quantification
%% in Idris) has a different interface than |const : a -> b -> a|, despite
%% the fact that the type variables scope over only the type signature they appear in.

%% \subsection{Agda}
%% Agda accepts both ordered and named parameters.
%% After defining |const : {a b : Set} -> a -> b -> a|, we can write expressions like
%% |const {Int}| (instantiating only |a|), |const {b = Bool}|, or |const {_} {Bool}|.
%% Despite using named parameters, order \emph{does} matter: we cannot instantiate
%% earlier parameters after later ones. Naming is useful for skipping parameters that
%% the user does not wish to instantiate. Because Agda requires explicit quantification
%% of variables used in types (except as allowed for in implicit generalisation, below),
%% the ordering of variables must be fixed by the programmer. However, like Idris,
%% Agda suffers from the fact that the choice of name of these local variables leaks to clients.

%% \subsection{Conclusion}

%% We see here how Haskell, Idris, and Agda all have a mix of explicit and implicit
%% features around type instantiation. This mix raises the potential
%% for language instability: they make it possible for small, apparently insignificant
%% changes to code to affect the semantics of programs. All three languages examined here
%% have taken steps to mitigate this instability, but none have eliminated it entirely.

\paragraph{Specificity}
\label{sec:specificity}

\citet[Section~3.1]{visible-type-application} introduce the notion of type variable
\emph{specificity}. The key idea is that quantified type variables are either
written by the user (these are called \emph{specified}) or invented by the
compiler (these are called \emph{inferred}). A specified variable is available
for explicit instantiation using, e.g., |@Int|; an inferred variable may not
be explicitly instantiated.

Following GHC, we use braces to denote inferred variables. Thus, if we have
the Haskell program
%if style == poly
%format id1
%format id2
%endif
\begin{code}
id1 :: a -> a
id1 x = x

id2 x = x
\end{code}
%
then we would write that |id1 :: forall a. a -> a| (with a specified |a|)
and |id2 :: forall {a}. a -> a| (with an inferred |a|). Accordingly, |id1 @Int|
is a function of type |Int -> Int|, while |id2 @Int| is a type error.

\subsection{Deep vs.~Shallow Instantiation}
The first aspect of instantiation we seek to vary is its \emph{depth},
which type variables get instantiated. Concretely, shallow
instantiation affects only the type variables bound before any explicit
arguments. Deep instantiation, on the other hand, also instantiates all
variables bound after any number of explicit arguments. For example,
consider a function |f :: forall a. a -> (forall b. b -> b) -> forall c. c -> c|.
A shallow instantiation of |f|'s type instantiates only |a|, whereas deep instantiation 
also affects |c|, despite |c|'s deep binding site. Neither instantiation flavour touches
|b| however, as |b| is not an argument of |f|.

Versions of GHC up to 8.10 perform deep instantiation, as originally introduced by
\citet{practical-type-inference}, but GHC~9.0 changes this design, as proposed
by \citet{proposal-287} and inspired by \citet{quick-look}.
In this paper, we study this change through the lens of stability.

\subsection{Eager vs.~Lazy Instantiation}
Our work also studies the \emph{eagerness} of instantiation,
which determines the location in the code where
instantiation happens. Eager instantiation immediately instantiates a polymorphic
type variable as soon as it is mentioned. In contrast, lazy instantiation holds
off instantiation as long as possible until instantiation is necessary in order
to, say, allow a variable to be applied to an argument.

For example, consider these functions:
%
\begin{code}
pair :: forall a. a -> forall b. b -> (a, b)
pair x y = (x,y)

myPairX x = pair x
\end{code}
%
What type do we expect to infer for |myPairX|? With eager instantiation,
the type of a polymorphic expression is instantiated as soon as it occurs.
Thus, |pair x| will have a type |beta -> (alpha, beta)|, assuming we have
guessed |x :: alpha|. (We use Greek letters to denote unification variables.)
With neither |alpha| nor |beta| constrained, we will
generalise both, and infer |forall {a} {b}. a -> b -> (a, b)| for |myPairX|.
Crucially, this type is \emph{different} than the type of |pair|.

Let us now replay this process with lazy instantiation. The
variable |pair| has type |forall a. a -> forall b. b -> (a, b)|. In order
to apply |pair| of that type to |x|, we must instantiate the first quantified
type variable |a| to a fresh unification variable |alpha|, yielding
the type |alpha -> forall b. b -> (alpha, b)|. This is indeed a function type,
so we can consume the argument |x|, yielding |pair x :: forall b. b -> (alpha, b)|.
We have now type-checked the expression |pair x|, and thus
we take the parameter |x| into account and generalise this
type to produce
the inferred type |myPairX :: forall {a}. a -> forall b. b -> (a, b)|.
This is the same as the type given for |pair|, modulo the specificity of |a|.

As we have seen, thus, the choice of eager or lazy instantiation can change
the inferred types of definitions. In a language that allows visible instantiation
of type variables, the difference between these types is user-visible. With
lazy instantiation, |myPairX True @Char 'x'| is accepted, whereas with eager
instantiation, it would be rejected.


%% \rae{What follows seems a bit like a distraction. Remove?}

%% Haskell's concept of provenance was invented solely to improve the stability
%% of the language, although we are the first to describe it that way. As tends
%% to happen in Haskell, the feature has attracted new uses, also to mitigate
%% existing problems around stability; GHC now allows users to explicitly
%% choose the provenance of a variable~\cite{proposal-99}.
%% The classic illustrative example is this:
%% %
%% %if style == poly
%% %format undefinedDots = "\ldots"
%% %else
%% %format undefinedDots = "undefined"
%% %endif
%% \begin{code}
%% typeRep :: Typeable a => TypeRep a
%% typeRep = undefinedDots
%% \end{code}
%% %
%% The |typeRep| function allows users to produce a runtime type
%% representation of a type |a|; the |Typeable a| constraint asserts
%% that this information is indeed available at runtime. \citet{typerep}
%% describe the details. 

%% Type representations are available for types of arbitrary kind. Accordingly,
%% |typeRep| is kind-polymorphic, as are |Typeable| and |TypeRep|:
%% its full type is |forall k (a :: k). Typeable @k a => TypeRep @k a|. However,
%% making the kind polymorphism in |typeRep|'s type signature explicit would hurt
%% clients, because it would change the provenance of |k|. In the signature for
%% |typeRep| above, |k| is not mentioned; it is thus an inferred type variable.
%% A client wanting the representation for |Int| can get it with |typeRep @Int|.
%% However, writing, for example, |typeRep :: Typeable a => TypeRep (a :: k)| both
%% makes the kind polymorphism explicit (helpful for readers of documentation) and
%% changes |k|'s provenance to be specified. With this changed signature, clients
%% would need to instantiate |k| before instantiating |a|, writing |typeRep @Type @Int|
%% or |typeRep (at _) @Int| to get the representation for |Int|. This degrades the
%% user interface of |typeRep| considerably.

%% The solution comes from \citet{proposal-99}: allow users to explicitly mark
%% variables as inferred (somewhat paradoxically). This proposal is implemented in GHC~9.0,
%% and now we can write |typeRep :: forall {k} (a :: k). Typeable @k a => TypeRep @k a|,
%% both making the kind polymorphism explicit and keeping a tidy user interface.

%% The lesson here is that Haskell's design around provenance is unstable: by making
%% the kind polymorphism in a type signature explicit (a seemingly innocuous, local
%% change), that function's interface is also altered. We thus must add a new feature
%% to Haskell---explicit provenance marking---in order to mitigate this instability.


==> tex/sections/CaseStudy.tex <==
%if style == newcode
\begin{code}
module CaseStudy where
\end{code}
%endif

\section{Instantiation in GHC}
\label{sec:ghc}

Given the connection between this work and GHC, we now turn to examine
some practicalities of how lazy instantiation might impact the implementation.

\subsection{Eagerness}

%% A tendency toward eager instantiation starts in
%% the original type inference algorithm of \citet{damas-milner}, where
%% polymorphic variables are instantiated at their occurrences. We functional
%% programmers are thus somewhat conditioned to prefer eager instantiation.

%% However, \citet{visible-type-application} (who introduce explicit type
%% instantiation in the context of Haskell) observe that this preference
%% for eager instantiation is incidental. An equally powerful type inference algorithm
%% can be constructed for the Hindley-Milner type system using lazy instantiation---that
%% is, instantiating at function applications, not variable occurrences. And,
%% we see that lazy instantiation leads to a more compositional language, allowing
%% constructions like |(let x = 5 in id) @Bool True|. Eager instantiation would
%% have to reject such a phrase, because the polymorphism in |id| would not survive
%% its wrapping in the |let|.

%Echoing this broader history, 
GHC used eager instantiation from the beginning, echoing \citet{damas-milner}.
However, the GHC~8 series, which contains support for explicit type application,
implements an uneasy truce, sometimes using lazy instantiation (as
advocated by \citet{visible-type-application}), and
sometimes eager. In contrast, GHC~9.0 uses eager instantiation everywhere.
This change was made for practical reasons: eager instantiation simplifies the
code somewhat. If we went back to using lazy instantiation, the recent experience
in going from lazy to eager suggests we will have to combat these challenges:

\paragraph{Displaying inferred types}
The types inferred for functions are more exotic with lazy instantiation.
For example, defining |f = \ _ -> id| would infer |f :: forall {a}. a -> forall b. b -> b|.
These types, which could be reported by tools (including GHCi), might be confusing for users.

\paragraph{Monomorphism restriction}
 Eager instantiation makes the monomorphism restriction easier to implement,
because %we can be more sure when a definition is constrained, as the 
relevant
constraints are instantiated.

The monomorphism restriction is a peculiarity of Haskell, introduced to avoid
unexpected runtime evaluation\footnote{The full description is in the Haskell Report,
Section 4.5.5~\cite{haskell2010}.}. It potentially applies whenever a variable is defined without
a type annotation and without any arguments to the left of the |=|: such a
definition is not allowed to infer a type constraint. %% . As an example,
%% the monomorphism restriction would apply to |let plus = (+) in ...| and
%% |let x = 5 in ...| (recalling that |5 :: Num a => a| in Haskell).
%% In these variable declarations, Haskell requires that the inferred type not be constrained.
%% The reason is that such a declaration looks like it is declaring a variable, not
%% a function. Accordingly, programmers might expect the variable to be evaluated
%% once, and then accessible with no runtime cost many times. However, a constrained
%% variable compiles to a function, taking the type-class dictionary~\cite{type-classes-impl}
%% containing the runtime implementations of class methods. Thus, if we inferred
%% |x :: Num a => a|, then every occurrence of |x| would have to be evaluated separately,
%% causing runtime slowdown. The monomorphism restriction avoids this surprise by
%% requiring an unconstrained type; in practice, the type will be defaulted.
%% The examples in this paragraph are inferred to have types |plus :: Integer -> Integer -> Integer| and |x :: Integer|, unless usage sites of the functions suggest a different
%% numeric type.

Eager instantiation is helpful in implementing the monomorphism restriction, as
the implementation of |let|-generalisation can look for unsolved constraints
and default the type if necessary. With lazy instantiation, on the other hand,
we would have to infer the type and then make a check to see whether it is
constrained, instantiating it if necessary. Of course, the monomorphism restriction
itself introduces instability in the language (note that |plus| and |(+)| have different
types), and so perhaps revisiting this design choice is worthwhile.

\paragraph{Type application with un-annotated variables}
%There is a desire for a simple policy around the availability of explicit
%type instantiation. Specifically, 
For simplicity, we want all variables without type signatures
not to work with explicit type instantiation. (\citet[Section 3.1]{visible-type-application}
expands on this point.) Eager instantiation accomplishes this,
because variables without type signatures would get their polymorphism via re-generalisation.
On the other hand, lazy instantiation would mean that some user-written variables
might remain in a variable's type, like in the type of |f|, just above.

Yet even with eager instantiation, if instantiation is shallow, we can \emph{still}
get the possibility of visible type application on un-annotated variables: the
specified variables might simply be hiding under a visible argument.
Consider |myPair| from Example~2: under eager shallow instantiation, it gets
assigned the type | forall {a}. a -> forall b. b -> (a,b) |.
This allows for visible type application despite the lack of a signature:
| myPair True @Char |.

\subsection{Depth}

From the introduction of support for higher-rank types in GHC~6.8, GHC has
done deep instantiation, as outlined by \citet{practical-type-inference}, the
paper describing the higher-rank types feature. However, deep instantiation
has never respected the runtime semantics of a program; \citet{proposal-287}
has the details. In addition, deep instantiation is required in order to
support covariance of result types in the type subsumption judgement
(\cite[Figure~7]{practical-type-inference}). This subsumption judgement, though,
weakens the ability to do impredicative type inference, as described by
\citet{guarded-impredicativity} and \citet{quick-look}. GHC has thus,
for GHC~9.0, changed to use shallow subsumption and shallow instantiation.

\subsection{The situation today: Quick Look impredicativity has arrived}

%% The analysis around stability in this paper strongly suggests that GHC should
%% use the lazy, shallow approach to instantiation. Yet the struggles with lazy
%% instantiation above remain. In order to simplify the implementation, % which has
%% %supported lazy instantiation with an extra eager instantiation before generalisation,
%% GHC has recently (for GHC~9.0) switched to use exclusively
%% eager instantiation. This choice sacrifices stability for convenience in implementation.

%% Still, one problem remains: what to do when a user asks for the type of an expression?
%% For example, when the user asks for the type of |const @Int| in GHCi, GHC's interactive
%% environment, we should see
%% |forall b. Int -> b -> Int|. Note that this type is \emph{not} instantiated eagerly.
%% There is thus a separate mechanism for getting the type of an expression in GHCi,
%% avoiding eager instantiation---the one inconvenience of using eager instantiation.

A recent innovation within GHC (due for release in the next version, GHC~9.2)
is the implementation of the Quick Look
algorithm for impredicative type inference~\cite{quick-look}. The design of that
algorithm walks a delicate balance between expressiveness and stability. It introduces
new instabilities: for example, if |f x y| requires impredicative instantiation,
|(let unused = 5 in f) x y| will fail. Given that users who opt into impredicative
type inference are choosing to lose stability properties, we deemed it more important
to study type inference without impredicativity in analysing stability. While our
formulation of the inference algorithm is easily integrated with the Quick Look
algorithm, we leave an analysis of the stability of the combination as future work.


==> tex/sections/Conclusion.tex <==
%if style == newcode
\begin{code}
module Conclusion where
\end{code}
%endif

\section{Conclusion}

This work introduces the concept of \emph{stability} as a proxy for the
usability of a language that supports both implicit and explicit arguments\footnote{Recent
work by \citet{cochis} also uses the term \emph{stability} to analyse a language
feature around implicit arguments. That work discusses the stability of type
class instance selection in the presence of substitutions, a different concern
than we have here.}.
We believe that designers of all languages supporting this mix of features
need to grapple with how to best mix these features; those other designers may wish to
follow our lead in formalising the problem to seek the most stable design.
While stability is uninteresting
in languages featuring pure explicit or pure implicit instantiation,
it turns out to be an important metric in the presence of mixed behaviour.

Other work on type systems tends to focus on other properties; there is
thus little related work beyond the papers we have already cited.

We introduced a family of type systems, parameterised over the instantiation
flavour, and featuring a mix of explicit and implicit behaviour; these systems
are inspired by \citet{practical-type-inference}, \citet{visible-type-application},
and \citet{quick-look}. Using this
family, we then evaluated the different flavours of instantiation, against a
set of formal stability properties.
The results are surprisingly unambiguous: (a) \emph{lazy instantiation} achieves the
highest stability for the compile time semantics, and (b) \emph{shallow instantiation}
results in the most stable runtime semantics.


==> tex/sections/FormalProofs.tex <==
%if style == newcode
\begin{code}
module FormalProofs where
\end{code}
%endif

\section{Proofs}
\label{app:formalproofs}

This section provides the proofs for the properties discussed in
Section~\ref{sec:evaluation}.

\subsection{Let-Inlining and Extraction}
\label{app:prop1}
% ---------- %
% PROPERTY 1 %
% ---------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:let_inlining}{Property \ref{prop:let_inlining}}
\begin{prop:let_inlining}[Let Inlining is Type Preserving]\
  \begin{shortItemize}
  \item \( \text{If}~[[ G |-E let x = ee1 in ee2 => ne ~> ef ]]~\text{then}~[[ G |-E [ ee1 / x ] ee2 => ne ~> ef ]] \)
  \item \( \text{If}~[[ G |-E let x = ee1 in ee2 <= s ~> ef ]]~\text{then}~[[ G |-E [ ee1 / x ] ee2 <= s ~> ef ]] \)
  \end{shortItemize}
\end{prop:let_inlining}
Before proving Property~\ref{prop:let_inlining}, we first introduce a number of helper lemmas:
\begin{lemma}[Expression Inlining is Type Preserving (Synthesis)]\ \\
  \( \text{If}~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , x : forall ias . ne1 , G2 |-E ee2 => ne2 ~> ef2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]] \) \\
  \( \text{then}~[[ G1 , G2 |-E [ ee1 / x ] ee2 => ne2 ~> ef3 ]] \)
  \label{lem:exp_inlining_type_synth}
\end{lemma}
\begin{lemma}[Expression Inlining is Type Preserving (Checking)]\ \\
  \( \text{If}~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , x : forall ias . ne1 , G2 |-E ee2 <= s2 ~> ef2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]] \) \\
  \( \text{then}~[[ G1 , G2 |-E [ ee1 / x ] ee2 <= s2 ~> ef3 ]] \)
  \label{lem:exp_inlining_type_check}
\end{lemma}
\begin{lemma}[Head Inlining is Type Preserving]\ \\
  \( \text{If}~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , x : forall ias . ne1 , G2 |-H h => s2 ~> ef2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]] \) \\
  \( \text{then}~[[ G1 , G2 |-H [ ee1 / x ] h => s2 ~> ef3 ]] \)
  \label{lem:head_inlining_type}
\end{lemma}
\begin{lemma}[Argument Inlining is Type Preserving]\ \\
  \( \text{If}~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , x : forall ias . ne1 , G2 |-A args <= s1 => s2 ~> fargs ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]] \) \\
  \( \text{then}~[[ G1 , G2 |-A [ ee1 / x ] args <= s1 => s2 ~> fargs ]] \)
  \label{lem:arg_inlining_type}
\end{lemma}
\begin{lemma}[Declaration Inlining is Type Preserving]\ \\
  \( \text{If}~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , x : forall ias . ne1 , G2 |-E edecl => G3 ~> x : s = ef3 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]] \) \\
  \( \text{then}~[[ G1 , G2 |-E [ ee1 / x ] edecl => G3 ~> x : s = ef3 ]] \)
  \label{lem:decl_inlining_type}
\end{lemma}

\begin{figure*}
  \input{tex/figures/Dependencies.mng}
  \caption{Relation dependencies}
  \label{fig:dependencies}
\end{figure*}

% \begin{figure}
%   \includegraphics[width=0.4\textwidth]{tex/figures/Prop1Helpers.png}
%   \caption{Property~\ref{prop:let_inlining} helper dependencies}
%   \label{fig:prop1helpers}
% \end{figure}

Figure~\ref{fig:dependencies} shows the dependencies between the different relations,
and by extension the different helper lemmas.
An arrow from $A$ to $B$ denotes that $B$ depends on $A$.
Note that these 5 lemmas need to be proven through mutual induction.
The proof proceeds by structural induction on the second typing derivation.
While the number of cases gets quite large, each case is entirely trivial.

Using these additional lemmas, we then continue proving Property~\ref{prop:let_inlining}. By case analysis on the premise (\rref{Tm-InfLet} or \rref{Tm-CheckLet}, followed by \rref{Decl-NoAnnSingle}), we learn that 
\( [[ G |-E x = ee1 => G , x : forall ias . ne1 ~> x : s = ef ]] \), 
\( [[ G |-E ee1  => ne1 ~> ef ]] \), and either
\( [[ G , x : forall ias . ne1 |-E ee2 => ne ~> ef ]] \) or
\( [[ G , x : forall ias . ne1 |-E ee2 <= s ~> ef ]] \).
Both parts of the goal now follow trivially from Lemma~\ref{lem:exp_inlining_type_synth} and~\ref{lem:exp_inlining_type_check} respectively.
\qed

% ---------- %
% PROPERTY 3 %
% ---------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:let_extraction}{Property \ref{prop:let_extraction}}
\begin{prop:let_extraction}[Let Extraction is Type Preserving]\
  \begin{shortItemize}
  \item \( \text{If}~[[ G |-E [ ee1 / x ] ee2 => ne2 ~> ef ]]~\text{and}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{then}~[[ G |-E let x = ee1 in ee2 => ne2 ~> ef ]] \)
  \item \( \text{If}~[[ G |-E [ ee1 / x ] ee2 <= s2 ~> ef ]]~\text{and}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{then}~[[ G |-E let x = ee1 in ee2 <= s2 ~> ef ]] \)
  \end{shortItemize}
\end{prop:let_extraction}
Similarly to before, we start by introducing a number of helper lemmas:
\begin{lemma}[Expression Extraction is Type Preserving (Synthesis)]\ \\
  \( \text{If}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G |-E [ ee1 / x ] ee2 => ne2 ~> ef3 ]] \) \\
  \( \text{then}~[[ G , x : forall ias . ne1 |-E ee2 => ne2 ~> ef2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G ) ]] \)
  \label{lem:exp_extraction_type_synth}
\end{lemma}
\begin{lemma}[Expression Extraction is Type Preserving (Checking)]\ \\
  \( \text{If}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G |-E [ ee1 / x ] ee2 <= s2 ~> ef3 ]] \) \\
  \( \text{then}~[[ G , x : forall ias . ne1 |-E ee2 <= s2 ~> ef2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G ) ]] \)
  \label{lem:exp_extraction_type_check}
\end{lemma}
\begin{lemma}[Head Extraction is Type Preserving]\ \\
  \( \text{If}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G |-H [ ee1 / x ] h => s2 ~> ef3 ]] \) \\
  \( \text{then}~[[ G , x : forall ias . ne1 |-H h => s2 ~> ef2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G ) ]] \)
  \label{lem:head_extraction_type}
\end{lemma}
\begin{lemma}[Argument Extraction is Type Preserving]\ \\
  \( \text{If}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G |-A [ ee1 / x ] args <= s1 => s2 ~> fargs ]] \) \\
  \( \text{then}~[[ G , x : forall ias . ne1 |-A args <= s1 => s2 ~> fargs ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G ) ]] \)
  \label{lem:arg_extraction_type}
\end{lemma}
\begin{lemma}[Declaration Extraction is Type Preserving]\ \\
  \( \text{If}~[[ G |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G |-E [ ee1 / x ] edecl => G , G' ~> x : s = ef3 ]] \) \\
  \( \text{then}~[[ G , x : forall ias . ne1 |-E edecl => G , x : forall ias . ne1 , G' ~> x : s = ef3 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G ) ]] \)
  \label{lem:decl_extraction_type}
\end{lemma}

In addition to these helper lemmas, we also introduce two typing context lemmas:
\begin{lemma}[Environment Variable Shifting is Type Preserving]\
  \begin{shortItemize}
  \item \( \text{If}~[[ G1 , x1 : s1 , x2 : s2 , G2 |-E ee => ne ~> ef ]]~\text{then}~[[ G1 , x2 : s2 , x1 : s1 , G2 |-E ee => ne ~> ef ]] \) 
  \item \( \text{If}~[[ G1 , x1 : s1 , x2 : s2 , G2 |-E ee <= s ~> ef ]]~\text{then}~[[ G1 , x2 : s2 , x1 : s1 , G2 |-E ee <= s ~> ef ]] \)
  \end{shortItemize}
  \label{lem:var_shifting_type}
\end{lemma}
\begin{lemma}[Environment Type Variable Shifting is Type Preserving]\
  \begin{shortItemize}
  \item \( \text{If}~[[ G1 , a , x : s , G2 |-E ee => ne ~> ef ]]~\text{and}~[[ empty = fv ( s ) \ dom ( G1 ) ]]~\text{then}~[[ G1 , x : s , a , G2 |-E ee => ne ~> ef ]] \)
  \item \( \text{If}~[[ G1 , a , x : s , G2 |-E ee <= s ~> ef ]]~\text{and}~[[ empty = fv ( s ) \ dom ( G1 ) ]]~\text{then}~[[ G1 , x : s , a , G2 |-E ee <= s ~> ef ]] \)
  \item \( \text{If}~[[ G1 , x : s , a , G2 |-E ee => ne ~> ef ]]~\text{then}~[[ G1 , a , x : s , G2 |-E ee => ne ~> ef ]] \)
  \item \( \text{If}~[[ G1 , x : s , a , G2 |-E ee <= s ~> ef ]]~\text{then}~[[ G1 , a , x : s , G2 |-E ee <= s ~> ef ]] \)
  \end{shortItemize}
  \label{lem:tyvar_shifting_type}
\end{lemma}
Lemmas~\ref{lem:var_shifting_type} and~\ref{lem:tyvar_shifting_type} are folklore, and can be proven through straightforward induction.

Now we can go about proving Lemmas~\ref{lem:exp_extraction_type_synth} till~\ref{lem:decl_extraction_type}. Similarly to the Property~\ref{prop:let_inlining} helper lemmas, they have to be proven using mutual induction. Most cases are quite straightforward, and we will focus only on Lemma~\ref{lem:head_extraction_type}. We start by performing case analysis on \( [[ h ]] \):

\case{\( [[ h ]] = [[ y ]]~\text{where}~[[ y ]] = [[ x ]] \)}

By evaluating the substitution, we know from the premise that
\( [[ G |-E ee1 => ne1 ~> ef1 ]] \) and \( [[ G |-H ee1 => s2 ~> ef2 ]] \), while the goal remains \( [[ G , x : forall ias . ne1 |-H x => s2 ~> ef3 ]] \). It is clear from \rref{H-Var} that in order for the goal to hold, \( [[ s2 ]] = [[ forall ias . ne1 ]] \). We proceed by case analysis on the second derivation:

\subcase{\rref{H-Var} \([[ ee1 ]] = [[ x' ]] \) : }
The rule premise tells us that \([[ x' : s2 \in G ]]\). The goal follows directly under lazy instantiation. However, under eager instantiation, \rref{Tm-InfApp} instantiates the type \([[ G |- s2 inst _ d ne1 ~> ewf ]]\) making the goal invalid.

\subcase{\rref{H-Con} \([[ ee1 ]] = [[ K ]] \), \rref{H-Ann} \([[ ee1 ]] = [[ ee3 : s3 ]] \), \rref{H-Inf} \([[ ee1 ]] = [[ ee1 ]] \), \rref{H-Undef} \([[ ee1 ]] = [[ undefined ]] \), or \rref{H-Seq} \([[ ee1 ]] = [[ seq ]] \) : }

Similarly to the previous case, the goal is only valid under eager instantiation.

\case{\( [[ h ]] = [[ y ]]~\text{where}~[[ y ]] \neq [[ x ]] \)}

This case is trivial, as the substitution \([[ [ ee1 / x ] ]]\) does not alter \([[h]]\). The result thus follows from weakening.

\case{\( [[ h ]] = [[ K ]] \), \( [[ h ]] = [[ undefined ]] \), or \( [[ h ]] = [[ seq ]] \)}

Similarly to the previous case, as the substitution does not alter \([[h]]\), the result thus follows from weakening.

\case{\( [[ h ]] = [[ ee : s ]] \)}

The result follows by applying Lemma~\ref{lem:exp_extraction_type_check}.

\case{\( [[ h ]] = [[ ee ]] \)}

The result follows by applying Lemma~\ref{lem:exp_extraction_type_synth}.
\qed

Using these lemmas, both Property~\ref{prop:let_extraction} goals follow straightforwardly using \rref{Decl-NoAnnSingle}, in combination with \rref{Tm-InfLet} and Lemma~\ref{lem:exp_extraction_type_synth} or \rref{Tm-CheckLet} and Lemma~\ref{lem:exp_extraction_type_check}, respectively.
\qed

\renewcommand\elab[1]{#1}
\subsection{Contextual Equivalence}
\label{app:ctx_equiv}
% ---------- %
% Ctx Equiv  %
% ---------- %
As we've now arrived at properties involving the runtime semantics of the language, we first need to formalise our definition of contextual equivalence, and introduce a number of useful lemmas.

\begin{definition}[Contextual Equavalence]
  \begin{align*}
    [[ef1 =ctx ef2]] &\equiv [[ G |- ef1 : s1 ]] \quad \wedge \quad [[ G |- s1 inst _ d r3 ~> ewf1 ]] \\
    &\wedge [[ G |- ef2 : s2]] \quad \wedge \quad [[ G |- s2 inst _ d r3 ~> ewf2 ]] \\
    &\wedge \forall [[ fctx : G ; r3 |-> empty ; Bool ]], \\
    & \exists [[ fval ]] : [[ fctx [ ewf1 [ ef1 ] ] |~>* fval ]] \quad \wedge \quad [[ fctx [ ewf2 [ ef2 ] ] |~>* fval ]]
  \end{align*}
\end{definition}
This definition for contextual equivalence is modified from~\citet[Chapter 46]{PFPL}.
Two core expressions are thus contextually equivalent,
if a common type exists to which both their types instantiate,
and if no (closed) context can distinguish between them.
This can either mean that both applied expressions evaluate to the same value $[[fval]]$
or both diverge.
Note that while we require the context to map to a closed, Boolean expression,
other base types, like $[[Int]]$, would have been valid alternatives as well.

We first introduce reflexivity, commutativity and transitivity lemmas:
\begin{lemma}[Contextual Equivalence Reflexivity]\ \\
  \( \text{If}~[[ G |- ef : s ]]~\text{then}~[[ ef =ctx ef ]] \)
  \label{lem:ctx_equiv_refl}
\end{lemma}
The proof follows directly from the definition of contextual equivalence, along with the determinism of System F evaluation.
\begin{lemma}[Contextual Equivalence Commutativity]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{then}~[[ ef2 =ctx ef1 ]] \)
  \label{lem:ctx_equiv_comm}
\end{lemma}
Trivial proof by unfolding the definition of contextual equivalence.
\begin{lemma}[Contextual Equivalence Transitivity]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{and}~[[ ef2 =ctx ef3 ]]~\text{then}~[[ ef1 =ctx ef3 ]] \)
  \label{lem:ctx_equiv_trans}
\end{lemma}
Trivial proof by unfolding the definition of contextual equivalence.

Furthermore, we also introduce a number of compatibility lemmas for the contextual equivalence relation, along with two helper lemmas:
\begin{lemma}[Compatibility Term Abstraction]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{then}~[[ \ x : s . ef1 =ctx \ x : s . ef2 ]] \)
  \label{lem:compat_abs}
\end{lemma}
\begin{lemma}[Compatibility Term Application]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{and}~[[ ef1' =ctx ef2' ]]~\text{then}~[[ ef1 ef1' =ctx ef2 ef2' ]] \)
  \label{lem:compat_app}
\end{lemma}
\begin{lemma}[Compatibility Type Abstraction]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{then}~[[ /\ a . ef1 =ctx /\ a . ef2 ]] \)
  \label{lem:compat_tyabs}
\end{lemma}
\begin{lemma}[Compatibility Type Application]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{then}~[[ ef1 s =ctx ef2 s ]] \)
  \label{lem:compat_tyapp}
\end{lemma}
\begin{lemma}[Compatibility Case Abstraction]\ \\
  \( \text{If}~\forall~i : [[ ef1i =ctx ef2i ]]~\text{then}~[[ case </ fpsi : fpsigs -> ef1i // i /> =ctx case </ fpsi : fpsigs -> ef2i // i /> ]] \)
  \label{lem:compat_case}
\end{lemma}
\begin{lemma}[Compatibility Expression Wrapper]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{then}~[[ ewf [ ef1 ] =ctx ewf [ ef2 ] ]] \)
  \label{lem:compat_wrapper}
\end{lemma}
\begin{lemma}[Compatibility Helper Forwards]\ \\
  \( \text{If}~[[ fctx [ ef1 ] |~>* fval ]]~\text{and}~[[ ef1 |~> ef2 ]]~\text{then}~[[ fctx [ ef2 ] |~>* fval ]] \)
  \label{lem:compat_helper_forward}
\end{lemma}
\begin{lemma}[Compatibility Helper Backwards]\ \\
  \( \text{If}~[[ fctx [ ef2 ] |~>* fval ]]~\text{and}~[[ ef1 |~> ef2 ]]~\text{then}~[[ fctx [ ef1 ] |~>* fval ]] \)
  \label{lem:compat_helper_backward}
\end{lemma}
The helper lemmas are proven by straightforward induction on the evaluation step derivation.
We will prove Lemma~\ref{lem:compat_tyabs} as an example, as it is non-trivial.
The other compatibility lemmas are proven similarly.

We start by unfolding the definition of contextual equivalence in both the premise:
\([[ G |- ef1 : s1 ]]\), \([[ G |- s1 inst _ d r3 ~> ewf1 ]]\),
\([[ G |- ef2 : s2 ]]\), \([[ G |- s2 inst _ d r3 ~> ewf2 ]]\),
\( \forall [[ fctx : G ; r3 |-> empty ; Bool ]]\),
\( \exists [[fval]] : [[ fctx [ ewf1 [ ef1 ] ] |~>* fval ]] \) and
\( [[ fctx [ ewf2 [ ef2 ] ] |~>* fval ]]\).
Unfolding the definition reduces the goal to be proven to
\([[ G' |- /\ a . ef1 : s1' ]]\), \([[ G' |- s1' inst _ d r3' ~> ewf1' ]]\),
\([[ G' |- /\ a . ef2 : s2' ]]\), \([[ G' |- s2' inst _ d r3' ~> ewf2' ]]\),
\( \forall [[ fctx' : G' ; r3' |-> empty ; Bool ]]\),
\( \exists [[fval']] : [[ fctx' [ ewf1' [ /\ a . ef1 ] ] |~>* fval' ]] \) and
\( [[ fctx' [ ewf2' [ /\ a . ef2 ] ] |~>* fval' ]]\).

The typing judgement goals follow directly from \rref{FTm-TyAbs},
where we take \([[ s1' ]] = [[ forall a . s1 ]]\), \([[ s2' ]] = [[ forall a . s2 ]]\)
and \([[ G' ]] = [[ [ t / a ] G ]]\) for some \([[t]]\).

As we know \([[ G |- s1 inst _ d r3 ~> ewf1 ]]\), it is easy to see that
\([[ [ t / a ] G |- [ t / a ] s1 inst _ d [ t / a ] r3 ~> [ t / a ] ewf1 ]]\),
and similarly for \([[ [ t / a ] s2 ]]\).
Using this, the instantiation goals follow from \rref{InstT-SForall} and~\rref{InstT-Forall}
with \([[ r3' ]] = [[ [ t / a ] r3 ]]\),
\([[ ewf1' ]] = [[ \ ef . ( [ t / a ] ewf1 [ ef t ] ) ]]\) and
\([[ ewf2' ]] = [[ \ ef . ( [ t / a ] ewf2 [ ef t ] ) ]]\).

Finally, by inlining the definitions, the first halve of the third goal becomes
\([[ fctx' [ ( \ ef . ( [ t / a ] ewf1 [ ef t ] ) ) [ /\ a . ef1 ] ] |~>* fval' ]]\).
This reduces to
\([[ fctx' [ [ t / a ] ewf1 [ ( /\ a . ef1 ) t ] ] |~>* fval' ]]\).
By lemma~\ref{lem:compat_helper_forward} (note that we can consider the combination
of a context and an expression wrapper as a new context):
\([[ fctx' [ [ t / a ] ewf1 [ [ t / a ] ef1 ] ] |~>* fval' ]]\).
We can now bring the substitutions to the front, and reduce the goal
(by Lemma~\ref{lem:compat_helper_backward})
\([[ fctx'' [ ewf1 [ ef1 ] ] |~>* fval' ]]\) where we define
\([[ fctx'' ]] = [[ \ ef . fctx' [ ( /\ a . ef ) t ] ]]\)
(note that we use \( \lambda t \) as meta-notation here, to simplify our definition of \([[fctx'']]\)).
We perform the same derivation for the second halve of the goal:
\([[ fctx'' [ ewf2 [ ef2 ] ] |~>* fval' ]]\).
As \([[ fctx'' : G ; r3 |-> empty ; Bool ]]\), the goal follows directly from
the unfolded premise, where \( [[ fval' ]] = [[ fval ]] \).
\qed

We introduce an additional lemma stating that instantiating the type of expressions does not alter their behaviour:
\begin{lemma}[Type Instantiation is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G |- ef : s ]]~\text{and}~[[ G |- s inst _ d r ~> ewf ]]~\text{then}~[[ ef =ctx ewf [ ef ] ]] \)
  \label{lem:inst_dyn}
\end{lemma}
The proof proceeds by induction on the instantiation relation:

\case{\rref{InstT-SInst} \( [[ ewf ]] = [[ [] ]] \) : }

Trivial case, as \( [[ ewf [ ef ] ]] = [[ ef ]] \), the goal follows directly from Lemma~\ref{lem:ctx_equiv_refl}.

\case{\rref{InstT-SForall} \( [[ ewf ]] = [[ \ ef1 . ( ewf' [ ef1 t ] ) ]] \) : }

We know from the first premise, along with \rref{FTm-TyApp} that \( [[ G |- ef t : [ t / a ] s' ]] \) where \( [[ s = forall a . s' ]] \). By applying the induction hypothesis we get \( [[ ef t =ctx ewf' [ ef t ] ]] \). The goal to be proven is \( [[ ef =ctx ( \ ef1 . ( ewf' [ ef1 t ] ) ) [ ef ] ]] \), which reduces to \( [[ ef =ctx ewf' [ ef t ] ]] \). By unfolding the definition of contextual equivalence in both the goal and the induction hypothesis result (using Lemma~\ref{lem:ctx_equiv_trans}), the remaining goals are:
\begin{shortItemize}
\item \( [[ G |- ef : s1 ]] \) : follows directly from the first premise.
\item \( [[ G |- forall a . s' instS _ S r' ~> ewf1 ]] \) and \( [[ G |- r' instS _ S r ~> ewf2 ]] \) : follows directly from the premise if we take \([[r']] = [[r]]\), \([[ ewf1 ]] = [[ ewf ]]\) and \([[ ewf2 ]] = [[ [] ]]\).
\item \( [[ fctx [ ewf1 [ ef ] ] |~>* fval ]] \) and \( [[ fctx [ ewf [ ef ] ] |~>* fval ]] \) : trivial as both sides are identical and evaluation is deterministic.
\end{shortItemize}

\case{\rref{InstT-SInfForall} \( [[ ewf ]] = [[ \ ef1 . ( ewf' [ ef1 t ] ) ]] \) : }

The proof follows analogously to the previous case. We have thus proven Lemma~\ref{lem:inst_dyn} under shallow instantiation.

\case{\rref{InstT-Mono} \( [[ ewf ]] = [[ [] ]] \) : }

Trivial case, as \( [[ ewf [ ef ] ]] = [[ ef ]] \), the goal follows directly from Lemma~\ref{lem:ctx_equiv_refl}.

\case{\rref{InstT-Function} \( [[ ewf ]] = [[ \ ef1 . \ x : s1 . ( ewf' [ ef1 x ] ) ]] \) : }

It is clear that the goal does not hold in this case. Under deep instantiation, full eta expansion is performed, which alters the evaluation behaviour. Consider for example \( [[ undefined ]] \) and its expansion \( [[ \ x : s . undefined x ]] \).
\qed

Finally, we introduce a lemma stating that evaluation preserves contextual equivalence.
However, in order to prove it, we first need to introduce the common preservation lemma:
\begin{lemma}[Preservation]\ \\
  \( \text{If}~[[ G |- ef : s ]]~\text{and}~[[ ef |~> ef' ]]~\text{then}~[[ G |- ef' : s ]] \)
  \label{lem:pres}
\end{lemma}
The preservation proof for System F is folklore, and proceeds by straightforward induction on the evaluation relation.

\begin{lemma}[Evaluation is Contextual Equivalence Preserving]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{and}~[[ ef2 |~> ef2' ]]~\text{then}~[[ ef1 =ctx ef2' ]] \)
  \label{lem:eval_pres}
\end{lemma}
The proof follows by Lemma~\ref{lem:pres} (to cover type preservation) and Lemma~\ref{lem:compat_helper_forward} (to cover the evaluation aspect).

\subsection{Let-Inlining and Extraction, Continued}
\label{app:prop2}
% ---------- %
% PROPERTY 2 %
% ---------- %
\newtheorem*{prop:let_inlining_dyn}{Property \ref{prop:let_inlining_dyn}}
\begin{prop:let_inlining_dyn}[Let Inlining is Runtime Semantics Preserving]\
  \begin{shortItemize}
  \item \( \text{If}~[[ G |-E let x = ee1 in ee2 => ne ~> ef1 ]]~\text{and}~[[ G |-E [ ee1 / x ] ee2 => ne ~> ef2 ]]~\text{then}~[[ ef1 =ctx ef2 ]] \)
  \item \( \text{If}~[[ G |-E let x = ee1 in ee2 <= s ~> ef1 ]]~\text{and}~[[ G |-E [ ee1 / x ] ee2 <= s ~> ef2 ]]~\text{then}~[[ ef1 =ctx ef2 ]] \)
  \end{shortItemize}
\end{prop:let_inlining_dyn}

We first need typing preservation lemmas before we can prove
Property~\ref{prop:let_inlining_dyn}.
\begin{lemma}[Expression Typing Preservation (Synthesis)]\ \\
  \( \text{If}~[[ G |-E ee => n ~> ef ]]~\text{then}~[[ G |- ef : n ]] \)
  \label{lem:expr_typ_pres_inf}
\end{lemma}
\begin{lemma}[Expression Typing Preservation (Checking)]\ \\
  \( \text{If}~[[ G |-E ee <= s ~> ef ]]~\text{then}~[[ G |- ef : s ]] \)
  \label{lem:expr_typ_pres_check}
\end{lemma}
\begin{lemma}[Head Typing Preservation]\ \\
  \( \text{If}~[[ G |-H h => s ~> ef ]]~\text{then}~[[ G |- ef : s ]] \)
  \label{lem:head_typ_pres}
\end{lemma}
\begin{lemma}[Argument Typing Preservation]\ \\
  \( \text{If}~[[ G |-A args <= s => s' ~> fargs ]]~\text{then}~\forall [[efi]] \in [[fargs]] : [[ G |- efi : si ]] \)
  \label{lem:args_typ_pres}
\end{lemma}
\begin{lemma}[Declaration Typing Preservation]\ \\
  \( \text{If}~[[ G |-E edecl => G' ~> x : s = ef ]]~\text{then}~[[ G |- ef : s ]] \)
  \label{lem:decl_typ_pres}
\end{lemma}
Similarly to the helper lemmas for Property~\ref{prop:let_inlining}, these lemmas need to be proven using mutual induction. The proofs follow through straightforward induction on the typing derivation.

We continue by introducing another set of helper lemmas:
\begin{lemma}[Expression Inlining is Runtime Semantics Preserving (Synthesis)]\ \\
  \( \text{If}~[[ G1 , x : forall ias . ne1 , G2 |-E ee2 => ne2 ~> ef2 ]],~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , G2 |-E [ ee1 / x ] ee2 => ne2 ~> ef3 ]] \)
  \( \text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]]~\text{then}~[[ ef3 =ctx ( \ x : forall as . ne1 . ef2 ) ef1 ]] \)
  \label{lem:prop2helper_expr_inf}
\end{lemma}
\begin{lemma}[Expression Inlining is Runtime Semantics Preserving (Checking)]\ \\
  \( \text{If}~[[ G1 , x : forall ias . ne1 , G2 |-E ee2 <= s2 ~> ef2 ]],~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , G2 |-E [ ee1 / x ] ee2 <= s2 ~> ef3 ]] \)
  \( \text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]]~\text{then}~[[ ef3 =ctx ( \ x : forall as . ne1 . ef2 ) ef1 ]] \)
  \label{lem:prop2helper_expr_check}
\end{lemma}
\begin{lemma}[Head Inlining is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G1 , x : forall ias . ne1 , G2 |-H h => s ~> ef2 ]],~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , G2 |-H [ ee1 / x ] h => s ~> ef3 ]] \)
  \( \text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]]~\text{then}~[[ ef3 =ctx ( \ x : forall as . ne1 . ef2 ) ef1 ]] \)
  \label{lem:prop2helper_head}
\end{lemma}
\begin{lemma}[Argument Inlining is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G1 , x : forall ias . ne1 , G2 |-A args <= s1 => s2 ~> fargs1 ]],~[[ G1 |-E ee1 => ne1 ~> ef1 ]] \) \\
  \( \text{and}~[[ G1 , G2 |-A [ ee1 / x ] args <= s1 => s2 ~> fargs2 ]]~\text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]] \) \\
  \( \text{then}~\forall [[efi]] \in [[fargs1]],~[[efi']] \in [[fargs2]]~:~[[ efi' =ctx ( \ x : forall as . ne1 . efi ) ef1 ]] \)
  \label{lem:prop2helper_args}
\end{lemma}
\begin{lemma}[Declaration Inlining is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G1 , x : forall ias . ne1 , G2 |-E edecl => G3 ~> y : s2 = ef2 ]],~[[ G1 |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G1 , G2 |-E [ ee1 / x ] edecl => G3 ~> y : s2 = ef3 ]] \)
  \( \text{where}~[[ as = fv ( ne1 ) \ dom ( G1 ) ]]~\text{then}~[[ ef3 =ctx ( \ x : forall as . ne1 . ef2 ) ef1 ]] \)
  \label{lem:prop2helper_decl}
\end{lemma}
As is probably clear by now, these lemmas are proven through mutual induction. The proof proceeds by structural induction on the first typing derivation. We will focus on the non-trivial cases:

\case{\rref{H-Var} \( [[ h ]] = [[ y ]]~\text{where}~[[ y ]] = [[ x ]] \) : }

The goal reduces to \( [[ ef1 =ctx ( \ x : forall as . ne1 . x ) ef1 ]] \), which follows directly from Lemmas~\ref{lem:ctx_equiv_refl} and~\ref{lem:eval_pres}.

\case{\rref{H-Var} \( [[ h ]] = [[ y ]]~\text{where}~[[ y ]] \neq [[ x ]] \) : }

The goal reduces to \( [[ y =ctx ( \ x : forall as . ne1 . y ) ef1 ]] \). Since \( [[ ( \ x : forall as . ne1 . y ) ef1 |~> y ]] \), the goal follows directly from Lemmas~\ref{lem:ctx_equiv_refl} and~\ref{lem:eval_pres}.

\case{\rref{Tm-InfAbs} \( [[ ee2 ]] = [[ \ y . ee4 ]] \) : }

The premise tells us \( [[ G1 , x : forall ias . ne1 , G2 , y : t1 |-E ee4 => ne4 ~> ef4 ]] \) and \( [[ G1 , G2 , y : t1 |-E [ ee1 / x ] ee4 => ne4 ~> ef5 ]] \).
Applying the induction hypothesis gives us \( [[ ef5 =ctx ( \ x : forall as . ne1 . ef4 ) ef1 ]] \).
The goal reduces to \( [[ \ y : t1 . ef5 =ctx ( \ x : forall as . ne1 . \ y : t1 . ef4 ) ef1 ]] \).
In order not to clutter the proof too much, we introduce an additional helper lemma~\ref{lem:prop2helper1}.
The goal then follows from Lemmas~\ref{lem:compat_abs} and~\ref{lem:prop2helper1}.

\case{\rref{Tm-InfTyAbs} \( [[ ee2 ]] = [[ /\ a . ee4 ]] \) : }

The premise tells us \( [[ G1 , x : forall ias . ne1 , G2 , a |-E ee4 => ne4 ~> ef4 ]] \), \( [[ G1 , G2 , a |-E [ ee1 / x ] ee4 => ne4 ~> ef5 ]] \) and \( [[ G1 , G2 |- forall a . ne4 inst _ d ne5 ~> ewf ]] \).
Applying the induction hypothesis gives us \( [[ ef5 =ctx ( \ x : forall as . ne1 . ef4 ) ef1 ]] \).
The goal reduces to \( [[ ewf [ /\ a . ef5 ] =ctx ( \ x : forall as . ne1 . ewf [ /\ a . ef4 ] ) ef1 ]] \).
Similarly to before, we avoid cluttering the proof by introducing an additional helper lemma~\ref{lem:prop2helper2}.
The goal then follows from Lemmas~\ref{lem:compat_tyabs}, \ref{lem:inst_dyn} and~\ref{lem:prop2helper2}.
\qed

\begin{lemma}[Property~\ref{prop:let_inlining_dyn} Term Abstraction Helper]\ \\
  \( \text{If}~[[ G |- \ x : s2 . ( ( \ y : s1 . ef2 ) ef1 ) : s3 ]]~\text{and}~[[ G |- ef1 : s1 ]]~\text{then}~[[ \ x : s2 . ( ( \ y : s1 . ef2 ) ef1 ) =ctx ( \ y : s1 . \ x : s2 . ef2 ) ef1 ]] \)
  \label{lem:prop2helper1}
\end{lemma}
\begin{lemma}[Property~\ref{prop:let_inlining_dyn} Type Abstraction Helper]\ \\
  \( \text{If}~[[ G |- /\ a . ( ( \ x : s1 . ef2 ) ef1 ) : s2 ]]~\text{and}~[[ a notin fv ( s1 ) ]]~\text{then}~[[ /\ a . ( ( \ x : s1 . ef2 ) ef1 ) =ctx ( \ x : s1 . /\ a . ef2 ) ef1 ]] \)
  \label{lem:prop2helper2}
\end{lemma}
Both lemmas follow from the definition of contextual equivalence.

We now return to proving Property~\ref{prop:let_inlining_dyn}. By case analysis (Either \rref{Tm-InfLet} or \rref{Tm-CheckLet}, followed by \rref{Decl-NoAnnSingle}) we know
\( [[ G , x : forall ias . ne1 |-E ee2 => ne ~> ef3 ]] \) or \( [[ G , x : forall ias . ne1 |-E ee2 <= s ~> ef3 ]] \)
where \( [[ ef1 = ( \ x : forall as . ne1 . ef3 ) ef4 ]] \), 
\( [[ G |-E ee1 => ne1 ~> ef4 ]] \) and \( [[ as = fv ( ne1 ) \ dom ( G ) ]] \).
The goal thus follows directly from Lemma~\ref{lem:prop2helper_expr_inf} or~\ref{lem:prop2helper_expr_check}. However, as Lemma~\ref{lem:inst_dyn} only holds under shallow instantiation, we cannot prove Property~\ref{prop:let_inlining_dyn} under deep instantiation.
\qed

\subsection{Type Signatures}
\label{app:prop5}
% ---------- %
% PROPERTY 5 %
% ---------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:signature_type_single}{Property \ref{prop:signature_type_single}}
\begin{prop:signature_type_single}[Signature Property is Type Preserving]\ \\
  \( \text{If}~[[ G |-E x ps = ee => G' ~> x : s = ef ]]~\text{and}~[[ x : s \in G' ]]~\text{then}~[[ G |-E x : s ; x ps = ee => G' ~> x : s = ef ]] \)
\end{prop:signature_type_single}

Before proving Property~\ref{prop:signature_type_single}, we first introduce a number of helper lemmas:
\begin{lemma}[Skolemisation Exists]\ \\
  \( \text{If}~[[ fv ( s ) \in G ]]~\text{then}~\exists [[r]], [[G']]~\text{such that}~[[ G |- s skol _ d r ; G' ~> ewf ]] \)
  \label{lem:skol_exists}
\end{lemma}
The proof follows through careful examination of the skolemisation relation.

\begin{lemma}[Skolemisation Implies Instantiation]\ \\
  \( \text{If}~[[ G |- s skol _ d r ; G' ~> ewf ]]~\text{then}~[[ G' |- s inst _ d r ~> ewf' ]] \)
  \label{lem:skol_implies_inst}
\end{lemma}
The proof follows by straightforward induction on the skolemisation relation. Note that as skolemisation binds all type variables in \([[G']]\), they can then be used for instantiation.

\begin{lemma}[Inferred Type Binders Preserve Expression Checking]\ \\
  \( \text{If}~[[ G |-E ee <= s ~> ef ]]~\text{then}~[[ G |-E ee <= forall ias . s ~> ef' ]] \)
  \label{lem:inf_binders_pres_check}
\end{lemma}
The proof follows by straightforward induction on the typing derivation.

\begin{lemma}[Pattern Synthesis Implies Checking]\ \\
  \( \text{If}~[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]~\text{then}~\forall [[ s' ]], \exists [[ s ]] : [[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]~\text{where}~[[ type ( psigs ; s' ~ s ) ]] \)
  \label{lem:pat_inf_implies_check}
\end{lemma}
The proof follows by straightforward induction on the pattern typing derivation.

\begin{lemma}[Expression Synthesis Implies Checking]\ \\
  \( \text{If}~[[ G |-E ee => ne ~> ef ]]~\text{then}~[[ G |-E ee <= ne ~> ef' ]] \)
  \label{lem:exp_inf_implies_check}
\end{lemma}
The proof follows by induction on the typing derivation. We will focus on the non-trivial cases below:

\case{\rref{Tm-InfAbs} \([[ ee ]] = [[ \ x . ee' ]] \) : }

We know from the premise of the typing rule that \( [[ G , x : t1 |-E ee' => ne2 ~> ef1 ]] \) where \( [[ ne ]] = [[ t1 -> ne2 ]] \).
By \rref{Tm-CheckAbs}, the goal reduces to \( [[ G |- t1 -> ne2 skolS _ S t1 -> ne2 ; G ~> [] ]] \) (which follows directly by \rref{SkolT-SInst})
and \( [[ G , x : t1 |-E ee' <= ne2 ~> ef4 ]] \) (which follows by the induction hypothesis).

\case{\rref{Tm-InfTyAbs} \([[ ee ]] = [[ /\ a . ee' ]] \) : }

The typing rule premise tells us that \( [[ G , a |-E ee' => ne1 ~> ef1 ]] \) and \( [[ G |- forall a . ne1 inst _ d ne2 ~> ewf ]] \).
By \rref{Tm-CheckTyAbs}, the goal reduces to \( [[ ne2 ]] = [[ forall ias . forall a . s' ]] \) and \( [[ G , ias , a |-E ee' <= s' ~> ef2 ]] \).
It is now clear that this property can never hold under eager instantiation, as the forall type in \( [[ forall a . ne1 ]] \) would always be instantiated away. We will thus focus solely on lazy instantiation from here on out, where \( [[ ne2 ]] = [[ forall a . ne1 ]] \).
In this case, the goal follows directly from the induction hypothesis.

\case{\rref{Tm-InfApp} \([[ ee ]] = [[ h args ]] \) : }

We know from the typing rule premise that \( [[ G |-H h => s ~> ef1 ]] \), \( [[ G |-A args <= s => s' ~> fargs ]] \) and \( [[ G |- s' inst _ d ne ~> ewf ]] \).
Note that as we assume lazy instantiation, \( [[ ne ]] = [[ s' ]] \).
By \rref{Tm-CheckInf}, the goal reduces to \( [[ G |- ne skol _ d r ; G' ~> ewf' ]] \) (follows by Lemma~\ref{lem:skol_exists}),
\( [[ G' |-E h args => ne1 ~> ef2 ]] \) (follows by performing environment weakening on the premise, with \( [[ ne1 ]] = [[ ne ]] \) )
and \( [[ G' |- ne1 inst _ d r ~> ewf'' ]] \) (given that \( [[ ne1 ]] = [[ ne ]] \), this follows by Lemma~\ref{lem:skol_implies_inst}).
\qed

We now proceed with proving Property~\ref{prop:signature_type_single}, through case analysis on the declaration typing derivation (\rref{Decl-NoAnnSingle}):

We know from the typing rule premise that \( [[ G |-P ps => psigs ; Del ~> fps : fpsigs ]] \), \( [[ G , Del |-E ee => ne ~> ef ]] \), \( [[ type ( psigs ; ne ~ s1 ) ]] \) and \( [[ s ]] = [[ forall ias . s1 ]] \) where \( [[ as = fv ( s1 ) \ dom ( G ) ]] \).
By \rref{Decl-Ann}, the goal reduces to \( [[ G |-P ps <= forall ias . s1 => s2 ; Del2 ~> fps' : fpsigs' ]] \) and \( [[ G , Del2 |-E ee <= s2 ~> ef' ]] \).
We know from Lemma~\ref{lem:pat_inf_implies_check} that \( [[ G |-P ps <= s1 => s3 ; Del ~> fps'' : fpsigs'' ]] \) where \( [[ type ( psigs ; s3 ~ s1 ) ]] \).
Furthermore, from Lemma~\ref{lem:exp_inf_implies_check} we get \( [[ G , Del |-E ee <= ne ~> ef' ]] \). Note that we thus only prove Property~\ref{prop:signature_type_single} under lazy instantiation.
We now proceed by case analysis on \( [[ ps ]] \):

\case{\( [[ ps ]] = [[ empty ]] \) : }

The first goal now follows trivially by \rref{Pat-CheckEmpty} with \( [[ s2 ]] = [[ forall ias . s1 ]] \), \( [[ s1 ]] = [[ ne ]] \) and \( [[ Del ]] = [[ Del2 ]] = [[ empty ]] \).
The second goal follows by Lemma~\ref{lem:inf_binders_pres_check}.

\case{\( [[ ps ]] \neq [[ empty ]] \) : }

The first goal follows by repeated application of \rref{Pat-CheckInfForall} with \( [[ s2 ]] = [[ s3 ]] = [[ ne ]] \). The second goal then follows directly from Lemma~\ref{lem:exp_inf_implies_check}.
\qed

% ---------- %
% PROPERTY 6 %
% ---------- %
\renewcommand\elab[1]{#1}
\newtheorem*{prop:signature_dyn}{Property \ref{prop:signature_dyn}}
\begin{prop:signature_dyn}[Signature Property is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G |-E </ x psi = eei // i /> => G' ~> x : s = ef1 ]]~\text{and}~[[ G |-E x : s ; </ x psi = eei // i /> => G' ~> x : s = ef2 ]]~\text{then}~[[ ef1 =ctx ef2 ]] \)
\end{prop:signature_dyn}
We start by introducing a number of helper lemmas:

\begin{lemma}[Pattern Typing Mode Preserves Translation]\ \\
  \( \text{If}~[[ G |-P ps => psigs ; Del ~> fps1 : fpsigs1 ]]~\text{and}~[[ G |-P ps <= s => s' ; Del ~> fps2 : fpsigs2 ]]~\text{where}~[[ type ( psigs ; s' ~ s ) ]] \) \\
  \( \text{then}~[[ fps1 ]] = [[ fps2 ]]~\text{and}~[[ fpsigs1 ]] = [[ fpsigs2 ]] \)
  \label{lem:pat_mode_pres}
\end{lemma}
The proof follows by straightforward induction on the pattern type inference derivation.

\begin{lemma}[Compatibility One-Sided Type Abstraction]\ \\
  \( \text{If}~[[ ef1 =ctx ef2 ]]~\text{then}~[[ ef1 =ctx /\ a . ef2 ]] \)
  \label{lem:compat_onesided_tyabs}
\end{lemma}
The proof follows by the definition of contextual equivalence. Note that while the left and right hand sides have different types, they still instantiate to a single common type.

\begin{lemma}[Partial Skolemisation Preserves Type Checking and Runtime Semantics]\ \\
  \( \text{If}~[[ G |-E ee <= forall ias . s ~> ef1 ]]~\text{then}~[[ G , as |-E ee <= s ~> ef2 ]]~\text{where}~[[ ef1 =ctx ef2 ]] \).
  \label{lem:partial_skol}
\end{lemma}
The proof proceeds by induction on the type checking derivation. Note that every case performs a (limited) form of skolemisation. Every case proceeds by applying the induction hypothesis, followed by Lemma~\ref{lem:compat_onesided_tyabs}.

\begin{lemma}[Typing Mode Preserves Runtime Semantics]\ \\
  \( \text{If}~[[ G |-E ee => ne ~> ef1 ]]~\text{and}~[[ G |-E ee <= s ~> ef2 ]]~\text{where}~[[ G |- ne inst _ d r ~> ewf1 ]]~\text{and}~[[ G |- s inst _ d r ~> ewf2 ]] \) \\
  \( \text{then}~[[ ef1 =ctx ef2 ]] \)
  \label{lem:mode_pres_dyn}
\end{lemma}
The proof proceeds by induction on the first typing derivation.
Each case follows straightforwardly by applying the induction hypothesis,
along with the corresponding compatibility lemma (Lemmas~\ref{lem:compat_abs} till \ref{lem:compat_case}).

We now turn to proving property~\ref{prop:signature_dyn}, through case analysis on the first declaration typing derivation:

\case{\rref{Decl-NoAnnSingle} : }

We know from the premise of the first derivation that \( [[ G |-P ps => psigs ; Del ~> fps1 : fpsigs1 ]] \), \( [[ G , Del |-E ee => ne ~> ef1' ]] \), \( [[ type ( psigs ; ne ~ s1 ) ]] \), \( [[ ef1 = case fps1 : fpsigs1 -> ef1' ]] \)~\text{and}~\( [[ s = forall ias . s1 ]] \)~\text{where}~\( [[ as = fv ( s1 ) \ dom ( G ) ]] \).
By case analysis on the second derivation (\rref{Decl-Ann}), we get \( [[ G |-P ps <= forall ias . s1 => s2 ; Del ~> fps2 : fpsigs2 ]] \), \( [[ G , Del |-E ee <= s2 ~> ef2' ]] \)~\text{and}~\( [[ ef2 ]] = [[ case fps2 : fpsigs2 -> ef2' ]] \).

We proceed by case analysis on the patterns \( [[ ps ]] \):

\subcase{\( [[ ps ]] = [[ empty ]] \) : }
We know from \rref{Pat-InfEmpty}, \rref{Pat-CheckEmpty} and \rref{Type-Empty} that \( [[ s2 ]] = [[ forall ias . s1 ]] = [[ forall ias . ne ]] \).
By applying Lemma~\ref{lem:partial_skol}, we get \( [[ G , as |-E ee <= ne ~> ef3 ]] \) where \( [[ ef2' =ctx ef3 ]] \).
The goal now follows by Lemma~\ref{lem:mode_pres_dyn} (after environment weakening, where \( [[ s ]] = [[ r ]] = [[ ne ]] \) ), and Lemma~\ref{lem:ctx_equiv_trans}.

\subcase{\( [[ ps ]] \neq [[ empty ]] \) : }
By case analysis on the pattern checking derivation (\rref{Pat-CheckInfForall}), we know that \( [[ G , as |-P ps <= s1 => s2 ; Del' ~> fps2 : fpsigs2']] \) where \( [[ Del ]] = [[ as , Del' ]] \) and \( [[ fpsigs2 ]] = [[ @as , fpsigs2' ]] \).
By Lemma~\ref{lem:pat_inf_implies_check} (where we take \( [[ s ]] = [[ s1 ]] \)), we know that \( [[ type ( psigs ; s2 ~ s1 ) ]] \).
This thus means that \( [[ s2 ]] = [[ ne ]] \).
By Lemma~\ref{lem:pat_mode_pres}, the goal reduces to \( [[ case fps1 : fpsigs1 -> ef1' =ctx case fps1 : fpsigs1 -> ef2' ]] \). Applying Lemma~\ref{lem:compat_case} reduces this goal further to \( [[ ef1' =ctx ef2' ]] \).
This follows directly from Lemma~\ref{lem:mode_pres_dyn} (where \( [[ s ]] = [[ r ]] = [[ ne ]] \) ).

\case{\rref{Decl-NoAnnMulti} : }

We know from the premise of the first derivation that \( \forall i : [[ G |-P psi => psigs ; Deli ~> fpsi : fpsigs ]] \), \( [[ G , Deli |-E eei => nei ~> efi ]] \) and \( [[ G , Deli |- nei inst _ d r' ~> ewfi ]] \).
Furthermore, \( [[ ef1 ]] = [[ case </ fpsi : fpsigs -> ewfi [ efi ] // i /> ]] \), \( [[ type ( psigs ; r' ~ s' ) ]] \) and \( [[ s ]] = [[ forall ias . s' ]] \) where \( [[ as = fv ( s' ) \ dom ( G ) ]] \).
By case analysis on the second derivation (\rref{Decl-Ann}), we know that \( \forall i : [[ G |-P psi <= forall ias . s' => si ; Deli ~> fpsi' : fpsigs' ]] \), \( [[ G , Deli |-E eei <= si ~> efi' ]] \) and \( [[ ef2 ]] = [[ case </ fpsi' : fpsigs' -> efi' // i /> ]] \).

We again perform case analysis on the patterns \( [[ ps ]] \):

\subcase{\( [[ ps ]] = [[ empty ]] \) : }
Similarly to last time, we know that \( [[ s' ]] = [[ r' ]] \) and \( \forall i : [[ si ]] = [[ forall ias . r' ]] \).
We know by Lemma~\ref{lem:partial_skol} that \( \forall i : [[ G , as |-E eei <= r' ~> efi'' ]] \) where \( [[ efi' =ctx efi'' ]] \).
The goal now follows by Lemma~\ref{lem:mode_pres_dyn} (where we take \( [[ s ]] = [[ r ]] = [[ r' ]] \) ) and Lemma~\ref{lem:ctx_equiv_trans}.

\subcase{\( [[ ps ]] \neq [[ empty ]] \) : }
Similarly to the previous case, we can derive that \( \forall i : [[ G , as |-P ps <= s' => si ; Deli' ~> fpsi' : fpsigs'' ]] \) where \( [[ Deli ]] = [[ as , Deli' ]] \) and \( [[ fpsigs' ]] = [[ @as , fpsigs'' ]] \).
We again derive by Lemma~\ref{lem:pat_inf_implies_check} that \( [[ type ( psigs ; si ~ s' ) ]] \) and thus that \( [[ si ]] = [[ r' ]] \).
By Lemma~\ref{lem:pat_mode_pres}, the goal reduces to \( [[ case </ fpsi : fpsigs -> ewfi [ efi ] // i /> =ctx case </ fpsi : fpsigs -> efi' // i /> ]] \).
We reduce this goal further by applying Lemma~\ref{lem:compat_case} to \( \forall i : [[ ewfi [ efi ] =ctx efi' ]] \).
This follows directly from Lemma~\ref{lem:mode_pres_dyn} (where \( [[ s ]] = [[ r ]] = [[ r' ]] \) ).

Note however, that as Lemma~\ref{lem:mode_pres_dyn} only holds under shallow instantiation, that the same holds true for Property~\ref{prop:signature_dyn}.
\qed

% ---------- %
% PROPERTY 7 %
% ---------- %
\renewcommand\elab[1]{#1}
\newtheorem*{prop:type_sig}{Property \ref{prop:type_sig}}
\begin{prop:type_sig}[Type Signatures are Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G |-E x : s1 ; </ x psi = eei // i /> => G1 ~> x : s1 = ef1 ]]~\text{and}~[[ G |-E x : s2 ; </ x psi = eei // i /> => G1 ~> x : s2 = ef2 ]] \)
  \( \text{where}~[[ G |- s1 inst _ d r ~> ewf1 ]]~\text{and}~[[ G |- s2 inst _ d r ~> ewf2 ]]~\text{then}~[[ ewf1 [ ef1 ] =ctx ewf2 [ ef2 ] ]] \)
\end{prop:type_sig}
We start by introducing a number of helper lemmas:

\begin{lemma}[Substitution in Expressions is Type Preserving (Synthesis)]\ \\
  \( \text{If}~[[ G , a |-E ee => ne ~> ef ]]~\text{then}~[[ G |-E [ t / a ] ee => [ t / a ] ne ~> [ t / a ] ef ]] \)
  \label{lem:exp_subst_type_synth}
\end{lemma}
\begin{lemma}[Substitution in Expressions is Type Preserving (Checking)]\ \\
  \( \text{If}~[[ G , a |-E ee <= s ~> ef ]]~\text{then}~[[ G |-E [ t / a ] ee <= [ t / a ] s ~> [ t / a ] ef ]] \)
  \label{lem:exp_subst_type_check}
\end{lemma}
\begin{lemma}[Substitution in Heads is Type Preserving]\ \\
  \( \text{If}~[[ G , a |-H h => s ~> ef ]]~\text{then}~[[ G |-H [ t / a ] h => [ t / a ] s ~> [ t / a ] ef ]] \)
  \label{lem:head_subst_type}
\end{lemma}
\begin{lemma}[Substitution in Arguments is Type Preserving]\ \\
  \( \text{If}~[[ G , a |-A args <= s => s' ~> fargs ]]~\text{then}~[[ G |-A [ t / a ] args <= [t / a ] s => [ t / a ] s' ~> [ t / a ] fargs ]] \)
  \label{lem:arg_subst_type}
\end{lemma}
\begin{lemma}[Substitution in Declarations is Type Preserving]\ \\
  \( \text{If}~[[ G , a |-E edecl => G , a , x : s ~> x : s = ef ]]~\text{then}~[[ G |-E [ t / a ] edecl => G , x : [ t / a ] s ~> x : s = [ t / a ] ef ]] \)
  \label{lem:decl_subst_type}
\end{lemma}
The proof proceeds by mutual induction on the typing derivation. While the number of cases gets pretty large, each is quite straightforward.

\begin{lemma}[Type Instantiation Produces Equivalent Expressions (Synthesis)]\ \\
  \( \text{If}~[[ G1 |-E ee => ne1 ~> ef1 ]],~[[ G2 |-E ee => ne2 ~> ef2 ]]~\text{and}~\exists~[[ as ]] \subseteq [[ fv ( ne1 ) ]] \cup [[ fv ( ne2 ) ]] \) \\
  \( \text{such that}~[[ G' ]] = [[ [ ts / as ] G1 ]] = [[ [ ts / as ] G2 ]]~\text{and}~[[ G' |- forall as . ne1 inst _ d r ~> ewf1 ]]~\text{and}~[[ G' |- forall as . ne2 inst _ d r ~> ewf2 ]] \) \\
  \( \text{then}~[[ ewf1 [ /\ as . ef1 ] =ctx ewf2 [ /\ as . ef2 ] ]] \)
  \label{lem:inst_dyn_inf}
\end{lemma}
\begin{lemma}[Type Instantiation Produces Equivalent Expressions (Checking)]\ \\
  \( \text{If}~[[ G1 |-E ee <= s1 ~> ef1 ]]~\text{and}~[[ G2 |-E ee <= s2 ~> ef2 ]]~\text{and}~\exists~[[ as ]] \subseteq [[ fv ( s1 ) ]] \cup [[ fv ( s2 ) ]] \) \\
  \( \text{such that}~[[ G' ]] = [[ [ ts / as ] G1 ]] = [[ [ ts / as ] G2 ]]~\text{and}~[[ G' |- forall as . s1 inst _ d r ~> ewf1 ]]~\text{and}~[[ G' |- forall as . s2 inst _ d r ~> ewf2 ]] \) \\
  \( \text{then}~[[ ewf1 [ /\ as . ef1 ] =ctx ewf2 [ /\ as . ef2 ] ]] \)
  \label{lem:inst_dyn_check}
\end{lemma}
\begin{lemma}[Type Instantiation Produces Equivalent Expressions (Head Judgement)]\ \\
  \( \text{If}~[[ G1 |-H h => s1 ~> ef1 ]],~[[ G2 |-H h => s2 ~> ef2 ]]~\text{and}~\exists~[[ as ]] \subseteq [[ fv ( ne1 ) ]] \cup [[ fv ( ne2 ) ]] \) \\
  \( \text{such that}~[[ G' ]] = [[ [ ts / as ] G1 ]] = [[ [ ts / as ] G2 ]]~\text{and}~[[ G' |- forall as . s1 inst _ d r ~> ewf1 ]]~\text{and}~[[ G' |- forall as . s2 inst _ d r ~> ewf2 ]] \) \\
  \( \text{then}~[[ ewf1 [ /\ as . ef1 ] =ctx ewf2 [ /\ as . ef2 ] ]] \)
  \label{lem:inst_dyn_head}
\end{lemma}
Note that we define \( [[ [ t / a ] G ]] \) as removing \( [[ a ]] \) from the environment \( [[ G ]] \) and substituting any occurrence of \( [[ a ]] \) in types bound to term variables.
Furthermore, we use \( [[ as1 ]] \cup [[ as2 ]] \) as a shorthand for list concatenation, removing duplicates.
The proof proceeds by induction on the first typing derivation.
Note that Lemmas~\ref{lem:inst_dyn_inf}, \ref{lem:inst_dyn_check} and~\ref{lem:inst_dyn_head} have to be proven using mutual induction. However, the proof for Lemma~\ref{lem:inst_dyn_head} is trivial, as every case besides \rref{H-Inf} is deterministic.
As usual, we will focus on the non-trivial cases:

\case{\rref{Tm-CheckAbs} \( [[ ee ]] = [[ \ x . ee' ]] \) : }

We know from the premise of the first and second (as the relation is syntax directed) typing derivation that \( [[ G1 |- s1 skolS _ S s4 -> s5 ; G1' ~> ewf1' ]] \), \( [[ G2 |- s2 skolS _ S s4' -> s5' ; G2' ~> ewf2' ]] \), \( [[ G1' , x : s4 |-E ee' <= s5 ~> ef3 ]] \) and \( [[ G2' , x : s4' |-E ee' <= s5' ~> ef4 ]] \),
where \( [[ ef1 ]] = [[ ewf1' [ \ x : s4 . ef3 ] ]] \) and \( [[ ef2 ]] = [[ ewf2' [ \ x : s4' . ef4 ] ]] \).

At this point, it is already clear that Lemma~\ref{lem:inst_dyn_check} can not hold under deep instantiation, as instantiation performs full eta expansion. We will thus focus on shallow instantiation from here on out.

By case analysis on the skolemisation and instantiation premises, it is clear that \( [[ G1' ]] = [[ G1 , as1 ]] \), \( [[ G2' ]] = [[ G2 , as2 ]] \) and \( [[ r ]] = [[ [ ts1 / as1 ] ( s4 -> s5) ]] = [[ [ ts2 / as2 ] ( s4' -> s5' ) ]] = [[ s3 -> s3' ]] \).
In order to apply the induction hypothesis, we take \([[ as' ]]\) as \([[ as ]] \cup [[ as1 ]] \cup [[ as2 ]] \).
Note that this does not alter the instantiation to \( [[ r ]] \) in any way, as these variables would already have been instantiated.
We apply the induction hypothesis with \( [[ G1 |- forall as' . s5 inst _ S s3' ~> ewf3 ]] \) and \( [[ G2 |- forall as' . s5' inst _ S s3' ~> ewf4 ]] \) (after weakening), producing \( [[ ewf3 [ /\ as' . ef3 ] =ctx ewf4 [ /\ as' . ef4 ] ]] \).
Under shallow instantiation, these two instantiations follow directly from the premise with \( [[ ewf3 ]] = [[ ewf1 ]] \) and \( [[ ewf4 ]] = [[ ewf2 ]] \).

The goal reduces to \( [[ ewf1 [ /\ as . ewf1' [ \ x : s4 . ef3 ] ] =ctx ewf2 [ /\ as . ewf2' [ \ x : s4' . ef4 ] ] ]] \).
By the definition of skolemisation, this further reduces to \( [[ ewf1 [ /\ as . /\ as1 . \ x : s4 . ef3 ] =ctx ewf2 [ /\ as . /\ as2 . \ x : s4' . ef4 ] ]] \).
Finally, the goal follows by the induction hypothesis and compatibility Lemmas~\ref{lem:compat_tyabs}, \ref{lem:compat_abs} and~\ref{lem:compat_wrapper}, along with transitivity Lemma~\ref{lem:ctx_equiv_trans}.

\case{\rref{Tm-CheckTyAbs} \( [[ ee ]] = [[ /\ a . ee' ]] \) : }

We know the premise of the typing derivation that \( [[ s1 = forall ias1 . forall a . s1' ]] \), \( [[ s2 = forall ias . forall a . s2' ]] \), \( [[ G1 , as1 , a |-E ee' <= s1' ~> ef1' ]] \), \( [[ G2 , as2 , a |-E ee' <= s2' ~> ef2' ]] \), \( [[ ef1 ]] = [[ /\ as1 . /\ a . ef1' ]] \) and \( [[ ef2 ]] = [[ /\ as2 . /\ a . ef2' ]] \).
By case analysis on the type instantiation (\rref{InstT-SForall} and~\rref{InstT-SInfForall}), we get \( [[ G' |- [ ts1 / as ] [ ts1' / as1 ] [ t1 / a ] s1' inst _ S r ~> ewf1' ]] \) and \( [[ G' |- [ ts2 / as ] [ ts2' / as2 ] [ t2 / a ] s2' inst _ S r ~> ewf2' ]] \) where \( [[ ewf1 ]] = [[ \ ef . ( ewf1' [ ef ts1 ts1' t1 ] ) ]] \) and \( [[ ewf2 ]] = [[ \ ef . ( ewf2' [ ef ts2 ts2' t2 ] ) ]] \).

The goal to be proven is \( [[ ewf1 [ /\ as . /\ as1 . /\ a . ef1' ] =ctx ewf2 [ /\ as . /\ as2 . /\ a . ef2' ] ]] \).
This reduces to \( [[ ewf1' [ ( /\ as . /\ as1 . /\ a . ef1' ) ts1 ts1' t1 ] =ctx ewf2' [ ( /\ as . /\ as2 . /\ a . ef2' ) ts2 ts2' t2 ] ]] \).

We now define a substitution \( [[ theta ]] = [[ [ ts1 / as ] . [ ts2 / as ] . [ ts1' / as1 ] . [ ts2' / as2 ] . [ t1 / a ] . [ t2 / a ] ]] \). From the instantiation relation (and the fact that both types instantiate to the same type \( [[r]] \), we conclude that if \( [[ [ ti / a ] ]] \in [[ theta ]] \) and \( [[ [ tj / a ] ]] \in [[ theta ]] \) that \( [[ ti ]] = [[ tj ]] \).
By applying Lemma~\ref{lem:exp_subst_type_check}, we transform the premise to \( [[ [ ts1 / as ] G1 |-E theta ee' <= theta s1' ~> theta ef1' ]] \) and \( [[ [ ts2 / as ] G2 |-E theta ee' <= theta s2' ~> theta ef2' ]] \).

By applying the induction hypothesis, we get that \( [[ ewf1' [ theta ef1' ] =ctx ewf2' [ theta ef2' ] ]] \). The goal follows directly from the definition of \( [[ theta ]] \).

\case{\rref{Tm-CheckInf} : }

We know from the premise of the typing derivation that \( [[ G1 |- s1 skol _ d r1 ; G1' ~> ewf1' ]] \), \( [[ G2 |- s2 skol _ d r2 ; G2' ~> ewf2' ]] \), \( [[ G1' |-E ee => ne1 ~> ef1' ]] \), \( [[ G2' |-E ee => ne2 ~> ef2' ]] \), \( [[ G1' |- ne1 inst _ d r1 ~> ewf1'' ]] \), \( [[ G2' |- ne2 inst _ d r2 ~> ewf2'' ]] \), \( [[ ef1 ]] = [[ ewf1' [ ewf1'' [ ef1' ] ] ]] \) and \( [[ ef2 ]] = [[ ewf2'' [ ewf2' [ ef2' ] ] ]] \).
The goal to be proven is thus \( [[ ewf1 [ /\ as . ewf1' [ ewf1'' [ ef1' ] ] ] =ctx  ewf2 [ /\ as . ewf2' [ ewf2'' [ ef2' ] ] ] ]] \).

From the definition of shallow skolemisation, we know that \( [[ G1' ]] = [[ G1 , as1 ]] \), \( [[ G2' ]] = [[ G2 , as2 ]] \), \( [[ ewf1' ]] = [[ \ ef . /\ as1 . ef ]] \) and \( [[ ewf2' ]] = [[ \ ef . /\ as2 . ef ]] \).
We now take \( [[ as' ]] = [[ as ]] \cup [[ as1 ]] \cup [[ as2 ]] \).
As \( [[ s1 ]] \) and \( [[ s2 ]] \) instantiate to the same type \( [[ r ]] \), it is not hard to see from the definition of skolemisation that \( [[ G1' |- forall as' . ne1 inst _ S r ~> ewf3 ]] \) and \( [[ G2' |- forall as' . ne2 inst _ S r ~> ewf4 ]] \).
By applying Lemma~\ref{lem:inst_dyn_inf}, we thus get \( [[ ewf3 [ /\ as' . ef1' ] =ctx ewf4 [ /\ as' . ef2' ] ]] \).
The goal follows through careful examination of the skolemisation and instantiation premises.
\qed

\begin{lemma}[Pattern Checking Implies Synthesis]\ \\
  \( \text{If}~[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]~\text{then}~\exists [[ psigs ]] : [[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]~\text{where}~[[ type ( psigs ; s' ~ s ) ]] \)
  \label{lem:pat_check_implies_inf}
\end{lemma}
The proof follows by straightforward induction on the pattern typing derivation.

We now go back to proving Property~\ref{prop:type_sig}, and proceed by case analysis on both typing derivations (\rref{Decl-Ann}).
We know from the premise that \( [[ G |-P psi <= s1 => si1 ; Deli1 ~> fpsi : fpsigs1 ]] \), \( [[ G |-P psi <= s2 => si2 ; Deli2 ~> fpsi : fpsigs2 ]] \), \( [[ G , Deli1 |-E eei <= si1 ~> efi1 ]] \), \( [[ G , Deli2 |-E eei <= si2 ~> efi2 ]] \), \( [[ ef1 ]] = [[ case </ fpsi : fpsigs1 -> efi1 // i /> ]] \) and \( [[ ef2 ]] = [[ case </ fpsi : fpsigs2 -> efi2 // i /> ]] \).
The goal to be proven is \( [[ ewf1 [ case </ fpsi : fpsigs1 -> efi1 // i /> ] =ctx ewf2 [ case </ fpsi : fpsigs2 -> efi2 // i /> ] ]] \). Lemma~\ref{lem:compat_case} reduces this to \( \forall i : [[ ewf1 [ efi1 ] =ctx ewf2 [ efi2 ] ]] \).

We take \( [[ asi ]] = [[ dom ( Deli1 ) ]] \cup [[ dom ( Deli2 ) \ dom ( G ) ]] \), and apply weakening to get \( [[ G , asi |-E eei <= si1 ~> efi1 ]] \) and \( [[ G , asi |-E eei <= si2 ~> efi2 ]] \).
The goal now follows directly from Lemma~\ref{lem:inst_dyn_check} with \( [[ asi ]] = [[ empty ]] \), if we can show that \( [[ G , asi |- si1 inst _ S r' ~> ewf1 ]] \) and \( [[ G , asi |- si2 inst _ S r' ~> ewf2 ]] \) for some \( [[r']] \) (Note that Lemma~\ref{lem:inst_dyn_check} only holds under shallow instantiation).

We know from Lemma~\ref{lem:pat_check_implies_inf} that \( \exists [[ fpsigs ]] : [[ G |-P psi => psigs ; Deli ~> fpsi : fpsigs ]] \) such that \( [[ type ( psigs ; si1 ~ s1 ) ]] \) and \( [[ type ( psigs ; si2 ~ s2 ) ]] \).
The remaining goal follows from the definition of the type relation, and shallow instantiation.
\qed

\subsection{Pattern Inlining and Extraction}
\label{app:prop8}
% ---------- %
% PROPERTY 8 %
% ---------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:pat_inlining_typ}{Property \ref{prop:pat_inlining_typ}}
\begin{prop:pat_inlining_typ}[Pattern Inlining is Type Preserving]\ \\
  \( \text{If}~[[ G |-E x ps = ee1 => G' ~> x : s = ef1 ]]~\text{and}~[[ wrap ( ps ; ee1 ~ ee2 ) ]]~\text{then}~[[ G |-E x = ee2 => G' ~> x : s = ef2 ]] \)
\end{prop:pat_inlining_typ}
We first introduce a helper lemma to prove pattern inlining in expressions preserves the type:

\begin{lemma}[Pattern Inlining in Expressions is Type Preserving (Synthesis)]\ \\
  \( \text{If}~[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]~\text{and}~[[ G , Del |-E ee1 => ne1 ~> ef1 ]]~\text{where}~[[ wrap ( ps ; ee1 ~ ee2 ) ]] \) \\
  \( \text{then}~[[ G |-E ee2 => ne2 ~> ef2 ]]~\text{and}~[[ type ( psigs ; ne1 ~ ne2 ) ]] \)
  \label{lem:pat_inlining_typ_inf}
\end{lemma}
The proof proceeds by induction on the pattern typing derivation. We will focus on the non-trivial cases below. Note that the \rref{Pat-InfCon} is an impossible case as \( [[ wrap ( K ps ; ee1 ~ ee2 ) ]] \) is undefined.

\case{\rref{Pat-InfVar} \( [[ ps ]] = [[ x , ps' ]] \), \( [[ psigs ]] = [[ t1 , psigs' ]] \) and \( [[ Del ]] = [[ x : t1 , Del' ]] \) : }

We know from the rule premise that \( [[ G , x : t1 |-P ps' => psigs' ; Del' ~> fps' : fpsigs' ]] \).
Furthermore, by inlining the definitions of \( [[ Del ]] \) and \( [[ ps ]] \) in the lemma premise, we get \( [[ G , x : t1 , Del' |-E ee1 => ne1 ~> ef1 ]] \) and \( [[ wrap ( x , ps' ; ee1 ~ \ x . ee2' ) ]] \) and thus (by \rref{PatWrap-Var}) \( [[ wrap ( ps' ; ee1 ~ ee2' ) ]] \).
By the induction hypothesis, we get \( [[ G , x : t1 |-E ee2' => ne3 ~> ef2' ]] \) and \( [[ type ( psigs' ; ne1 ~ ne3 ) ]] \).
The goal follows by \rref{Tm-InfAbs} and \rref{Type-Var}.

\case{\rref{Pat-InfTyVar} \( [[ ps ]] = [[ @a , ps' ]] \), \( [[ psigs ]] = [[ @a , psigs' ]] \) and \( [[ Del ]] = [[ a , Del' ]] \) : }

We know from the rule premise that \( [[ G , a |-P ps' => psigs' ; Del' ~> fps' : fpsigs' ]] \).
Again, by inlining the definitions in the lemma premise, we get \( [[ G , a , Del' |-E ee1 => ne1 ~> ef1 ]] \) and \( [[ wrap ( @a , ps' ; ee1 ~ /\ a . ee2' ) ]] \) and thus (by \rref{PatWrap-TyVar}) \( [[ wrap ( ps' ; ee1 ~ ee2' ) ]] \).
By the induction hypothesis, we get \( [[ G , a |-E ee2' => ne3 ~> ef2' ]] \) and \( [[ type ( psigs' ; ne1 ~ ne3 ) ]] \).

The goal to be proven is \( [[ G |-E /\ a . ee2' => forall a . ne3 ~> ef2 ]] \) where \( [[ type ( @a , psigs' ; ne1 ~ forall a . ne3 ) ]] \) (follows by \rref{Type-TyVar}).
However, under eager instantiation, this goal can never hold as \rref{Tm-InfTyAbs} would instantiate the forall binder away. We can thus only prove this lemma under lazy instantiation, where the goal follows trivially from \rref{Tm-InfTyAbs}.
\qed

We now proceed with proving Property~\ref{prop:pat_inlining_typ}, through case analysis on the declaration typing relation (\rref{Decl-NoAnnSingle}).
We know from the premise of the first derivation that \( [[ G |-P ps => psigs ; Del ~> fps : fpsigs ]] \), \( [[ G , Del |-E ee1 => ne1 ~> ef1 ]] \), \( [[ type ( psigs ; ne1 ~ s ) ]] \) and \( [[ G' ]] = [[ G , x : forall ias . s ]] \) where \( [[ as = fv ( s ) \ dom ( G ) ]] \).
The goal to be proven thus becomes \( [[ G |-P empty => empty ; empty ~> empty : empty ]] \) (follows directly from \rref{Pat-InfEmpty}) and \( [[ G |-E ee2 => ne2 ~> ef2 ]] \) where \( [[ ne2 ]] = [[ s ]] \) (follows from Lemma~\ref{lem:pat_inlining_typ_inf}).
Note that as we require Lemma~\ref{lem:pat_inlining_typ_inf}, we can only prove Property~\ref{prop:pat_inlining_typ} under lazy instantiation.
\qed

% ----------- %
% PROPERTY 10 %
% ----------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:pat_extraction_typ}{Property \ref{prop:pat_extraction_typ}}
\begin{prop:pat_extraction_typ}[Pattern Extraction is Type Preserving]\ \\
  \( \text{If}~[[ G |-E x = ee2 => G' ~> x : s = ef2 ]]~\text{and}~[[ wrap ( ps ; ee1 ~ ee2 ) ]]~\text{then}~[[ G |-E x ps = ee1 => G' ~> x : s = ef1 ]] \)
\end{prop:pat_extraction_typ}

We first introduce another helper lemma to prove that pattern extraction from expressions preserves the typing:
\begin{lemma}[Pattern Extraction from Expressions is Type Preserving (Synthesis)]\ \\
  \( \text{If}~[[ G |-E ee2 => ne2 ~> ef2 ]]~\text{and}~\exists~[[ ee1 ]], [[ ps ]]~\text{such that}~[[ wrap ( ps ; ee1 ~ ee2 ) ]] \) \\
  \( \text{then}~[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]~\text{and}~[[ G , Del |-E ee1 => ne1 ~> ef1 ]]~\text{where}~[[ type ( psigs ; ne1 ~ ne2 ) ]] \)
  \label{lem:pat_extraction_typ_inf}
\end{lemma}
The proof proceeds by induction on the \([[ee2]]\) typing derivation. As usual, we will focus on the non-trivial cases:

\case{\rref{Tm-InfAbs} \( [[ ee2 ]] = [[ \ x . ee2' ]] \) and \( [[ ne2 ]] = [[ t2 -> ne3 ]] \) : }

We know from the rule premise that \( [[ G , x : t2 |-E ee2' => ne3 ~> ef2' ]] \).
It is clear by case analysis on \( [[ wrap ( ps ; ee1 ~ \ x . ee2' ) ]] \) that \( [[ ps ]] = [[ x , ps' ]] \) and \( [[ wrap ( ps' ; ee1 ~ ee2' ) ]] \).
By applying the induction hypothesis, we get \( [[ G , x : t2 |-P ps' => psigs' ; Del' ~> fps' : fpsigs' ]] \), \( [[ G , x : t2 , Del' |-E ee1 => ne1 ~> ef1 ]] \) and \( [[ type ( psigs' ; ne1 ~ ne3 ) ]] \).
The goal thus follows straightforwardly by \rref{Pat-InfVar} and \rref{Type-Var}.

\case{\rref{Tm-InfTyAbs} \( [[ ee2 ]] = [[ /\ a . ee2' ]] \) : }

We know from the rule premise that \( [[ G , a |-E ee2' => ne3 ~> ef2' ]] \) and \( [[ G |- forall a . ne3 inst _ d ne2 ~> ewf2 ]] \).
Furthermore, it is clear by case analysis on \( [[ wrap ( ps ; ee1 ~ /\ a . ee2' ) ]] \) that \( [[ ps ]] = [[ @a , ps' ]] \) and \( [[ wrap ( ps' ; ee1 ~ ee2' ) ]] \).
By the induction hypothesis, we get \( [[ G , a |-P ps' => psigs' ; Del' ~> fps' : fpsigs' ]] \), \( [[ G , a , Del' |-E ee1 => ne1 ~> ef1 ]] \) and \( [[ type ( psigs' ; ne1 ~ ne3 ) ]] \).

The goal to be proven is \( [[ G |-P @a , ps' => @a , psigs' ; a , Del' ~> fps : fpsigs ]] \) (follows by \rref{Pat-InfTyVar}), \( [[ G , a , Del' |-E ee1 => ne1 ~> ef1 ]] \) (follows by the induction hypothesis) and \( [[ type ( @a , psigs' ; ne1 ~ ne2 ) ]] \).
However, it is clear that this final goal does not hold under eager instantiation, as \rref{Tm-InfTyAbs} instantiates the forall binder away. Under lazy instantiation, the remaining goal follows directly from the premise.

\case{\rref{Tm-InfApp} \( [[ ee2 ]] = [[ h args ]] \) and \( [[ args ]] = [[ empty ]] \) and \( [[ h ]] = [[ ee ]] \) : }

The goal follows directly by the induction hypothesis.

\case{\rref{Tm-InfApp} \( [[ ee2 ]] = [[ h args ]] \) and \( [[ args ]] \neq [[ empty ]] \) or \( [[ h ]] \neq [[ ee ]] \) : }

It is clear from the definition of \( [[ wrap ( ps ; ee1 ~ h args ) ]] \) that \( [[ ps ]] = [[ empty ]] \). The goal thus follows trivially.
\qed

We now return to prove Property~\ref{prop:pat_extraction_typ} by case analysis on the declaration typing derivation (\rref{Decl-NoAnnSingle}).
We know from the derivation premise that \( [[ G |-E ee2 => ne2 ~> ef2 ]] \) and \( [[ s = forall ias . ne2 ]] \) where \( [[ as = fv ( ne2 ) \ dom ( G ) ]] \).
The goal follows directly from Lemma~\ref{lem:pat_extraction_typ_inf}.
Note that as Lemma~\ref{lem:pat_extraction_typ_inf} only holds under lazy instantiation, the same holds true for Property~\ref{prop:pat_extraction_typ}.
\qed

% ---------- %
% PROPERTY 9 %
% ---------- %
\renewcommand\elab[1]{#1}
\newtheorem*{prop:pat_inlining_dyn}{Property \ref{prop:pat_inlining_dyn}}
\begin{prop:pat_inlining_dyn}[Pattern Inlining / Extraction is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G |-E x ps = ee1 => G' ~> x : s = ef1 ]],~[[ wrap ( ps ; ee1 ~ ee2 ) ]],~\text{and}~[[ G |-E x = ee2 => G' ~> x : s = ef2 ]]~\text{then}~[[ ef1 =ctx ef2 ]] \)
\end{prop:pat_inlining_dyn}
We start by introducing a helper lemma, proving pattern inlining preserves the runtime semantics for expressions.

\begin{lemma}[Pattern Inlining in Expressions is Runtime Semantics Preserving]\ \\
  \( \text{If}~[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]~\text{and}~[[ G , Del |-E ee1 => ne1 ~> ef1 ]]~\text{and}~[[ G |-E ee2 => ne2 ~> ef2 ]]~\text{where}~[[ wrap ( ps ; ee1 ~ ee2 ) ]] \) \\
  \( \text{then}~[[ case fps :fpsigs -> ef1 =ctx ef2 ]] \)
  \label{lem:pat_inlining_dyn_inf}
\end{lemma}
The proof proceeds by induction on the pattern typing derivation. We will focus on the non-trivial cases. Note that, as \( [[ wrap ( K ps ; ee1 ~ ee2 ) ]] \) is undefined, \rref{Pat-InfCon} is an impossible case.

\case{\rref{Pat-InfVar} \( [[ ps ]] = [[ x , ps' ]] \), \( [[ psigs ]] = [[ t1 , psigs' ]] \) , \( [[ Del ]] = [[ x : t1 , Del' ]] \), \( [[ fps ]] = [[ x : t1 , fps' ]] \) and \( [[ fpsigs ]] = [[ t1 , fpsigs' ]] \) : }

We know from the pattern typing derivation premise that \( [[ G , x : t1 |-P ps' => psigs' ; Del' ~> fps' : fpsigs' ]] \).
By inlining the definitions and \rref{PatWrap-Var}, we get \( [[ ee2 ]] = [[ \ x . ee2' ]] \) and \( [[ wrap ( ps' ; ee1 ~ ee2' ) ]] \).
By case analysis on the \( [[ ee2 ]] \) typing derivation (\rref{Tm-InfAbs}), we know \( [[ G , x : t1 |-E ee2' => ne3 ~> ef2' ]] \) where \( [[ ne2 ]] = [[ t1 -> ne3 ]] \) and \( [[ ef2 ]] = [[ \ x : t1 . ef2' ]] \).
By applying the induction hypothesis, we get \( [[ case fps' : fpsigs' -> ef1 =ctx ef2' ]] \).
The goal to be proven is \( [[ \ x : t1 . case fps' : fpsigs' -> ef1 = \ x : t1 . ef2' ]] \), and follows directly from Lemma~\ref{lem:compat_abs}.

\case{\rref{Pat-InfTyVar} \( [[ ps ]] = [[ @a , ps' ]] \), \( [[ psigs ]] = [[ @a , psigs' ]] \) , \( [[ Del ]] = [[ a , Del' ]] \), \( [[ fps ]] = [[ @a , fps' ]] \) and \( [[ fpsigs ]] = [[ @a , fpsigs' ]] \) : }

We know from the pattern typing derivation premise that \( [[ G , a |-P ps' => psigs' ; Del' ~> fps' : fpsigs' ]] \).
Similarly to the previous case, by inlining and \rref{PatWrap-TyVar}, we get \( [[ ee2 ]] = [[ /\ a . ee2' ]] \) and \( [[ wrap ( ps' ; ee1 ~ ee2' ) ]] \).
By case analysis on the \( [[ ee2 ]] \) typing derivation (\rref{Tm-InfTyAbs}), we get \( [[ G , a |-E ee2' => ne3 ~> ef2' ]] \), \( [[ G |- forall a . ne3 inst _ d ne2 ~> ewf ]] \) and \( [[ ef2 ]] = [[ ewf [ /\ a . ef2' ] ]] \).
Applying the induction hypothesis tells us that \( [[ case fps' : fpsigs' -> ef1 =ctx ef2' ]] \).

The goal to be proven is \( [[ /\ a . case fps' : fpsigs' -> ef1 =ctx ewf [ /\ a . ef2' ] ]] \).
By applying Lemma~\ref{lem:compat_tyabs} to the result of the induction hypothesis, we get \( [[ /\ a . case fps' :fpsigs' -> ef1 =ctx /\ a . ef2' ]] \).
Under lazy instantiation, the goal follows directly from this result, as \( [[ ewf ]] = [[ [] ]] \).
Under eager deep instantiation, it is clear that the goal does not hold, as \( [[ ewf ]] \) might perform eta expansion, thus altering the runtime semantics.
Under eager shallow instantiation, the goal follows straightforwardly, as \( [[ ewf ]] \) can only perform type applications. Note that this implies that \( [[ /\ a . case fps' : fpsigs' -> ef1 ]] \) and \( [[ ewf [ /\ a . ef2' ] ]] \) could thus have different types, but can always instantiate to the same type.
\qed

We now return to proving Property~\ref{prop:pat_inlining_dyn}, by case analysis on the first declaration typing relation (\rref{Decl-NoAnnSingle}).
We know from the derivation premise that \( [[ G |-P ps => psigs ; Del ~> fps : fpsigs ]] \), \( [[ G , Del |-E ee1 => ne1 ~> ef1' ]] \), \( [[ ef1 = case fps : fpsigs -> ef1' ]] \), \( [[ type ( psigs ; ne1 ~ s' ) ]] \), \( [[ s ]] = [[ forall ias . s' ]] \) where \( [[ as = fv ( s' ) \ dom ( G ) ]] \).
The premise of the second declaration typing derivations tells us that \( [[ G |-E ee2 => ne2 ~> ef2 ]] \).
The goal now follows directly from Lemma~\ref{lem:pat_inlining_dyn_inf}. Note that as Lemma~\ref{lem:pat_inlining_dyn_inf} does not hold under eager deep instantiation, the same is true for Property~\ref{prop:pat_inlining_dyn}.
\qed

\subsection{Single vs.~Multiple Equations}
\label{app:prop11}
% ----------- %
% PROPERTY 11 %
% ----------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:single_multi}{Property \ref{prop:single_multi}}
\begin{prop:single_multi}[Single/multiple Equations is Type Preserving]\ \\
  \( \text{If}~[[ G |-E x ps = ee => G , x : s ~> x : s = ef ]]~\text{then}~[[ G |-E x ps = ee, x ps = ee => G' ~> x : s = ef]] \)
\end{prop:single_multi}
The proof proceeds by case analysis on the declaration typing derivation (\rref{Decl-NoAnnSingle}).
From the derivation premise, we get \( [[ G |-P ps => psigs ; Del ~> fps : fpsigs ]] \), \( [[ G , Del |-E ee => ne ~> ef' ]] \), \( [[ type ( psigs ; ne ~ s1 ) ]] \) and \( [[ s ]] = [[ forall ias1 . s1 ]] \) where \( [[ as1 = fv ( s1 ) \ dom ( G ) ]] \).
The goal to be proven thus reduces to \( [[ G , Del |- ne inst _ d r ~> ewf ]] \), \( [[ type ( psigs ; r ~ s2 ) ]] \) and \( [[ s ]] = [[ forall ias2 . s2 ]] \) where \( [[ as2 = fv ( s2 ) \ dom ( G ) ]] \).
It is clear that the property can not hold under lazy instantiation, as \rref{Decl-NoAnnMulti} performs an additional instantiation step, thus altering the type.
Under eager instantiation, \( [[ ne ]] \) is already an instantiated type by the type inference relation, making the instantiation in the goal a no-op (by definition).
The goal is thus trivially true.
\qed

\subsection{$\eta$-expansion}
\label{app:prop12}
% ----------- %
% PROPERTY 12 %
% ----------- %
\renewcommand\elab[1]{}
\newtheorem*{prop:eta_restr}{Property \ref{prop:eta_restr}}
\begin{prop:eta_restr}[$\eta$-expansion is Type Preserving]\ 
\begin{shortItemize}
\item  \( \text{If}~[[ G |-E ee => ne ~> ef]]~\text{where}~\mathit{numargs}([[ne]]) = n ~\text{and}~[[ G |- ne inst _ d t ~> ewf ]]~\text{then}~[[ G |-E \ xsn . ee xsn => ne ~> ef]] \)
\item  \( \text{If}~[[ G |-E ee <= s ~> ef]]~\text{where}~\mathit{numargs}([[r]]) = n ~\text{then}~[[ G |-E \ xsn . ee xsn <= s ~> ef]] \)
\end{shortItemize}
\end{prop:eta_restr}
A formal definition of $\mathit{numargs}$ is shown in Figure~\ref{fig:numargs}.
We prove Property~\ref{prop:eta_restr} by first introducing a slightly more general lemma:

\begin{figure}
  \input{tex/figures/Numargs.mng}
  \caption{Counting Explicit Arguments}
  \label{fig:numargs}
\end{figure}

\begin{lemma}[$\eta$-expansion is Type Preserving - Generalised]\ 
\begin{shortItemize}
\item  \( \text{If}~[[ G |-E ee => ne ~> ef]]~\text{where}~0 \leq n \leq \mathit{numargs}([[ne]])~\text{and}~[[ G |- ne inst _ d t ~> ewf ]]~\text{then}~[[ G |-E \ xsn . ee xsn => ne ~> ef]] \)
\item  \( \text{If}~[[ G |-E ee <= s ~> ef]]~\text{where}~0 \leq n \leq \mathit{numargs}([[r]])~\text{then}~[[ G |-E \ xsn . ee xsn <= s ~> ef]] \)
  \label{lem:eta_gen}
\end{shortItemize}
\end{lemma}
The proof proceeds by induction on the integer \(n\).

\case{\( n = 0 \) : }

This case is trivial, as it follows directly from the premise.

\case{\( n = m + 1 \leq \mathit{numargs}([[ne]]) \) : }

\subcase{synthesis mode : }
We know from the induction hypothesis that \( [[ G |-E \ xsm . ee xsm => ne ~> ef ]] \).
We perform case analysis on this result (\(m\) repeated applications of \rref{Tm-InfAbs}) to get \( [[ G , </ xi : ti // i IN m /> |-E ee xsm => ne1 ~> ef' ]] \) where \( [[ ne ]] = [[ </ ti // i IN m /> -> ne1 ]] \).
Performing case analysis again on this result (\rref{Tm-InfApp}), gives us \( [[ G , </ xi : ti // i IN m /> |-H ee => s1 ~> ef1 ]] \), \( [[ G , </ xi : ti // i IN m /> |-A xsm <= s1 => s2 ~> fargs ]] \) and \( [[ G , </ xi : ti // i IN m /> |- s2 inst _ d ne1 ~> ewf ]] \).

The goal to be proven is \( [[ G |-E \ xsmplus . ee xsmplus => ne ~> ef ]] \), which (by \rref{TmInfAbs}) reduces to \( [[ G , </ xi : ti // i IN m /> , x : t |-E ee xsmplus => ne2 ~> ef' ]] \), where \( [[ ne ]] = [[ </ ti // i IN m /> -> t -> ne2 ]] \).

Note that this requires proving that \( [[ ne1 ]] = [[ t -> ne2 ]] \). While we know that \( m < \mathit{numargs}([[ne]]) \), we can only prove this under eager deep instantiation. Under lazy instantiation, type inference does not instantiate the result type at all. Under eager shallow, it is instantiated, but only up to the first function type.
From here on out, we will thus assume eager deep instantiation.
Furthermore, note that as even deep instantiation does not instantiate argument types,
we need the additional premise that \([[ne]]\) instantiates into a monotype, in order to
prove this goal.

This result in turn (by \rref{Tm-InfApp}) reduces to \( [[ G , </ xi : ti // i IN m /> , x : t |-H ee => s1 ~> ef1 ]] \) (follows by weakening), \( [[ G , </ xi : ti // i IN m /> , x : t |-A x , xsm <= s1 => s3 ~> fargs ]] \) (follows by \rref{Arg-Inst}, \rref{Arg-App} and the fact that \( [[ ne1 ]] = [[ t -> ne2 ]] \) ) and \( [[ G , </ xi : ti // i IN m /> , x : t |- s3 inst _ d ne2 ~> ewf ]] \) (follows by the definition of instantiation).

\subcase{checking mode : }
We know from the induction hypothesis that \( [[ G |-E \ xsm . ee xsm <= s ~> ef ]] \).
The proof proceeds similarly to the synthesis mode case, by case analysis on this result (\rref{Tm-CheckAbs}).
One additional step is that \rref{Tm-CheckInf} is applied to type \( [[ ee xsm ]] \).
The derivation switches to synthesis mode at this point, and becomes completely identical to the previous case.
\qed

The proof for Property~\ref{prop:eta_restr} now follows directly by Lemma~\ref{lem:eta_gen}, by taking \( n = \mathit{numargs}([[ ne ]]) \).
\qed


==> tex/sections/Haskell98.tex <==
%if style == newcode
\begin{code}
module Haskell98 where
\end{code}
%endif

% no elaboration here
\renewcommand\elab[1]{}
% no explicit type application here
\renewcommand\invisTyApp[1]{}

\section{The Implicit Polymorphic $\lambda$-Calculus}
\label{sec:first-system}
\label{sec:haskell98}

\begin{figure}
  \input{tex/figures/SimpleSyntax.mng}
  \caption{Implicit Polymorphic $\lambda$-Calculus (IPLC) Syntax}
  \label{fig:Ssyn}
\end{figure}

In order to assess our design choices against the transformations we desire
to ensure stability, this section and the next develop detailed calculi
to model our language. We start with a simpler calculus in this section:
a polymorphic, stratified $\lambda$-calculus with implicit polymorphism (only).
We call it the Implicit Polymorphic $\lambda$-calculus, or IPLC.
By ``implicit'', we mean that terms cannot explicitly instantiate or bind
types. However, type signatures are allowed in the calculus, and
the bidirectional type system~\cite{local-type-inference}
 permits higher-rank~\cite{odersky-laufer} functions. Some other features,
such as local $[[let]]$ declarations defining functions with multiple equations,
are added to bring this closer to our real-world application of Haskell.

We have built this system to support flexibility in both of our
axes of instantiation scheme design. That is, the calculus is parameterised
over choices of instantiation depth and eagerness. In this way, our
calculus is essentially a \emph{family} of type systems: choose your
design, and you can instantiate our rules accordingly.

The syntax for IPLC is shown in Figure~\ref{fig:Ssyn}.
We define two meta parameters $[[d]]$ and $[[ep]]$ denoting the depth and
eagerness of instantiation respectively. In the remainder of this paper, grammar
and relations which are affected by one of these parameters will be annotated as
such. A good example of this are types $[[qd]]$ and $[[ne]]$, as
explained below. 

\renewcommand\elab[1]{}
Keeping all the moving pieces straight can be challenging. We thus offer
some mnemonics to help the reader:
In the remainder of the paper, aspects pertaining to
\textbf{e}ager instantiation are highlighted in \instE{\textbf{e}merald}, while 
\textbf{l}azy features are highlighted in \instL{\textbf{l}avender}.
Similarly, instantiation under the \textbf{s}hallow scheme is drawn using a
\textbf{s}triped line, as in $[[ G |- s instS _ S r ~> ewf ]]$.

\paragraph{Types}
Our presentation of the IPLC contains several different type categories,
which we explain here. These categories are introduced to support
the different instantiation schemes discussed in this paper, altering the
behaviour of the typing rules accordingly.
Monotypes $[[t]]$ represent simple ground types without any polymorphism. They
are entirely standard, incorporating type variables $[[a]]$,
functions $[[t1 -> t2]]$ and saturated type constructors $[[T ts]]$\footnote{We
work only with saturated type constructors, as we wish to avoid complications
arising from a kind system. Such concerns would be orthogonal to our main object
of study: instantiation.}.
On the other side of the spectrum are type schemes $[[s]]$, which can be fully
polymorphic, with forall binders on the top-level, and nested on both sides of
the function arrow.

So far, none of these definitions depend on the instantiation flavour. This
changes with instantiated types $[[r]]$.
These types cannot have any top-level polymorphism, as their quantified type
variables have already been instantiated.
However, depending on whether instantiation happens shallowly
or deeply, they may or may not feature nested foralls on the right
of function arrows. This dependency on the depth $[[d]]$ of type
instantiation is denoted using an instantiated result type $[[qd]]$
on the right of the function
arrow. This type becomes a full type scheme $[[s]]$ under shallow
instantiation ($[[S]]$)---thus allowing foralls on the right of the function
arrow---and
becomes an instantiated type $[[r]]$ under deep instantiation ($[[D]]$)---thus
disallowing foralls on the right of the function arrow.
No matter the instantiation flavour,
function arguments within an instantiated type $[[r]]$
can still be polymorphic, as instantiating a function does not
affect polymorphism to the left of an arrow.
We also have synthesised types $[[ne]]$ to denote the output of the type synthesis
judgement $[[G |- e => ne ~> ef]]$, which infers a type from an expression. This
type depends on the eagerness $[[ep]]$ of type instantiation: under lazy
instantiation ($[[L]]$) inference can produce full type schemes $[[s]]$, but
under eager instantiation ($[[E]]$) synthesised types $[[ne]]$ must be instantiated types $[[r]]$:
any top-level quantified variable would have been instantiated away.

Finally, an argument descriptor $[[psig]]$ represents a type synthesised from
analysing a function argument pattern.
While this might not seem very useful in the IPLC (as they are just monotypes),
argument descriptors will be extended beyond regular types in the next section.
Descriptors are assembled
into type schemes $[[s]]$ with the $[[type (psigs; s0 ~ s ) ]]$ judgement,
in Figure~\ref{fig:STmb}.

\paragraph{Expressions}
Expressions $[[e]]$ are standard, except for $[[let]]$-expressions, which
are modelled on the syntax of Haskell.
These contain a single (non recursive) declaration
$[[decl]]$, which may optionally have a type signature $[[x : s]]$, followed by
the definition $[[</ x psi = ei // i />]]$. 
The patterns $[[ps]]$ on the left of the equals sign can each be either a simple
variable $[[x]]$ or a saturated data constructor $[[K ps]]$.

\paragraph{Contexts}
Typing contexts $[[G]]$ are entirely standard, storing both the term variables
$[[x]]$ with their types and the type variables $[[a]]$ in scope; these type
variables may not appear in the term (remember: this is an entirely \emph{implicit}
calculus), but they may be in scope in types. The type constructors and
data constructors are stored in a static context $[[Sig]]$, which
forms the basis of typing contexts $[[G]]$.
This static context contains the data type definitions by storing both type
constructors $[[T as]]$ and data constructors $[[K : as ; ss ; T]]$. Data
constructor types contain the list of quantified variables $[[as]]$, the argument
types $[[ss]]$, and the resulting type $[[T]]$; when $[[K : as ; ss ; T]]$, then
the use of $[[K]]$ in an expression would have type $[[forall as. ss -> T as]]$, abusing
syntax slightly to write a list of types $[[ss]]$ to the left of an arrow.

\subsection{Typing rules}
\label{sec:basic_typing}

\begin{figure}
  \input{tex/figures/SimpleTyping.mng}
  \caption{Term Typing for Implicit Polymorphic $\lambda$-Calculus}
  \label{fig:STm}
\end{figure}

\begin{figure}
  \input{tex/figures/SimpleTypingC.mng}
  \caption{Declaration Checking for Implicit Polymorphic $\lambda$-Calculus}
  \label{fig:STmc}
\end{figure}

\begin{figure}
  \input{tex/figures/SimpleTypingD.mng}
  \caption{Pattern Typing for Implicit Polymorphic $\lambda$-Calculus}
  \label{fig:STmd}
\end{figure}

\begin{figure}
  \input{tex/figures/SimpleTypingB.mng}
  \caption{Type Instantiation and Skolemisation}
  \label{fig:STmb}
\end{figure}

Figures~\ref{fig:STm}, \ref{fig:STmc}, \ref{fig:STmd} and~\ref{fig:STmb} show
the typing rules for our the IPLC.
 In order to support both type synthesis and checking,
we use a bidirectional type system. We review the high-level role of the judgements
and then examine details.

\paragraph{Type Synthesis}
Synthesis for expressions is performed by the $[[ G |- e => ne ~> ef ]]$ relation: ``Under typing
context $[[G]]$, the expression $[[e]]$ is assigned the type $[[ne]]$''.
As mentioned previously, the shape of the output type $[[ne]]$ is parameterised over the
eagerness of type instantiation $[[ep]]$. Under lazy instantiation, type
synthesis produces a type scheme $[[s]]$; under eager instantiation, the
output will be an instantiated type $[[r]]$.
Similar to expressions, pattern synthesis is performed by the $[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$ relation:
``Under typing context $[[G]]$, patterns $[[ps]]$ are assigned the argument descriptors $[[psigs]]$,
producing the context extension $[[Del]]$''.
Declaration synthesis is performed by the $[[ G |- decl => G' ~> x : s = ef ]]$ relation:
``The declaration $[[ decl ]]$ extends the typing context $[[G]]$ into $[[G']]$''.

\paragraph{Type Checking}
Checking for expressions is performed by the $[[ G |- e <= s ~> ef ]]$ relation: ``Under typing context
$[[G]]$, the expression $[[e]]$ is checked to have the type $[[s]]$''.
The type serves as an input here: an algorithmic interpretation of this relation
would simply return a pass/fail result.
Similarly, pattern checking is performed by the $[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$ relation:
``Under typing context $[[G]]$, patterns $[[ps]]$ match element-wise against $[[s]]$, producing the residual type $[[s']]$ and the context extension $[[Del]]$''.

\paragraph{Type Instantiation}
\renewcommand\elab[1]{}
The behaviour of both the instantiation $[[G |- s inst _ d r ~> ewf ]]$ and skolemisation
$[[ G |- s skol _ d r ; G' ]]$ judgements depends on whether the depth $[[ d ]]$
is deep $[[ D ]]$ or shallow $[[ S ]]$; see Figure~\ref{fig:STmb}.
The relations gather the binders of $[[s]]$ and instantiates or skolemises these with
monotypes $[[ts]]$ or fresh type variables, respectively.
Both invoke $[[ binders _ d ( s ) = as ; r ]]$, which splits a
type scheme $[[s]]$ into a list of its bound type variables $[[as]]$ and the
remaining instantiated type $[[r]]$. Under shallow instantiation (\rref{Bndr-Shallow}), this relation just
returns all type variables bound at the top of the input type scheme.
Under deep instantiation however (which is based directly on relations in \citet[Section~4.6.2]{practical-type-inference}), this gathers variables bound both at the top
level and on the right of function arrows.

The instantiation and skolemisation relations as presented here work properly only
when going from a type scheme $[[s]]$ to an instantiated type $[[r]]$. However,
we see some rules relate other types. For example, \rref{Tm-InfVar} instantiates
the type scheme $[[s]]$ assigned to a variable from a context to a synthesised type
$[[ne]]$ (the $[[ep]]$ is included to remind us on the importance of the eagerness parameter).
Because a synthesised type \emph{is} a type scheme when we work with lazy instantiation,
this instantiation in \rref{Tm-InfVar} is actually a no-op in that scenario;
however, under eager instantiation,
a synthesised type is the same as an instantiated type (with no $[[forall]]$s at the top),
and we must actually instantiate. This is why the use of instantiation in \rref{Tm-InfVar} is
coloured in \instE{emerald}. Conversely, examine \rref{Tm-InfApp}. This rule handles when we are applying
one expression to another. If we have instantiated eagerly, then we need take no action before
applying the function to the argument: any type variables in the function's type have already
been instantiated. Under lazy instantiation, however, function application is a point where we might
need to finally instantiate. Accordingly, the rule instantiates the synthesised $[[ne]]$ to
$[[s1 -> qd2]]$, which is an instantiated type, meta variable $[[r]]$. Recall that, under eager
instantiation, a synthesised type $[[ne]]$ is \emph{already} an instantiated type $[[r]]$, and
then this instantiation is a no-op. The instantiation applies only under the lazy scheme, and
thus is coloured in \instL{lavender}.

\paragraph{Data constructors}
Typing
a data constructor (\rref{Tm-InfCon}) works identically to typing variables,
after assembling the data constructor type from its pieces.

\paragraph{$\lambda$-expressions}
Synthesis for abstractions (\rref{Tm-InfAbs}) works as usual, by assigning
a monotype $[[t]]$ to the variable $[[x]]$ when checking the
expression $[[ee]]$. Type checking for abstractions (\rref{Tm-CheckAbs}) works
similarly, but also allows a full type scheme as argument type.
Note that we first need to skolemise the given type $[[s]]$ into a function
type $[[ s1 -> qd2 ]]$ (if this is not possible, type checking fails).
Skolemisation takes the available binders of $[[s]]$ and simply adds them to the
context $[[G']]$.
These variables behave as skolem constants when checking $[[ee]]$.

\paragraph{Function Application}
Let us examine \rref{Tm-InfApp} more closely, which synthesises the type
for an application $[[e1 e2]]$.
First,
the type of $[[e1]]$ is synthesised. Under eager instantiation, this produces an
instantiated type which should be a function type $[[ s1 -> qd2 ]]$; if it's not,
type synthesis fails.
Under lazy instantiation, and as described above, the type of $[[e1]]$ is now instantiated.
Then we must check the argument $[[e2]]$ against known type $[[s1]]$.
Having checked the application
itself, we must now perhaps instantiate the result type $[[qd2]]$. This would happen
only with eager instantiation, and there can be variables to instantiate only
when the previous eager instantiation did not find them---that is, when instantiation
is shallow. Thus the final premise to \rref{Tm-InfApp} applies only in the eager,
shallow scheme, marked in \instE{emerald} and with stripes.

\paragraph{Mode Changing}
Going from type synthesis to type checking is achieved using an
annotation. Typing an annotated expression $[[ ee : s ]]$ (\rref{Tm-InfAnn})
works by checking the expression $[[ee]]$ under the given type $[[s]]$.
Note that under eager instantiation, the
type for this annotated expression is not the type scheme $[[s]]$, but an
instantiated form of this type.

Going from checking to synthesis mode is also allowed (\rref{Tm-CheckInf}),
but only when \([[ee]]\) is not a lambda or let expression,
and thus when no other type checking rule would apply.
We first skolemise the given type $[[s]]$ to bind any new type variables in $[[G']]$.
We then infer a type for the expression $[[ee]]$ and match it against the skolemised type $[[r]]$.
Note that under lazy instantiation, the
synthesised type still needs to be instantiated in order to match $[[r]]$.

\paragraph{Let Binders}
As mentioned previously, $[[let]]$-expressions $[[ let edecl in ee ]]$ define a single
variable, with or without a type signature. See Figure~\ref{fig:STmc}, which
defines the judgement $[[ G |-E edecl => G' ~> x : s = ef ]]$. This judgement
examines a declaration to produce a new context $[[G']]$, extended with a binding
for the declared variable. 

\Rref{Decl-NoAnnSingle,Decl-NoAnnMulti} 
distinguish between a single equation without a type signature
and multiple equations. In the former case, we synthesise the types
of the patterns using the $[[|-P]]$ judgement and then the type of
the right-hand side. We assemble the complete type with $[[type]]$,
and then generalise. The multiple-equation case is broadly similar,
synthesising types for the patterns (note that each equation must
yield the \emph{same} types $[[psigs]]$) and then synthesising types
for the right-hand side. These types are then instantiated (only
necessary under \instL{lazy} instantiation---eager instantiation would
have already done this step).
This additional instantiation step is the only difference between
the single-equation case and the multiple-equation case.
The reason is that \rref{EDecl-NoAnnMulti} needs to construct a single type
that subsumes the types of every branch.
Following GHC, we simplify this process by first instantiating the types.
% Indeed, this difference is the only
% reason we have separated out the single-equation case, to be able
% to define synonyms of variables with higher-rank or non-prenex types.

\Rref{Decl-Ann} checks a declaration with a type signature. It
works by first checking the patterns $[[psi]]$ on the left
of the equals sign against the provided type $[[s]]$. The right-hand sides $[[eei]]$
are then checked against the remaining type $[[si']]$.
%% The pattern type checking relation $[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$ (see
%% Figure~\ref{fig:STmd}) checks the list of patters $[[ps]]$ under type scheme
%% $[[s]]$, and produces the remaining type $[[s']]$ and the typing context
%% extension $[[Del]]$.

\paragraph{Patterns}
The pattern synthesis relation $[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$ is presented in
Figure~\ref{fig:STmd}. As the full type is not yet available, it produces
argument descriptors $[[psigs]]$ and a typing context extension $[[Del]]$. Inferring a
type for a variable pattern (\rref{Pat-InfVar}) works similarly to expression
inference, by constructing a monotype and placing it in the context.
Inferring a type for a data constructor pattern (\rref{Pat-InfCon})
works by looking up the type $[[forall as0 . ss0 -> T as0]]$ of
the constructor $[[K]]$ in the typing context, and checking the applied
patterns $[[ps]]$ under this instantiated type.
Note that as there are no forall binders to the right of an arrow, instantiation
simply needs to supply types $[[ts0]]$ for the top level $[[as0]]$ variables.
The remaining type should be the
result type for the constructor, meaning that the constructor always needs to be
fully applied. Finally, the remaining patterns are typed under this extended
environment.

Checking a variable pattern in \rref{Pat-CheckVar} works by placing the
variable in the typing context, with its type $[[s1]]$, extracted from
the known type of the function we are checking. The same holds for checking against a polytype
 (\rref{Pat-CheckForall}), which gets skolemised by placing it in the
typing context.
Note that in order for the rules to be syntax-directed, \rref{Pat-CheckForall}
does not apply when the patterns are empty.
Checking a data constructor pattern (\rref{Pat-CheckCon}) works similarly to synthesis mode.
The type $[[forall as0 . ss0 -> T as0]]$
of the constructor is looked up in
the typing context. Then, the patterns $[[ps]]$ are
checked under an instantiated form of $[[forall as0 . ss0 -> T as0]]$.
The remaining type should then
be equal to an instantiated form of the provided type $[[s1]]$. Finally, the remaining
patterns $[[ps']]$ are checked under the extended context\footnote{Extending
the context for later patterns
is not used in the basic system, but it would be required for extensions like view
patterns.}.

\subsection{Alternative Formalisation}
\label{sec:alt}

Section~\ref{sec:modern} presents an extension of our $\lambda$-calculus
formalisation to a more advanced language, mixing
implicit and explicit polymorphism.
Notably, this covers features like recursive let bindings, visible type
application and variable specificity.
However, under eager instantiation, explicit type application poses an issue with
our current formalisation, as it requires temporarily postponing type
instantiation during inference.
Here, we replace our typing rules based on nested applications from
Section~\ref{sec:basic_typing} with an alternative formalisation
inspired by the structure from \citet{quick-look}.
The reason for this will become clear in Section~\ref{sec:modern}, as this
representation can easily be extended with explicit type application.

\begin{figure}
  \input{tex/figures/AltSyntax.mng}
  \input{tex/figures/AltTyping.mng}
  \input{tex/figures/AltTypingB.mng}
  \caption{Alternative formulation for the Implicit Polymorphic $\lambda$-Calculus}
  \label{fig:Asyn}
\end{figure}

%% \begin{figure}
%%   \caption{Alternative Term Typing for Implicit Polymorphic $\lambda$-Calculus}
%%   \label{fig:ATm}
%% \end{figure}

%% \begin{figure}
%%   \caption{Argument Type Checking for Implicit Polymorphic $\lambda$-Calculus}
%%   \label{fig:ATmb}
%% \end{figure}

Figure~\ref{fig:Asyn} shows the updated system. These rules implement the \emph{same}
language as the rules we reviewed previously, but it is recast
in a way easier to extend later.

\paragraph{Application}
In order to simplify the introduction of explicit type application, applications
are now modelled as applying a head $[[h]]$ to a (maximally long)
list of arguments $[[args]]$.
This concept of modelling applications is inspired by \citet{quick-look},
 which also features visible type application and eager instantiation.
The main idea is that under eager instantiation, type instantiation
for the head is postponed until it has been applied to its arguments.
A head $[[h]]$ is thus defined to be either a variable $[[x]]$, a data
constructor $[[K]]$, an annotated expression $[[e : s]]$ or a simple expression
$[[e]]$. This last form will not be typed with a type scheme under eager
instantiation---that is, we will not be able to use explicit instantiation---but is required to enable application of a lambda expression.
At the moment, as we have only term application (not type application), an argument $[[arg]]$ is defined to
just be an expression $[[e]]$. This will be extended in Section~\ref{sec:modern}
to include type application as well.

When inferring a type for an application $[[h args]]$ (\rref{ETm-InfApp}), a
type scheme $[[s]]$ is inferred for the head $[[h]]$.
The arguments $[[args]]$ are then checked under this type $[[s]]$, producing a
residual type $[[s']]$\footnote{The application judgement is inspired
by \citet{simple-bidirectional}.}. Finally, after the head has been applied to all its
arguments, the remaining type $[[s']]$ is instantiated (under eager
instantiation), producing a type $[[ne]]$ for the final expression.

Note that as applications are always typed in this fashion, head typing
needs only a synthesis mode, and argument typing needs to be defined only for
checking mode.
Type synthesis for heads $[[ G |-H h => s ~> ef ]]$ works identically to expressions
from the basic system, except that the types are not instantiated.
Argument type checking $[[ G |-A args <= s => s' ~> fargs ]]$ bears a close resemblance
to pattern checking, taking a typing context $[[G]]$, a list of arguments
$[[args]]$ and a type scheme $[[s]]$ and producing a residual type $[[s']]$.
Concretely, this means that bound type variables in the given type are instantiated
(\rref{Arg-Inst}) and the list of arguments are type checked to have the given type.


==> tex/sections/IdrisAgdaHaskell.tex <==
%if style == newcode
\begin{code}
module IdrisAgdaHaskell where

\end{code}
%endif

\section{Instabilities around instantiation beyond Haskell}
\label{sec:idris-agda-haskell}

The concept of stability is important in languages that have a mix of implicit
and explicit features---a very common combination, appearing in Coq, Agda, Idris,
modern Haskell, C++, Java, C\#, Scala, F\#, and Rust, among others.
 This appendix walks through how a mixing of implicit
and explicit features in
Idris\footnote{\raggedright We work with Idris 2, as available from \url{https://github.com/idris-lang/Idris2},
at commit \textsf{a7d5a9a7fdfbc3e7ee8995a07b90e6a454209cd8}.} and Agda\footnote{We work with Agda~2.6.0.1.} 
causes instability, alongside the features of Haskell we describe in the
main paper. We use these languages to show how the issues we 
describe are likely going to arise in any language mixing implicit and explicit
features---and how stability is a worthwhile metric in examining these features---not
to critique these languages in particular.

%% Many of the key terms in this line of work have subtly different meanings
%% throughout the existing literature. We pin down terminology here.

%% \paragraph{Polymorphism} A function exhibits polymorphism when it can be
%% used at multiple different concrete types. We consider two forms of
%% polymorphism: \emph{Parametric polymorphism} describes a function that
%% treats all types identically---the choice of type is irrelevant at runtime.
%% The |const| function from the introduction is parametrically polymorphic.
%% \emph{Ad-hoc polymorphism} describes a function with different
%% behavior for different types. A function like |+| that works over different
%% numeric types would have ad-hoc polymorphism. Many functional languages
%% use type classes~\cite{wadler-blott} to implement ad-hoc polymorphism; other
%% languages use operator overloading or object-oriented class-based polymorphism
%% to accomplish similar goals.

%% \paragraph{Generalization} Some languages---notably, those derived from the
%% Hindley-Milner type system---perform generalization. If a programmer writes
%% a function that could work over multiple types, the type system assigns a
%% polymorphic (general) type to that function, instead of a specific type
%% that works over only one argument type. For example, if we define |id x = x|
%% in Haskell, we get the type |id :: forall a. a -> a|, not the type |id :: Int -> Int|.

%% \paragraph{Type signatures} Languages may require that all defined variables
%% have a type signature, declaring in advance the type of that variable. These
%% include both C-like languages (though recent innovations such as $\keyword{auto}$
%% in C++ and $\keyword{var}$ in Java blur this distinction) and many dependently
%% typed languages, such as Agda or Idris. Languages derived from Hindley-Milner,
%% including Haskell and ML, generally support but do not require type signatures,
%% instead using type inference to assign types to variables. Some languages support
%% \emph{partial type signatures}~\cite{partial-type-signatures}, where there is a
%% mix of known and unknown information. For example, Haskell allows us to declare
%% %
%% \begin{code}
%% not :: _ -> Bool
%% not  True   =  False
%% not  False  =  True
%% \end{code}
%% %
%% and the type for |not| is inferred to be |Bool -> Bool|. This uses a recent---and
%% somewhat exotic---feature in GHC. However, partial
%% type signatures exist beyond this one Haskell extension. For example, Idris allows
%% %
%% \begin{spec}
%% len : (a : _) -> List a -> Int
%% len _  []         =  0
%% len a  (_ :: xs)  =  1 + len a xs
%% \end{spec}
%% %
%% Here, the interpreter can figure out that the type of |a| is really |Type|, but
%% that is not specified by the user. Clever uses of this feature can lead Idris
%% to perform generalization, even though the language requires type signatures. See \pref{sec:idris-generalization}
%% for an example. \rae{Check with Idris 2.}

%% \paragraph{Bidirectional type checking}
%% In order to support advanced type system features, many languages support
%% \emph{bidirectional type checking}~\cite{?}, where the type checker uses type annotations
%% to direct how to interpret the annotated expressions. \rae{More here}

%% \rae{I've stopped updating this section, thinking that this is better to revisit when 
%% we have a better idea of what will be needed by the final paper.}

%% \subsection{Type Signatures}

%% Writing type signatures is always a good idea as they serve as both a sanity
%% check and as machine-checked documentation.
%% However, as the compiler can often infer the type automatically, most languages
%% do not require programmers to explicitly write type signatures.
%% Indeed, the compiler can use a bidirectional type system, which
%% can both check user-written type annotations and infer missing types.

%% In order to achieve this, the type system has to be able to instantiate
%% polymorphic types, as well as generalise types. The former means that the
%% compiler can fill in either a concrete type, or a unification variable (to be
%% instantiated later on) for a type variable. The latter means that unsolved
%% unification variables can be abstracted over in a \texttt{forall} binder.
%% Section~\ref{sec:inst} discusses different options regarding where and how this
%% instantiation may happen.
%% Note both this abstraction and instantiation happens implicitly.

\subsection{Explicit Instantiation}

Our example languages
feature explicit instantiation of implicit arguments, allowing the programmer to manually
instantiate a polymorphic type, for example.
Explicit instantiation broadly comes in two flavours: ordered or
named parameters.

\subsection{Idris}
Idris supports named parameters.
If we define |const : {a, b : Type} -> a -> b -> a| (this syntax is the Idris
equivalent of the Haskell type |forall a b. a -> b -> a|), then we can write |const {b = Bool}|
to instantiate only the second type parameter or |const {a = Int} {b = Bool}| to instantiate
both. Order does not matter; |const {b = Bool} {a = Int}| works as well as the previous example.
Named parameters may be easier to read than ordered parameters and are robust to the addition
of new type variables.

Idris's approach suffers from an instability inherent with named parameters.
Unlike Haskell, the order of quantified variables does
not matter. Yet now, the choice of \emph{names} of the parameters naturally \emph{does} matter.
Thus |const : c -> d -> c| (taking advantage of the possibility of omitting explicit quantification
in Idris) has a different interface than |const : a -> b -> a|, despite
the fact that the type variables scope over only the type signature they appear in.

\subsection{Agda}
Agda accepts both ordered and named parameters.
After defining |const : {a b : Set} -> a -> b -> a|, we can write expressions like
|const {Int}| (instantiating only |a|), |const {b = Bool}|, or |const {_} {Bool}|.
Despite using named parameters, order \emph{does} matter: we cannot instantiate
earlier parameters after later ones. Naming is useful for skipping parameters that
the user does not wish to instantiate. Because Agda requires explicit quantification
of variables used in types (except as allowed for in implicit generalisation, below),
the ordering of variables must be fixed by the programmer. However, like Idris,
Agda suffers from the fact that the choice of name of these local variables leaks to clients.

\subsection{Explicit Abstraction \gertjan{Improve the flow of this section}}
\label{sec:explicit-abstraction}

\paragraph{Binding implicit variables in named function definitions}
If we sometimes want to explicitly instantiate an implicit argument, we will also sometimes
want to explicitly abstract over an implicit argument. A classic example of why this is
useful is in the |replicate| function for length-indexed vectors, here written in Idris:
%
\begin{spec}
replicate : {n : Nat} -> a -> Vect n a
replicate {n = Z}    _  =  []
replicate {n = S _}  x  =  x :: replicate x
\end{spec}
%
Because a length-indexed vector |Vect| includes its length in its type, we need not
always pass the desired length of a vector into the |replicate| function: type inference
can figure it out. We thus decide here to make the |n : Nat| parameter to be implicit,
putting it in braces. However, in the definition of |replicate|, we must pattern-match
on the length to decide what to return. The solution is to use an explicit pattern,
in braces, to match against the argument |n|.

Idris and Agda both support explicit abstraction in parallel to their support of explicit
instantiation: when writing equations for a function, the user can use braces to denote
the abstraction over an implicit parameter. Idris requires such parameters to be named,
while Agda supports both named and ordered parameters, just as the languages do for
instantiation. The challenges around stability are the same here as they are for explicit
instantiation.

Haskell has no implemented feature analogous to this. Its closest support is that
for scoped type variables, where a type variable introduced in a type signature becomes
available in a function body. For example:
%
\begin{code}
const :: forall a b. a -> b -> a
const x y = (x :: a)
\end{code}
%
The |forall a b| brings |a| and |b| into scope both in the type signature \emph{and}
in the function body. This feature in Haskell means that, like in Idris and Agda,
changing the name of an apparently local variable in a type signature may affect
code beyond that type signature. It also means that the top-level |forall| in a type
signature is treated specially. For example, neither of the following examples
are accepted by GHC:
%
%format const1
%format const2
\begin{spec}
const1 :: forall . forall a b. a -> b -> a
const1 x y = (x :: a)

const2 :: (forall a b. a -> b -> a)
const2 x y = (x :: a)
\end{spec}
%
In |const1|, the vacuous |forall .| (which is, generally, allowed)
stops the scoped-type variables mechanism from
bringing |a| into scope; in |const2|, the parentheses around the type serve the same
function. Once again, we see how Haskell is unstable: programmers might reasonably
think that syntax like |forall a b .| is shorthand for |forall a. forall b.| or that
outermost parentheses would be redundant, yet neither of these facts is true.

\paragraph{Binding implicit variables in an anonymous function}
Sometimes, binding a type variable only in a function declaration is not expressive
enough, however---we might want to do this in an anonymous function in the middle
of some other expression.

Here is a (contrived) example of this in Agda,
where $\ni$ allows for prefix type annotations:
%
%format NAT = "\mathbb{N}"
%format x1
%format x2
%format Set1
%format _ni_ = "\_{\ni}\_"
%format ni x y = x "\ni" y
\begin{spec}
_ni_ : (A : Set) -> A -> A
ni A x = x

ChurchBool  :  Set1
ChurchBool  =  {A : Set} -> A -> A -> A

churchBoolToBit : ChurchBool -> NAT
churchBoolToBit b = b 1 0

one  :  NAT
one  =  churchBoolToBit (\ {A} x1 x2 -> ni A x1)
\end{spec}
%
Here, we bind the implicit variable |A| in the argument to |churchBoolToBit|. (Less
contrived examples are possible; see the Motivation section of \citet{proposal-155}.)

Binding an implicit variable in a $\lambda$-expression is subtler than doing it in
a function clause. Idris does not support this feature at all, requiring
a named function to bind an implicit variable. Agda supports this feature, as written
above, but with caveats: the construct only works sometimes. For example, the following
is rejected:
%
\begin{spec}
id : {A : Set} -> A -> A
id = \ {A} x -> ni A x
\end{spec}
%
The fact that this example is rejected, but |id {A} x = ni A x| is accepted is another
example of apparent instability---we might na\"\i{}vely expect that writing a function
with an explicit $\lambda$ and using patterns to the left of an |=| are equivalent.
\gertjan{Add a brief explanation why this is the case}
Another interesting aspect of binding an implicit variable
in a $\lambda$-abstraction is that the name of the variable is utterly arbitrary: instead
of writing |(\ {A} x1 x2 -> ni A x1)|, we can write |(\ {anything = A} x1 x2 -> ni A x1)|.
This is an attempt to use Agda's support for named implicits, but the name can be, well,
|anything|. This would appear to be a concession to the fact that the proper name for this
variable, |A| as written in the definition of |ChurchBool|, can be arbitrarily far away
from the usage of the name, so Agda is liberal in accepting any replacement for it.

An accepted proposal~\cite{proposal-155} adds this feature to Haskell, though it has
not been implemented as of this writing. That proposal describes that the feature
would be available only when we are \emph{checking} a term against a known type,
taking advantage of GHC's bidirectional type system~\cite{practical-type-inference,visible-type-application}.
One of the motivations that inspired this paper was to figure out whether we
could relax this restriction. After all, it would seem plausible that we should
accept a definition like |id = \ @a (x :: a) -> a| without a type signature.
(Here, the |@a| syntax binds |a| to an otherwise-implicit type argument.)
It will turn out that, in the end, we can do this only when we instantiate
lazily---see Section~\ref{sec:evaluation}.

\subsection{Implicit Generalisation}

%% As introduced above, this paper uses \emph{stability} as a method for evaluating
%% the usability of a language; recall that a \emph{stable} language is resistant
%% to seemingly innocuous changes. We consider here some challenges for maintaining
%% stability in a language with both implicit and explicit type instantiation.

All three languages support some form of implicit generalisation, despite the fact
that the designers of Haskell famously declared that |let| should not
be generalised~\cite{let-should-not-be-generalised} and that both Idris
and Agda require type signatures on all declarations.

\paragraph{Haskell}
Haskell's |let|-generalisation is the most active, as type signatures are
optional.\footnote{Though not relevant for our analysis, some readers
may want the details: Without any language extensions enabled, all declarations without
signatures are generalised, meaning that defining |id x = x| will give |id|
the type |forall a. a -> a|. With the @MonoLocalBinds@ extension enabled,
which is activated by either of @GADTs@ or @TypeFamilies@, local
definitions that capture variables from an outer scope are not generalised---this
is the effect of the dictum that |let| should not be generalised. As an example,
the |g| in |f x = let g y = (y, x) in (g 'a', g True)| is not generalised, because
its body mentions the captured |x|. Accordingly, |f| is rejected, as it uses |g|
at two different types (|Char| and |Bool|). Adding a type signature to |g| can fix the problem.}
%
Suppose we have defined |const x y = x|, without a signature.
What type do we
infer? It could be |forall a b. a -> b -> a| or |forall b a. a -> b -> a|.
This choice matters, because it affects the meaning of explicit type
instantiations. A natural reaction is to suggest choosing the former inferred
type, following the left-to-right scheme described above.
However, in a language with a type system
as rich as Haskell's, this guideline does not always work. Haskell supports
type synonyms (which can reorder the occurrence of variables), class
constraints (whose ordering is arbitrary)~\cite{type-classes}, functional
dependencies (which mean that a type variable might be mentioned \emph{only}
in constraints and not in the main body of a
type)~\cite{fundeps}, and arbitrary type-level computation
through type families~\cite{chak1,closed-type-families}. With all of these features potentially
in play, it is unclear how to order the type variables. Thus, in a concession to
language stability, Haskell brutally
forbids explicit type instantiation on any function whose type is inferred;
we discuss the precise mechanism in the next section.

Since GHC~8.0, Haskell allows dependency within
type signatures~\cite{nokinds}, meaning that the straightforward left-to-right ordering
of variables---even in a user-written type signature---might not be well-scoped.
As a simple example, consider |tr :: TypeRep (a :: k)|, where |TypeRep :: forall k. k -> Type|
allows runtime type representation and is part of GHC's standard library.
A naive left-to-right extraction of type variables would yield |forall a k. TypeRep (a :: k)|,
which is ill-scoped when we consider that |a| depends on |k|.
Instead, we must reorder to |forall k a. TypeRep (a :: k)|. In order to support
stability when instantiating explicitly, GHC thus defines a concrete sorting
algorithm, called ``ScopedSort'', that reorders the variables; it has become part of GHC's user-facing
specification. Any change to this algorithm may break user programs, and it
is specified in \href{https://downloads.haskell.org/ghc/latest/docs/html/users_guide/glasgow_exts.html#index-20}{GHC's user manual}.

\paragraph{Idris}
Idris's support for implicit generalisation is harder to trigger; see \pref{app:idris-generalisation}
for an example of how to do it.
The problem that arises in Idris is predictable: if the compiler
performs the quantification, then it must choose the name of the quantified
type variable. How will clients know what this name is, necessary in order
to instantiate the parameter? They cannot. Accordingly,
in order to support stability, Idris uses a special name for generalised variables:
the variable name itself includes braces (for example, it might be |{k:265}|) and
thus can never be parsed\footnote{Idris 1 does not use an exotic name, but still
prevents explicit instantiation, using a mechanism similar to Haskell's specificity
mechanism.}.

\paragraph{Agda}
Recent versions of Agda support a new \keyword{variable} keyword\footnote{See
\url{https://agda.readthedocs.io/en/v2.6.0.1/language/generalization-of-declared-variables.html} in
the Agda manual for an description of the feature.}. Here is an example of it
in action:
%
%format l1
%format l2
%format variable = "\keyword{variable}"
\begin{spec}
variable
  A : Set
  l1 l2 : List A
\end{spec}
%
The declaration says that an out-of-scope use of, say, |A| is a hint to Agda
to implicitly quantify over |A : Set|. The order of declarations in a |variable|
block is significant: note that |l1| and |l2| depend on |A|. However, because
explicit instantiation by order is possible in Agda, we must specify the
order of quantification when Agda does generalisation. Often, this order
is derived directly from the |variable| block---but not always. Consider this
(contrived) declaration:
%
%format === = "\equiv"
\begin{spec}
property : length l2 + length l1 === length l1 + length l2
\end{spec}
%
What is the full, elaborated type of |property|? Note that the two lists
|l1| and |l2| can have \emph{different} element types |A|. The Agda manual
calls this \emph{nested} implicit generalisation, and it specifies an algorithm---similar to
GHC's ScopedSort---to specify the ordering of variables. Indeed it must
offer this specification, as leaving this part out would lead to instability; that is,
it would lead to the inability for a client of |property| to know how to order
their type instantiations.


==> tex/sections/IdrisGeneralisation.tex <==
%if style == newcode
\begin{code}
module IdrisGeneralisation where
\end{code}
%endif

\section{Example of Implicit Generalisation in Idris}
\label{app:idris-generalisation}

It is easy to believe that a language that requires type signatures on all definitions
will not have implicit generalisation. However, Idris does allow generalisation to creep in,
with just the right definitions.

We start with this:
%
\begin{spec}
data Proxy : {k : Type} -> k -> Type where
  P : Proxy a
\end{spec}
%
The datatype |Proxy| here is polymorphic; its one explicit argument can be of any type.

Now, we define |poly|:
%
\begin{spec}
poly : Proxy a
poly = P
\end{spec}
%
We have not given an explicit type to the type variable |a| in |poly|'s type. Because
|Proxy|'s argument can be of any type, |a|'s type is unconstrained. Idris \emph{generalises}
this type, giving |poly| the type |{k : Type} -> {a : k} -> Proxy a|.

At a use site of |poly|, we must then distinguish between the possibility of instantiating
the user-written |a| and the possibility of instantiating the compiler-generated |k|. This
is done by giving the |k| variable an unusual name, @{k:446}@ in our running Idris session.


==> tex/sections/Instantiation.tex <==
%if style == newcode
\begin{code}
{-# LANGUAGE RankNTypes, BangPatterns #-}

module Instantiation where

pair = (,)
\end{code}
%endif

\section{Type Instantiation}
\label{sec:inst}

We now turn to our main feature of study: implicit instantiation. This section lays out
several alternative ways of designing this feature.
Section~\ref{sec:stability} shows that each can cause instability,
and Section~\ref{sec:calculus} develops typing rules
(based on the current behaviour
of GHC/Haskell, with key inspiration from \citet{practical-type-inference,visible-type-application,quick-look}) so that we
can prove how our choices of instantiation technique either respect or do not respect
the similarities.

Our key question: Given a polymorphic function |f|, how and when should we instantiate it to
concrete types? 

We introduce several different flavours of instantiation algorithm,
 differing in two orthogonal axes: when types
 are instantiated, and the depth to which binders are instantiated.
 Section~\ref{sec:stability} will showcase several examples
 where these choices make a real difference.

%% \rae{I don't think this observation is all that helpful.}
%% These two represent the extreme edges of the spectrum, but are far from the only
%% options, as one can easily come up with intermediate alternatives such as
%% only instantiating before generalising, or even more exotic variants like
%% eagerly instantiating type variables but instantiating class constraints lazily.

%% \paragraph{Example 7: |plus|}

%% One of Haskell's more exotic features is its \emph{monomorphism restriction}.
%% Simplifying to single definitions (the actual restriction applies to mutually
%% recursive groups of definitions), the restriction states that all non-function
%% bindings must be unconstrained. Here, a ``non-function binding'' is a binding
%% that looks like |x = undefinedDots|, for example; note that there are no
%% parameters included to the left of the |=|. This restriction applies to a
%% definition like |x = expensive 100|, where
%% |expensive :: forall a. Num a => a -> a|. We could imagine inferring the type
%% |forall a. Num a => a| for |x|, and doing so would be sound. However, it would
%% mean that we would be forced to recalculate |expensive 100| every time we use
%% |x| and make a concrete choice of numerical representation. Given that |x| certainly
%% does not look like a function, it is possible that this recomputation would come
%% as a surprise to programmers. Thus, Haskell requires that the inferred type of |x|
%% be unconstrained. The precise numerical representation would be determined by use
%% sites of |x| or would be defaulted (to |Integer|, absent any Haskell |default|
%% directives changing the defaulting scheme).

%% With that in mind, consider this definition for |plus|:
%% %
%% \begin{code}
%% plus = (+)
%% \end{code}
%% %
%% This innocent definition uses |(+) :: Num a => a -> a -> a|, the overloaded
%% addition operator. Here are the types inferred for |plus|:
%% \begin{center}
%% \begin{tabular}{l||l||l}
%% |plus| & eager & lazy \\ \hline
%% deep/shallow & |Integer -> Integer -> Integer| & |forall a. Num a => a -> a -> a| \\ \hline
%% \end{tabular}
%% \end{center}
%% With eager instantiation, we instantiate |(+)|. We then fail to re-generalize, because
%% doing so would end up putting a constraint on the type of |plus|, forbidden by the
%% monomorphism restriction. We then default the type to the one in the table. However,
%% with lazy instantiation, we never get the chance to monomorphize; |plus| gets the
%% full polymorphic type of |(+)|. This is problematic, because it violates the
%% specification of standard Haskell, with its monomorphism restriction. Worse, the
%% problem might appear only as a performance regression at runtime.

%% While we might imagine that, even under lazy instantiation, we look ahead to detect
%% this case and handle it correctly. However, that would be harder with a definition
%% like |constPlus = \ _ -> (+)|, where we would have to look arbitrarily deeply to
%% find an offending constraint.

%if 0
% I've commented this example out, as it's a red herring. It might be an interesting
% red herring to GHC aficionados, but we don't need it in the paper
\paragraph{Example 8: |diverge|}

Haskell famously includes the |undefined| variable. Since GHC~8.0, its type
has been |forall a. HasCallStack => a|\footnote{We are ignoring the
levity polymorphism~\cite{levity-polymorphism} in |undefined|'s type here.}.
The |HasCallStack| nullary constraint is a mechanism to help produce stack
traces when an exception is thrown: all usage sites of |undefined| thus pack
their source location into a |CallStack| structure and pass that to the
|undefined| function, which reports it. While these details are unimportant,
the fact that there is a constraint on |undefined| is critical: it means that
|undefined| is a \emph{function}, and, like all functions, is a value.

We now look at another thorny example:
%
\begin{code}
diverge = let BANG x = undefined in ()
\end{code}
%
The |bang| ensures that the binding is strict; we want this to diverge.
Unlike the other scenarios we have explored, the critical question here
is not one of \emph{compile time} semantics, but one of \emph{runtime} semantics.
We use the symbol $\reduces$ in our table to denote that we are talking
about runtime behaviour here.
\begin{center}
\begin{tabular}{l||l||l}
|diverge| & eager & lazy \\ \hline
deep or shallow & $\reduces \bot$ & $\reduces |()|$ \\
\end{tabular}
\end{center}
%
Why, under lazy instantiation, would |diverge| reduce to |()|? Because
|undefined| is a function; forcing it reveals that it is a function, and
no exception is thrown. This is surely counter intuitive!
However, under eager instantiation, the occurrence
of |undefined| is instantiated with a concrete type for |a| and a call stack,
and then forcing the result of that instantiation indeed does diverge.

Consider now this alternative:
%
\begin{code}
diverge2 = let  x       ::  Int
                BANG x  =   undefined in ()
\end{code}
%
Here, in order to check |undefined| at type |Int|, we must instantiate
under both the eager and lazy schemes. Thus |diverge2| always diverges.

This example shows another way in which instability can arise: we might
expect that adding a type annotation can affect only static semantics,
but (since types are erased) should not affect runtime semantics. However,
under lazy instantiation, the type signature drastically changes the
behaviour in this example.
%endif

%if 0
This is commented out (by lhs2TeX). But I'm including it in case we want yet
another example.

\begin{code}
{-# LANGUAGE ImplicitParams #-}

x :: (?i :: Int) => Int
x = ?i

y :: (?i :: Int) => Int
y = let ?i = 5 in x

z :: Int
z = let ?i = 6 in y
\end{code}

Lazy instantiation makes a hash of that example.
%endif



==> tex/sections/Introduction.tex <==
%if style == newcode
\begin{code}
module Introduction where
\end{code}
%endif

\section{Introduction}

Programmers naturally wish to get the greatest possible utility from their
work. They thus embrace \emph{polymorphism}: the idea that one function
can work with potentially many types. A simple example is |const :: forall a b. a -> b -> a|,
which returns its first argument, ignoring its second. The question then
becomes: what concrete types should |const| work with at a given call site?
For example, if we say |const True 'x'|, then a compiler needs to figure out
that |a| should become |Bool| and |b| should become |Char|. The process
of taking a type variable and substituting in a concrete type is called
\emph{instantiation}. Choosing a correct instantiation is important; for
|const|, the choice of |a =-> Bool| means that the return type of |const True 'x'|
is |Bool|. A context expecting a different type would lead to a type error.

In the above example, the choices for |a| and |b| in the type of |const| were
inferred. Haskell, among other languages, also gives programmers the opportunity to \emph{specify}
the instantiation for these arguments~\cite{visible-type-application}.
For example, we might say
|const @Bool @Char True 'x'| (choosing the instantiations for both |a| and |b|)
or |const @Bool True 'x'| (still allowing inference for |b|). However, once we start
allowing user-directed instantiation, many thorny design issues arise. For example,
will |let f = const in f @Bool True 'x'| be accepted? %% Many language systems additionally allow
%% users to query the type of an expression. What is the type of |const True|, then?
%% If you say |forall b. b -> Bool|, then is |const True @Char 'x'| acceptable?

%% More generally than thinking only about type variable instantiation, we can
%% consider the specification of implicit arguments. Type variables are just
%% one form of implicit argument, but many languages support default arguments
%% or other implicits. The questions we float
%% above can become even more pressing when passing implicit arguments that
%% are relevant at runtime. 
%% We use the term \emph{instantiation} broadly to include both the selection of
%% concrete types for type variables and also the supply of runtime-relevant
%% implicit arguments.

%% This paper considers both implicit and explicit instantiation in Haskell, and how
%% design decisions around instantiation can affect the ease of programming.
%% Beyond Haskell, every language that supports polymorphism must make decisions
%% around instantiation. It is our opinion that many designers grapple with
%% these issues; this paper aims to unpack these issues and lay out a framework
%% in which one can assess what design choices are best for a language.

Our concerns are rooted in concrete design questions in Haskell, as embodied by the
Glasgow Haskell Compiler (GHC). Specifically, as Haskell increasingly has
features in support of type-level programming, how should its instantiation
behave? Should instantiating a type like |Int -> forall a. a -> a| yield
|Int -> alpha -> alpha| (where |alpha| is a unification variable), or should
instantiation stop at the regular argument of type |Int|?
This is a question of the \emph{depth}
of instantiation. Suppose now |f :: Int -> forall a. a -> a|. Should |f 5| have
type |forall a. a -> a| or |alpha -> alpha|? This is a question of the
\emph{eagerness} of instantiation. As we explore in \pref{sec:stability},
these questions have real impact on our users.

Unlike much type-system research, our goal is \emph{not} simply to make a type-safe
and expressive language.
Type-safe instantiation is well understood~\cite[e.g.,][]{reynolds-systemf,damas-milner}. Instead,
we wish to examine the \emph{usability} of a design around instantiation. Unfortunately,
proper scientific studies around usability are essentially intractable, as we would
need pools of comparable experts in several designs executing a common task. Instead
of usability, then, we draw a fresh focus to a property we name \emph{stability}.

Intuitively,
a language is \emph{stable} if small, seemingly-in\-noc\-u\-ous changes to the source code
of a program do not
cause large changes to the program's behaviour; we expand on this definition
in \pref{sec:stability}. We use stability as our metric for evaluating instantiation
schemes in GHC.
%%  input of the language implementation
%% do not cause large changes
%% to the output (i.e., the compiled executable or the behaviour of an interpreter).
%% Yet we do not mean exactly that: changing an index in a program from 0
%% to 1 might reasonably drastically change a program's behaviour. Instead, we identify a
%% set of program changes that programmers might expect to have no effect; we call these
%% \emph{program similarities}. A language is stable if changing one program into
%% a similar one produces no change in behaviour. We say a language \emph{respects}
%% a similarity if similar programs indeed have the same behaviour. For example, we generally expect
%% that |a + b| in a program text has the same meaning as |b + a|; we would thus say
%% that |a + b| is similar to |b + a|. Yet a language with implicit type conversions might
%% not always respect
%% this similarity, perhaps leading the two expressions to have different types.
%% In the context of instantiation, we present
%% a set of similarities; different instantiation strategies cause a design to
%% respect different similarities. \rae{This paragraph is not the sharpest. Also,
%% I changed from \emph{equivalence} to \emph{similarity}. When I said stuff about
%% ``equivalent programs have the same behavior'' it sounded too tautological.}

%% The concept of stability becomes even more relevant in the context of high-level
%% languages with implicit features. If we imagine a fully explicit language---say, System F~\cite{reynolds-systemf}---stability
%% is essentially guaranteed; the explicit nature of the language means that programmers
%% say exactly what they mean. Even in the more implicit Hindley-Milner type system~\cite{hindley,milner},
%% we have stability, via careful design of the type system. One could say that the
%% success and ease of Hindley-Milner is precisely due to their design being stable.
%% However, beyond the
%% scope of Hindley-Milner, using a mix of implicit and explicit features (such
%% as visible type instantiation~\cite{visible-type-application}), stability becomes
%% an important and non-trivial concern. For this reason, this paper defines a concrete notion
%% of stability, and then uses it to analyse a type system parameterised on the way
%% it instantiates implicit arguments.

%% This paper proceeds by explaining \emph{stability}, our metric for understanding
%% and evaluating language design. The concept of stability and our general approach
%% of analysis with respect to stability is language- and feature-agnostic.
%% We then identify how mixing implicit with explicit
%% instantiation can lead to instability in several languages (Haskell, Agda, and Idris);
%% accordingly, choosing a design around instantiation is a key design step in any
%% language mixing implicit and explicit instantiation. Having laid out our approach
%% (stability) and our problem (how to design instantiation), we then explore how to
%% apply this approach to the concrete setting of the problem in Haskell, concluding that
%% \emph{shallow}, \emph{lazy} instantiation leads to the most stable design. This
%% result came as something of a surprise: as recently as GHC~8.10, Haskell used a deep, eager
%% strategy. GHC~9.0 updated this to use shallow and eager. We advocate here to take
%% a further step to be shallow and lazy.

Our contributions are as follows:
\begin{itemize}
  \item The introduction of stability properties relevant for examining
    instantiation in Haskell, along with examples of how these properties affect programmer
    experience. (Section~\ref{sec:stability})
%%   \item A comparison of the instantiation strategies in Haskell, Agda, and Idris (Section~\ref{sec:language-comparison}), illustrated with a number of concrete examples of potential
%% confusion in Haskell (Section~\ref{sec:inst}). These motivate our interest in
%% exploring instantiation in detail.
  \item A family of type systems, based on the bidirectional type-checking algorithm
    implemented in GHC~\cite{practical-type-inference,visible-type-application,quick-look}. It is parameterised
    over the flavour of type instantiation. (Section~\ref{sec:calculus})
  \item An analysis of how different choices of instantiation flavour either
    respect or do not respect the similarities we identify. We conclude that
    lazy, shallow instantiation
    is the most stable. (Section~\ref{sec:evaluation}; proofs in Appendix~\ref{app:formalproofs})
  %% \item An application of our results to the concrete use case of GHC/Haskell (Section~\ref{sec:ghc}) \rae{Is this still a separate contribution?}
\end{itemize}

Though we apply stability as the mechanism of studying instantiation within
Haskell, we believe our approach is more widely applicable, both to other
user-facing design questions within Haskell and in the context of other
languages.

%% We use Haskell both as a \emph{lingua franca} throughout this paper, and also as
%% inspiration for the main technical development in this paper. Stability issues
%% are necessarily language-specific, as authors in different languages will naturally
%% have different expectations as to what programs are considered similar. However,
%% our general approach---examining a language though the lens of \emph{stability}---is
%% portable across languages, and our work serves as a template for how one might perform
%% this analysis in a different setting.

The appendices mentioned in the text can be found in the extended version at
\url{http://arxiv.org/abs/2106.14938}.


==> tex/sections/Metatheory.tex <==
%if style == newcode
\begin{code}
module Metatheory where
\end{code}
%endif

\section{Evaluation}
\label{sec:evaluation}

This section evaluates the impact of the type instantiation flavour on the
stability of the programming language.
To this end, we define a set of eleven properties, based on the informal
definition of stability from Section~\ref{sec:stability}.
Every property is analysed against the four instantiation flavours, the results
of which are shown in Table~\ref{tab:prop}, which also references the
proof appendix for each of the properties, in the column labeled App.

We do not investigate the type safety of our formalism, as 
the MPLC is a subset of System~F. We can thus be confident
that programs in our language can be assigned a sensible runtime
semantics without going wrong.

\subsection{Contextual Equivalence}

Following the approach of GHC, rather than providing an operational semantics
of our type system directly, we instead define an elaboration of the surface
language presented in this paper to explicit System~F, our core language.
It is important to remark that elaborating deep instantiation into this core
language involves semantics-changing $\eta$-expansion.
This allows us to understand the behaviour of Example~5, |swizzle|, which
demonstrates a change in runtime semantics arising from a type signature.
This change is caused by $\eta$-expansion, observable only in the core language.

The definition of this core language and the elaboration from MPLC to core are
in \pref{app:systemf}. The meta variable $[[ef]]$ refers to core terms,
and $[[~>]]$ denotes elaboration.
In the core language, $\eta$-expansion is expressed through the use of an
expression wrapper $[[ewf]]$, an expression with a hole, which retypes the
expression that gets filled in. The full details can be found in \pref{app:systemf}.
We now provide an intuitive definition of contextual equivalence
in order to describe what it means for runtime semantics to remain unchanged.

\begin{definition}[Contextual Equivalence]
  Two core expressions \( [[ ef1 ]] \) and \( [[ ef2 ]] \) are contextually
  equivalent, written \( [[ ef1 =ctx ef2 ]] \), if there does not exist a context
  that can distinguish them. That is, $[[ef1]]$ and $[[ef2]]$ behave identically
  in all contexts.
\end{definition}

Here, we understand a context to be a core expression with a hole, similar to an
expression wrapper, which instantiates the free variables of the expression that
gets filled in.
More concretely, the expression built by inserting $[[ef1]]$ and $[[ef2]]$
to the context should either both evaluate to the same value, or both diverge.
A formal definition of contextual equivalence can be found in \pref{app:ctx_equiv}.

\subsection{Properties}

\begin{table}[]
  \input{tex/figures/PropTable.mng}
  \caption{Property Overview}
  \label{tab:prop}
\end{table}

\paragraph{$[[let]]$-inlining and extraction}
We begin by analysing Similarity 1, which expands to the three properties described
in this subsection.

\renewcommand\elab[1]{}
\begin{property}{1}[Let Inlining is Type Preserving]\
  \begin{shortItemize}
  \item \( [[ G |-E let x = ee1 in ee2 => ne ~> ef ]]~\then[[ G |-E [ ee1 / x ] ee2 => ne ~> ef ]] \)
  \item \( [[ G |-E let x = ee1 in ee2 <= s ~> ef ]]~\then[[ G |-E [ ee1 / x ] ee2 <= s ~> ef ]] \)
  \end{shortItemize}
  \label{prop:let_inlining}
\end{property}

\renewcommand\elab[1]{}
\begin{property}{2}[Let Extraction is Type Preserving]\
  \begin{shortItemize}
  \item \( [[ G |-E [ ee1 / x ] ee2 => ne2 ~> ef ]]~\band~[[ G |-E ee1 => ne1 ~> ef1 ]] \\
    \then[[ G |-E let x = ee1 in ee2 => ne2 ~> ef ]] \)
  \item \( [[ G |-E [ ee1 / x ] ee2 <= s2 ~> ef ]]~\band~[[ G |-E ee1 => ne1 ~> ef1 ]] \\
    \then[[ G |-E let x = ee1 in ee2 <= s2 ~> ef ]] \)
  \end{shortItemize}
  \label{prop:let_extraction}
\end{property}

\renewcommand\elab[1]{#1}
\begin{property}{3}[Let Inlining is Runtime Semantics Preserving]\
  \begin{shortItemize}
  \item \( [[ G |-E let x = ee1 in ee2 => ne ~> ef1 ]] \\
    \band~[[ G |-E [ ee1 / x ] ee2 => ne ~> ef2 ]]~\then[[ ef1 =ctx ef2 ]] \)
  \item \( [[ G |-E let x = ee1 in ee2 <= s ~> ef1 ]] \\
    \band~[[ G |-E [ ee1 / x ] ee2 <= s ~> ef2 ]]~\then[[ ef1 =ctx ef2 ]] \)
  \end{shortItemize}
  \label{prop:let_inlining_dyn}
\end{property}

As an example for why Property~\ref{prop:let_extraction} does not hold under
eager instantiation, consider \([[ id @Int ]]\).
Extracting the \([[id]]\) function into a new $[[let]]$-binder fails to type check, because
\([[id]]\) will be instantiated and then re-generalised. This means that explicit type instantiation
can no longer work on the extracted definition. % We discuss this further in Section~\ref{sec:expl_type}.

The runtime semantics properties (both these and later ones)
struggle under deep instantiation. This is demonstrated by
Example~5, |swizzle|, where we see that non-prenex quantification can cause $\eta$-expansion
during elaboration and thus change runtime semantics.

\paragraph{Signature Property}
Similarity 2 gives rise to these properties about signatures.

\renewcommand\elab[1]{}
\begin{property}{4}[Signature Property is Type Preserving]\ \\
  \( [[ G |-E </ x psi = eei // i /> => G' ~> x : s = ef ]]~\band~[[ x : s \in G' ]] \\
  \then[[ G |-E x : s ; </ x psi = eei // i /> => G' ~> x : s = ef ]] \)
  \label{prop:signature_type}
\end{property}

As an example of how this goes wrong under eager instantiation, consider the definition
\( [[ x = /\ a . \ y . ( y : a ) ]] \).
Annotating \([[x]]\) with its inferred type
\( [[ forall ia . a -> a ]] \) is rejected,
because \rref{Tm-CheckTyAbs} requires a \emph{specified} quantified variable,
not an \emph{inferred} one.

However, similarly to eager evaluation, even lazy instantiation needs to instantiate the types at some point.
In order to type a multi-equation declaration, a single type needs to be constructed that subsumes the types of every branch.
In our type system, \rref{Decl-NoAnnMulti} simplifies this process by first
instantiating every branch type (following the example set by GHC),
thus breaking Property~\ref{prop:signature_type}.
We thus introduce a simplified version of this property, limited to single equation declarations.
This raises a possible avenue of future work: parameterising the type system over the handling of multi-equation declarations.

\begin{property}{4b}[Signature Property is Type Preserving (Single Equation)]\ \\
  \( [[ G |-E x ps = ee => G' ~> x : s = ef ]]~\band~[[ x : s \in G' ]]~\then[[ G |-E x : s ; x ps = ee => G' ~> x : s = ef ]] \)
  \label{prop:signature_type_single}
\end{property}

\renewcommand\elab[1]{#1}
\begin{property}{5}[Signature Property is Runtime Semantics Preserving]\ \\
  \( [[ G |-E </ x psi = eei // i /> => G' ~> x : s = ef1 ]] \\
  \band~[[ G |-E x : s ; </ x psi = eei // i /> => G' ~> x : s = ef2 ]]~\then~[[ ef1 =ctx ef2 ]] \)
  \label{prop:signature_dyn}
\end{property}

\paragraph{Type Signatures}
Similarity 3 gives rise to the following property about runtime semantics.

\renewcommand\elab[1]{#1}
\begin{property}{6}[Type Signatures are Runtime Semantics Preserving]\ \\
  \( [[ G |-E x : s1 ; </ x psi = eei // i /> => G1 ~> x : s1 = ef1 ]] \\
  \band~[[ G |-E x : s2 ; </ x psi = eei // i /> => G1 ~> x : s2 = ef2 ]] \\
  \where~[[ G |- s1 inst _ d r ~> ewf1 ]]~\band~[[ G |- s2 inst _ d r ~> ewf2 ]] \\
  \then~[[ ewf1 [ ef1 ] =ctx ewf2 [ ef2 ] ]] \)
  \label{prop:type_sig}
\end{property}

Consider \([[ let  x : forall a . Int -> a -> a ; x = undefined in x ` seq ` () ]]\),
which diverges. Yet under deep instantiation, this version terminates:
\([[ let x : Int -> forall a . a -> a ; x = undefined in x ` seq ` () ]]\).
Under shallow instantiation, the second program is rejected, because \([[ undefined ]]\)
cannot be instantiated to the type \([[ Int -> forall a . a -> a ]]\), as that would be
impredicative. You can find the typing rules for \([[undefined]]\) and \([[seq]]\) in \pref{app:elab}.

\paragraph{Pattern Inlining and Extraction}
The properties in this section come from Similarity 4. Like in that similarity, we assume
that the patterns are just variables (either implicit type variables or explicit term variables).

\renewcommand\elab[1]{}
\begin{property}{7}[Pattern Inlining is Type Preserving]\ \\
  \( [[ G |-E x ps = ee1 => G' ~> x : s = ef1 ]]~\band~[[ wrap ( ps ; ee1 ~ ee2 ) ]]~\then~[[ G |-E x = ee2 => G' ~> x : s = ef2 ]] \)
  \label{prop:pat_inlining_typ}
\end{property}

The failure of pattern inlining under eager instantiation will feel similar:
if we take \( [[ id @ a {,} x = x : a ]] \),
we will infer a type \( [[ forall a . a -> a ]] \).
Yet if we write \( [[ id = /\ a . \ x . ( x : a ) ]] \), then eager
instantiation will give us the different type \( [[ forall ia . a -> a ]] \).

\renewcommand\elab[1]{#1}
\begin{property}{8}[Pattern Inlining / Extraction is Runtime Semantics Preserving]\ \\
  \( [[ G |-E x ps = ee1 => G' ~> x : s = ef1 ]]~\band~[[ wrap ( ps ; ee1 ~ ee2 ) ]] \\
  \band~[[ G |-E x = ee2 => G' ~> x : s = ef2 ]]~\then~[[ ef1 =ctx ef2 ]] \)
  \label{prop:pat_inlining_dyn}
\end{property}

\renewcommand\elab[1]{}
\begin{property}{9}[Pattern Extraction is Type Preserving]\ \\
  \( [[ G |-E x = ee2 => G' ~> x : s = ef2 ]]~\band~[[ wrap ( ps ; ee1 ~ ee2 ) ]]~\then~[[ G |-E x ps = ee1 => G' ~> x : s = ef1 ]] \)
  \label{prop:pat_extraction_typ}
\end{property}

\paragraph{Single vs.~multiple equations}

Similarity 5 says that there should be no observable change between the
case for a single equation and multiple (redundant) equations with the same right-hand side. That gets
formulated into the following property.

\renewcommand\elab[1]{}
\begin{property}{10}[Single/multiple Equations is Type Preserving]\ \\
  \( [[ G |-E x ps = ee => G , x : s ~> x : s = ef ]]~\then~[[ G |-E x ps = ee, x ps = ee => G' ~> x : s = ef]] \)
\label{prop:single_multi}
\end{property}

This property favours the otherwise-unloved eager flavour.
Imagine |f _ = pair|.
Under eager instantiation, this definition is accepted as type synthesis
produces an instantiated type.
Yet if we simply duplicate this equation under lazy instantiation
(realistic scenarios would vary the patterns on the left-hand side, but duplication
is simpler to state and addresses the property we want),
then \rref{Decl-NoAnnMulti} will reject as it requires the type to be instantiated.

\paragraph{$\eta$-expansion}

Similarity 6 leads to the following property.

\renewcommand\elab[1]{}
\begin{property}{11}[$\eta$-expansion is Type Preserving]\ 
\begin{shortItemize}
\item  \( [[ G |-E ee => ne ~> ef]]~\where~\mathit{numargs}([[ne]]) = n ~\then~[[ G |-E \ xsn . ee xsn => ne ~> ef]] \)
\item  \( [[ G |-E ee <= s ~> ef]]~\where~\mathit{numargs}([[r]]) = n ~\then~[[ G |-E \ xsn . ee xsn <= s ~> ef]] \)
\end{shortItemize}
\label{prop:eta}
\end{property}

Here, \([[ xsn ]]\) represents \(n\) variables.
We use $\mathit{numargs}([[s]])$ to count the number of explicit arguments an expression
can take, possibly instantiating any intervening implicit arguments.
A formal definition can be found in Figure~\ref{fig:numargs} in the appendix.
However, in synthesis mode this property fails for every flavour: \([[ne]]\) might be a function type \([[s1 -> s2]]\) taking a type scheme \([[s1]]\) as an argument, while we only synthesise monotype arguments.
We thus introduce a restricted version of Property~\ref{prop:eta}, with the additional premise that \([[ne]]\) can not contain any binders to the left of an arrow.

\begin{property}{11b}[$\eta$-expansion is Type Preserving (Monotype Restriction)]\ 
\begin{shortItemize}
\item  \( [[ G |-E ee => ne ~> ef]]~\where~\mathit{numargs}([[ne]]) = n ~\band~[[ G |- ne inst _ d t ~> ewf ]] \\
  \then~[[ G |-E \ xsn . ee xsn => ne ~> ef]] \)
\item  \( [[ G |-E ee <= s ~> ef]]~\where~\mathit{numargs}([[r]]) = n ~\then~[[ G |-E \ xsn . ee xsn <= s ~> ef]] \)
\end{shortItemize}
\label{prop:eta_restr}
\end{property}

This (restricted) property fails for all
but the eager/deep flavour as $\eta$-expansion forces other flavours to instantiate
arguments they otherwise would not have.

%% \subsection{Explicit Type Instantiation}
%% \label{sec:expl_type}

%% The stability properties discussed above predominantly favour lazy instantiation,
%% which is at least partly due to the presence of explicit type instantiation.
%% Limiting the language to implicit type instantiation only implies that
%% Property~\ref{prop:let_extraction} holds under eager instantiation as well.
%% The reason is that while instantiation prevents any explicit type application
%% afterwards, re-generalised types can still be implicitly instantiated.
%% Furthermore, as the distinction between inferred and specified types becomes
%% irrelevant, Properties~\ref{prop:signature_type_single}, \ref{prop:pat_inlining_typ}
%% and~\ref{prop:pat_extraction_typ} now also hold under eager instantiation.

%% Note that the opposite holds true as well: discussing the compile time semantics
%% stability for a language with only explicit type instantiation is uninteresting
%% as all compile time properties discussed above trivially hold.

\subsection{Conclusion}

A brief inspection of Table~\ref{tab:prop} suggests how we should proceed: choose
\emph{lazy}, \emph{shallow} instantiation. While this configuration does not
respect all properties, it is the clear winner---even more so when we consider
that Property~\ref{prop:eta_restr} (one of only two that favour another mode)
must be artificially restricted in order for any of our flavours to support
the property.

We should note here that we authors were surprised by this result. This paper arose
from the practical challenge of designing instantiation in GHC. After considerable
debate among the authors of GHC, we were unable to remain comfortable with any
one decision---as we see here, no choice is perfect, and so any suggestion was
met with counter-examples showing how that suggestion was incorrect. Yet we had
a hunch that eager instantiation was the right design. We thus formulated the
similarities of \pref{sec:stability} and went about building a formalisation
and proving properties. Crucially, we did \emph{not} select the similarities
to favour a particular result, though we did choose to avoid reasonable similarities
that would not show any difference between instantiation flavours.
At an early stage of this work, we continued to
believe that eager
instantiation was superior. It was only through careful analysis, guided by our
proofs and counter-examples, that we realised that lazy instantiation was winning.
We are now convinced by our own analysis.





==> tex/sections/MixedCalc.tex <==
%if style == newcode
\begin{code}
module Calculus where
\end{code}
%endif

% no elaboration here
\renewcommand\elab[1]{}
% explicit type application here
\renewcommand\invisTyApp[1]{#1}

\section{The Mixed Polymorphic $\lambda$-Calculus}
\label{sec:calculus}

\begin{figure*}
  \input{tex/figures/Syntax.mng}
  \caption{Mixed Polymorphic $\lambda$-Calculus (MPLC) Syntax}
  \label{fig:Syntax}
\end{figure*}

In order to assess the stability of our different designs, this section develops a 
polymorphic, stratified $\lambda$-calculus with both implicit and
explicit polymorphism. We call it the Mixed Polymorphic $\lambda$-calculus,
or MPLC.
Our formalisation (based on \citet{visible-type-application} and \citet{quick-look})
features explicit type instantiation and abstraction,
as well as type variable specificity. In order to support
visible type application, even when instantiating eagerly, we
must consider all the arguments to a function before doing our instantiation,
lest some arguments be type arguments.
Furthermore, type signatures are allowed in the calculus, and
the bidirectional type system~\cite{local-type-inference}
permits higher-rank~\cite{odersky-laufer} functions. Some other features,
such as local $[[let]]$ declarations defining functions with multiple equations,
are added to support some of the similarities we wish to study.

We have built this system to support flexibility in both of our
axes of instantiation scheme design. That is, the calculus is parameterised
over choices of instantiation depth and eagerness. In this way, our
calculus is essentially a \emph{family} of type systems: choose your
design, and you can instantiate our rules accordingly.

\subsection{Syntax}

The syntax for MPLC is shown in Figure~\ref{fig:Syntax}.
We define two meta parameters $[[d]]$ and $[[ep]]$ denoting the depth and
eagerness of instantiation respectively. In the remainder of this paper, grammar
and relations which are affected by one of these parameters will be annotated as
such. A good example of this are types $[[qd]]$ and $[[ne]]$, as
explained below. 

\renewcommand\elab[1]{}
Keeping all the moving pieces straight can be challenging. We thus offer
some mnemonics to help the reader:
In the remainder of the paper, aspects pertaining to
\textbf{e}ager instantiation are highlighted in \instE{\textbf{e}merald}, while 
\textbf{l}azy features are highlighted in \instL{\textbf{l}avender}.
Similarly, instantiation under the \textbf{s}hallow scheme is drawn using a
\textbf{s}triped line, as in $[[ G |- s instS _ S r ~> ewf ]]$.

\paragraph{Types}
Our presentation of the MPLC contains several different type categories,
used to constrain type inference.
%% which we explain here. %% These categories are introduced to support
%% the different instantiation schemes discussed in this paper, altering the
%% behaviour of the typing rules accordingly.
Monotypes $[[t]]$ represent simple ground types without any polymorphism, %%  They
%% are entirely standard, incorporating type variables $[[a]]$,
%% functions $[[t1 -> t2]]$ and saturated type constructors $[[T ts]]$\footnote{We
%% work only with saturated type constructors, as we wish to avoid complications
%% arising from a kind system. Such concerns would be orthogonal to our main object
%% of study: instantiation.}.
while type schemes $[[s]]$ can be
polymorphic, including under arrows.
In contrast, instantiated types $[[r]]$
cannot have any top-level polymorphism.
However, depending on the depth $[[d]]$ of instantiation, 
a $[[r]]$-type may or may not feature nested foralls on the right
of function arrows. This dependency on the depth $[[d]]$ of type
instantiation is denoted using an instantiated result type $[[qd]]$
on the right of the function
arrow. Instantiating shallowly, $[[q_S]]$ is a type scheme $[[s]]$,
but deep instantiation sees $[[q_D]]$ as an instantiated type $[[r]]$.
This makes sense: $[[Int -> forall a. a -> a]]$ \emph{is} a fully instantiated
type under shallow instantiation, but not under deep.
%% No matter the instantiation flavour,
%% function arguments within an instantiated type $[[r]]$
%% can still be polymorphic, as instantiating a function does not
%% affect polymorphism to the left of an arrow.
We also have synthesised types $[[ne]]$ to denote the output of the type synthesis
judgement $[[G |-E ee => ne ~> ef]]$, which infers a type from an expression. The
shape of this
type depends on the eagerness $[[ep]]$ of type instantiation: under lazy
instantiation ($[[L]]$), inference can produce full type schemes $[[s]]$; but
under eager instantiation ($[[E]]$), synthesised types $[[ne]]$ are always
instantiated types $[[r]]$:
any top-level quantified variable would have been instantiated away.

Finally, an argument descriptor $[[psig]]$ represents a type synthesised from
analysing a function argument pattern.
Descriptors are assembled
into type schemes $[[s]]$ with the $[[type (psigs; s0 ~ s ) ]]$ judgement,
in Figure~\ref{fig:InstSkol}.

\paragraph{Expressions}
Expressions $[[ee]]$ are mostly standard; we explain the less common forms here.

As inspired by \citet{quick-look}, applications are modelled as applying a head
$[[h]]$ to a (maximally long) list of arguments $[[args]]$.
The main idea is that under eager instantiation, type instantiation
for the head is postponed until it has been applied to its arguments.
A head $[[h]]$ is thus defined to be either a variable $[[x]]$, a data
constructor $[[K]]$, an annotated expression $[[ee : s]]$ or a simple expression
$[[ee]]$. This last form will not be typed with a type scheme under eager
instantiation---that is, we will not be able to use explicit instantiation---but
is required to enable application of a lambda expression.
As we feature both term and type application, an argument $[[arg]]$ is defined to
be either an expression $[[ee]]$ or a type argument $[[ @ s ]]$.

Our syntax additionally includes explicit abstractions over type variables,
written with $[[ /\ ]]$. Though the design of this feature (inspired by
\citet[Appendix B]{type-variables-in-patterns})
is straightforward
in our system, its inclusion drives some of the challenge of maintaining
stability.

Lastly, $[[let]]$-expressions are modelled on the syntax of Haskell.
These contain a single (non-recursive) declaration
$[[edecl]]$, which may optionally have a type signature $[[x : s]]$, followed by
the definition $[[</ x psi = eei // i />]]$. 
The patterns $[[ps]]$ on the left of the equals sign can each be either a simple
variable $[[x]]$, type $[[ @ s ]]$ or a saturated data constructor $[[K ps]]$.

\paragraph{Contexts}
Typing contexts $[[G]]$ are entirely standard, storing both the term variables
$[[x]]$ with their types and the type variables $[[a]]$ in scope; these type
variables may appear in both terms (as the calculus features explicit type application)
and types. The type constructors and
data constructors are stored in a static context $[[Sig]]$, which
forms the basis of typing contexts $[[G]]$.
This static context contains the data type definitions by storing both type
constructors $[[T as]]$ and data constructors $[[K : as ; ss ; T]]$. Data
constructor types contain the list of quantified variables $[[as]]$, the argument
types $[[ss]]$, and the resulting type $[[T]]$; when $[[K : as ; ss ; T]]$, then
the use of $[[K]]$ in an expression would have type $[[forall as. ss -> T as]]$, abusing
syntax slightly to write a list of types $[[ss]]$ to the left of an arrow.

\subsection{Type system overview}
\label{sec:basic_typing}

\begin{figure}
  \input{tex/figures/TermTyping.mng}
  \caption{Term Typing for Mixed Polymorphic $\lambda$-Calculus}
  \label{fig:TermTyping}
\end{figure}

\begin{figure}
  \input{tex/figures/DeclTyping.mng}
  \caption{Declaration Typing for Mixed Polymorphic $\lambda$-Calculus}
  \label{fig:DeclTyping}
\end{figure}

\begin{figure}
  \input{tex/figures/PatternTyping.mng}
  \caption{Pattern Typing for Mixed Polymorphic $\lambda$-Calculus}
  \label{fig:PatternTyping}
\end{figure}

\begin{figure}
  \input{tex/figures/InstSkol.mng}
  \caption{Type Instantiation and Skolemisation}
  \label{fig:InstSkol}
\end{figure}

\begin{table}[]
  \input{tex/figures/RelationTable.mng}
  \caption{Relation Overview}
  \label{tab:rel}
\end{table}

Table~\ref{tab:rel} provides a high-level overview of the different
typing judgements for the MPLC.
The detailed rules can be found in
Figures~\ref{fig:TermTyping}--\ref{fig:InstSkol}. The starting place to understand our rules
is in Figure~\ref{fig:TermTyping}. These judgements implement a bidirectional type system,
fairly standard with the exception of their treatment of a list of arguments all at
once\footnote{This is a well-known technique to reduce the number of traversals
through the applications, known as \emph{spine form}~\cite{spine}.}.

Understanding this aspect of the system hinges on \rref{Tm-InfApp}, which synthesises
the type of the head $[[h]]$ and uses its type to check the arguments $[[args]]$.
The argument-checking judgement $[[G |-A args <= s => s' ~> fargs]]$ (inspired by
\citet{simple-bidirectional})
uses the function's
type $[[s]]$ to learn what type is expected of each argument; after checking all arguments,
the judgement produces a residual type $[[s']]$. The judgement's rules walk down the list,
checking term arguments (\rref{Arg-App}), implicitly instantiating specified variables
where necessary (\rref{Arg-Inst}, which spots a term-level argument $[[ee]]$ but does
not consume it), uses type arguments for instantiation (\rref{Arg-TyApp}), and
eagerly instantiates inferred type arguments (\rref{Arg-InfInst}).

%% When synthesising a type for an explicit type abstraction \( [[ /\ a . ee ]] \)
%% (\rref{Tm-InfTyAbs}), the expression \( [[ ee ]] \) is typed under an
%% extended environment, and the resulting forall type is instantiated under eager
%% instantiation. Type checking (\rref{Tm-CheckTyAbs}) skolemises any top level
%% inferred binders, and recursively checks \( [[ee]] \) under an extended environment.

Our type system also includes $[[let]]$-declarations, which allow for the definition
of functions, with or without type signatures, and supporting multiple equations defined
by pattern-matching. Checking declarations and dealing with patterns is accomplished
by the judgements in Figures~\ref{fig:DeclTyping} and~\ref{fig:PatternTyping}, respectively,
although
the details may be skipped on a first reading: we include these rules for completeness
and as the basis of our stability-oriented evaluation (Section~\ref{sec:evaluation}).
These rules do not directly offer insight into our treatment of instantiation.

Instead, the interesting aspects of our formulation are in the instantiation
and skolemisation judgements.

%% \paragraph{Type Synthesis}
%% Synthesis for expressions is performed by the $[[ G |-E ee => ne ~> ef ]]$ relation: ``Under typing
%% context $[[G]]$, the expression $[[ee]]$ is assigned the type $[[ne]]$''.
%% As mentioned previously, the shape of the output type $[[ne]]$ is parameterised over the
%% eagerness of type instantiation $[[ep]]$. Under lazy instantiation, type
%% synthesis produces a type scheme $[[s]]$; under eager instantiation, the
%% output will be an instantiated type $[[r]]$.

%% Similar to expressions, type synthesis for heads $[[ G |-H h => s ~> ef ]]$ reads:
%% ``Under typing context $[[G]]$, the head $[[h]]$ is assigned the type $[[s]]$''.
%% Pattern synthesis is performed by the $[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]$ relation:
%% ``Under typing context $[[G]]$, patterns $[[ps]]$ are assigned the argument descriptors $[[psigs]]$,
%% producing the context extension $[[Del]]$''.
%% Finally, declaration synthesis is performed by the $[[ G |-E edecl => G' ~> x : s = ef ]]$ relation:
%% ``The declaration $[[ edecl ]]$ extends the typing context $[[G]]$ into $[[G']]$''.

%% \paragraph{Type Checking}
%% Checking for expressions is performed by the $[[ G |-E ee <= s ~> ef ]]$ relation: ``Under typing context
%% $[[G]]$, the expression $[[ee]]$ is checked to have the type $[[s]]$''.
%% The type serves as an input here: an algorithmic interpretation of this relation
%% would simply return a pass/fail result.
%% Similarly, pattern checking is performed by the $[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]$ relation:
%% ``Under typing context $[[G]]$, patterns $[[ps]]$ match element-wise against $[[s]]$, producing the residual type $[[s']]$ and the context extension $[[Del]]$''.
%% Argument type checking $[[ G |-A args <= s => s' ~> fargs ]]$ bears a close resemblance
%% to pattern checking, taking a typing context $[[G]]$, a list of arguments
%% $[[args]]$ and a type scheme $[[s]]$ and producing a residual type $[[s']]$.
%% Concretely, this means that bound type variables in the given type are instantiated
%% (\rref{Arg-Inst}) and the list of arguments are type checked to have the given type.

\subsection{Instantiation and Skolemisation}
\renewcommand\elab[1]{}
When we are type-checking the application of a polymorphic function,
we must \emph{instantiate} its
type variables: this changes a function |id :: forall a. a -> a| into |id :: tau -> tau|,
where |tau| is any monotype. On the other hand, when we are type-checking
the body of a polymorphic definition, we must \emph{skolemise} its type
variables: this changes a definition |(\x -> x) :: forall a. a -> a| so that we
assign |x| to have type |a|, where |a| is a \emph{skolem constant}---a fresh
type, unequal to any other. These constants are bound in the context returned
from the skolemisation judgement.

Naturally, the behaviour of both instantiation and skolemisation depend on the
instantiation depth; see Figure~\ref{fig:InstSkol}.
Both \rref{Inst-Inst} and \rref{Skol-Skol} use the $[[ebinders]]$ helper function:
$[[ ebinders_d(s) = as;r]]$ extracts out bound type variables $[[as]]$ and a residual type $[[r]]$
from a polytype $[[s]]$. The depth, though, is key: the shallow ($[[S]]$) version
of our type system, $[[ebinders]]$ gathers only type variables bound at the top,
while the deep ($[[D]]$) version looks to the right past arrows. As examples, we
have $[[ebinders_S(forall a. a -> forall b. b -> b) = a; a -> forall b. b -> b]]$
and $[[ebinders_D(forall a. a -> forall b. b -> b) = a,b; a -> b -> b]]$. The full
definition (inspired by \citet[Section~4.6.2]{practical-type-inference})
is in Appendix~\ref{app:addrel}.

%% The relations gather the binders of $[[s]]$ and instantiates or skolemises these with
%% monotypes $[[ts]]$ or fresh type variables, respectively.
%% Using $[[ ebinders ]]$ (see Appendix~\ref{app:elab}), these binders encompass
%% either the type variables bound at the top of the type scheme (under
%% shallow instantiation), or variables bound both at the top level and on the
%% right of function arrows (under deep instantiation, based directly on
%% relations in \citet[Section~4.6.2]{practical-type-inference}).

Some usages of these relations happen only for certain choices of instantiation
flavour. For example, see \rref{Tm-InfApp}. We see the last premise instantiates
the result of the application---but its \instE{emerald} colour tells us that this
instantiation happens only under the eager flavour\footnote{We can also spot this
fact by examining the metavariables. Instantiation takes us from a $[[s]]$-type
to a $[[r]]$-type, but the result in \rref{Tm-InfApp} is a $[[ne]]$-type: a
$[[r]]$-type in the eager flavour, but a $[[s]]$-type in the lazy flavour.}.
Indeed, this particular use of
instantiation is the essence of eager instantiation: even after a function has
been applied to all of its arguments, the eager scheme continues to instantiate.
Similarly, \rref{Tm-InfTyAbs} instantiates eagerly in the eager flavour.

The \instL{lazy} counterpart to the eager instantiation in \rref{Tm-InfApp} is the
instantiation in \rref{Tm-CheckInf}. This rule is the catch-all case in the
checking judgement, and it is used when we are checking an application against an
expected type, as in the expression |f a b c :: T Int Bool|. In this example, if
|f a b c| still has a polymorphic type, then we will need to instantiate it in order
to check the type against the monomorphic |T Int Bool|. This extra instantiation
would always be redundant in the eager flavour (the application is instantiated
eagerly when inferring its type) but is vital in the lazy flavour.

%% The instantiation and skolemisation relations as presented here
%% are defined as going from a type scheme $[[s]]$ to an instantiated type $[[r]]$.
%% However, some rules relate other types.
%% Consider $[[ instE ( G |- s inst _ d ne ~> ewf ) ]]$ (e.g. \rref{Tm-InfApp}):
%% as a synthesised type $[[ne]]$ \emph{is} a type scheme when we work with lazy
%% instantiation, this instantiation is actually a no-op in that scenario;
%% however, under eager instantiation, a synthesised type is the same as an
%% instantiated type (with no $[[forall]]$s at the top), and we must actually
%% instantiate. We colour this instantiation in \instE{emerald}.
%% Conversely, $[[ instL ( G |- ne inst _ d r ~> ewf ) ]]$ (e.g. \rref{Tm-CheckInf})
%% applies only under the lazy scheme, and is thus coloured in \instL{lavender}.

%% \gertjan{If needed, we can dramatically shorten the next paragraph, as the typing rules are repeated in the next sections}
%% The instantiation and skolemisation relations as presented here
%% are defined as going from a type scheme $[[s]]$ to an instantiated type $[[r]]$.
%% However, we see some rules relate other types.
%% For example, \rref{Tm-InfApp} instantiates
%% the type scheme $[[s']]$ inferred for the head $[[h]]$ to a synthesised type
%% $[[ne]]$ (the $[[ep]]$ is included to remind us on the importance of the eagerness parameter).
%% Because a synthesised type \emph{is} a type scheme when we work with lazy instantiation,
%% this instantiation in \rref{Tm-InfApp} is actually a no-op in that scenario;
%% however, under eager instantiation,
%% a synthesised type is the same as an instantiated type (with no $[[forall]]$s at the top),
%% and we must actually instantiate. This is why the use of instantiation in \rref{Tm-InfApp} is
%% coloured in \instE{emerald}. Conversely, examine \rref{Tm-CheckInf}.
%% This rule handles the case when no other rule matches under checking mode,
%% by typing the expression in synthesis mode.
%% If we have instantiated eagerly, then no further action is required and the
%% synthesised type $[[ne]]$ should correspond to--the skolemised version of--the
%% type $[[r]]$ we are checking against.
%% Under lazy instantiation, however, type synthesis might produce a type scheme,
%% which now needs to be instantiated to compare against the skolemised type $[[r]]$.
%% Recall that, under eager instantiation, a synthesised type $[[ne]]$ is
%% \emph{already} an instantiated type $[[r]]$, and then this instantiation is a
%% no-op. The instantiation applies only under the lazy scheme, and
%% thus is coloured in \instL{lavender}.

%% \paragraph{Data constructors}
%% Typing a data constructor (\rref{H-Con}) works identically to typing variables
%% (entirely standard; \rref{H-Var}),
%% after assembling the data constructor type from its pieces.

Several other rules interact with instantiation in interesting ways:

\paragraph{$\lambda$-expressions}
\Rref{Tm-CheckAbs} checks a $\lambda$-expression
against an expected type $[[s]]$. However, this expected type may be a polytype.
We thus must first skolemise it, revealing a function type $[[ s1 -> s2 ]]$
underneath (if this is not possible, type checking fails).
%% Skolemisation takes the available binders of $[[s]]$ and simply adds them to the
%% context $[[G']]$.
%% These variables behave as skolem constants when checking $[[ee]]$.
In order to support explicit type abstraction inside a lambda binder
\( [[ \ x . /\ a . ee ]] \), \rref{Tm-CheckAbs}
never skolemises under an arrow: note the fixed $[[S]]$ visible in the rule.
As an example, this is necessary in order to accept |(\ x @b (y :: b) -> y) :: forall a. a -> forall b. b -> b|, where it would be disastrous to deeply skolemise the expected
type when examining the outer $\lambda$.

\paragraph{Declarations without a type annotation}
\Rref{Decl-NoAnnMulti} is used for synthesising a type for a multiple-equation
function definition that is not given a type signature. When we have multiple
equations for a function, we might imagine synthesising different polytypes for
each equation. We could then imagine trying to find some type that each equation's
type could instantiate to, while still retaining as much polymorphism as possible.
This would seem to be hard for users to predict, and hard for a compiler to
implement. Our type system here follows GHC in instantiating the types of all
equations to be a monotype, which is then re-generalised. This extra instantiation
is not necessary under eager instantiation, which is why it is coloured in \instL{lavender}.

For a single equation (\rref{Decl-NoAnnSingle}), synthesising the original polytype,
without instantiation and regeneralisation is straightforward, and so that is
what we do (also following GHC).

%% \paragraph{Application}
%% Let us examine \rref{Tm-InfApp} more closely, which synthesises the type
%% for applications $[[h args]]$.
%% First, the type of $[[h]]$ is synthesised, using the head synthesis relation.
%% This produces a type scheme, independently of the eagerness of instantiation.
%% The arguments $[[args]]$ are then checked under this type $[[s]]$, producing a
%% residual type $[[s']]$\footnote{The application judgement is inspired
%% by \citet{simple-bidirectional}.}. Finally, after the head has been applied to all its
%% arguments, the remaining type $[[s']]$ is instantiated (under eager
%% instantiation), producing a type $[[ne]]$ for the final expression.

%% Note that as applications are always typed in this fashion, head typing
%% needs only a synthesis mode, and argument typing needs to be defined only for
%% checking mode.
%% Argument checking under a function type (\rref{Arg-App}) only works for an
%% expression argument. Checking under a forall type instantiates the bound type
%% variable with the given argument type (\rref{Arg-TyApp}) or a freshly
%% generated type (\rref{Arg-Inst}). Similarly, checking under an inferred forall
%% type requires instantiating the type variable.

%% \paragraph{Mode Changing}
%% Going from type synthesis to type checking is achieved using an
%% annotation. Typing an annotated expression $[[ ee : s ]]$ (\rref{H-Ann})
%% works by checking the expression $[[ee]]$ under the given type $[[s]]$.
%% Note that under eager instantiation, the type for this annotated expression
%% gets instantiated instiated in \rref{Tm-InfApp}.

%% Going from checking to synthesis mode is also allowed (\rref{Tm-CheckInf}),
%% but only when \([[ee]]\) is not a lambda or let expression,
%% and thus when no other type checking rule would apply.
%% We first skolemise the given type $[[s]]$ to bind any new type variables in $[[G']]$.
%% We then infer a type for the expression $[[ee]]$ and match it against the skolemised type $[[r]]$.
%% Note that under lazy instantiation, the
%% synthesised type still needs to be instantiated in order to match $[[r]]$.




==> tex/sections/ModernHaskell.tex <==
%if style == newcode
\begin{code}
module ModernHaskell where
\end{code}
%endif

% explicit type application here
\renewcommand\invisTyApp[1]{#1}

\section{Mixing Implicit and Explicit Types}
\label{sec:modern}
\label{sec:last-system}

\begin{figure}
  \input{tex/figures/ModSyntax.mng}
  \input{tex/figures/ModTypingB.mng}
  \input{tex/figures/ModTypingG.mng}
  \input{tex/figures/ModTypingE.mng}
  \caption{The Mixed Polymorphic $\lambda$-calculus (Extension of Figures~\ref{fig:Ssyn}, \ref{fig:STmc}, \ref{fig:STmb}, and \ref{fig:Asyn})}
  \label{fig:Msyn}
\end{figure}

%% \begin{figure}
%%   \caption{Argument Type Checking for the Mixed Polymorphic $\lambda$-calculus (Extension of Figure~\ref{fig:Asyn})}
%%   \label{fig:MTmb}
%% \end{figure}
%% %% \begin{figure}
%% %%   \input{tex/figures/ModTypingC.mng}
%% %%   \caption{Declaration typing for Mixed Polymorphic System F}
%% %%   \label{fig:MTmc}
%% %% \end{figure}
%% \begin{figure}
%%   \caption{Expression Typing for the Mixed Polymorphic $\lambda$-calculus (Extension of Figure~\ref{fig:Asyn})}
%%   \label{fig:MTmg}
%% \end{figure}
%% \begin{figure}
%%   \caption{Pattern Typing for the Mixed Polymorphic $\lambda$-calculus (Extension of Figures~\ref{fig:STmc} and~\ref{fig:STmb})}
%%   \label{fig:MTme}
%% \end{figure}

Figure~\ref{fig:Msyn} shows the extension of the language syntax to handle mixed
implicit and explicit features. We call this extended system Mixed Polymorphic $\lambda$-calculus,
or MPLC. Our formalisation is based on \citet{visible-type-application} and \citet{quick-look},
and extends the IPLC with explicit
type instantiation and abstraction, along with type variable specificity.
Application arguments are extended with visible type
application arguments $[[ @ t ]]$, and both expressions and patterns are extended
with explicit type abstraction $[[ /\ a . ee ]]$ and $[[ @ t ]]$, respectively.
Type schemes $[[s]]$ now allow inferred variables $[[forall ias . s]]$.
Note, however, that the context $[[G]]$ does not differentiate between specified
and inferred variables, as the specificty of variables no longer has any impact
after skolemising.
Argument types $[[psig]]$ are extended with type
abstractions $[[ @ a ]]$, used in a function definition like $[[ f @a {,} x = (x : a) ]]$
and which corresponds to a polytype $[[ forall a . s ]]$ when assembled with $[[type]]$.
The $[[binders]]$ operation is updated to extract out inferred type variables;
and the declaration typing relation receives a minor update, marking generalised 
variables as inferred.
Both updated definitions can be found in Appendices~\ref{app:addrel}
and~\ref{app:systemf}, respectively.

\paragraph{Explicit Type Instantiation}
See \rref{Arg-TyApp}, which shows the
new argument type checking relation. The alternative formalisation of
the language presented in Section~\ref{sec:alt} reduces the introduction of
explicit type application---by all accounts a non-trivial language feature---to
the addition of a single typing rule. Note that inferred type variables
(as presented in Section~\ref{sec:specificity}), handled
in \rref{Arg-InfInst}, are unconditionally instantiated.

\paragraph{Explicit Type Abstraction}
The definition of patterns $[[p]]$ now includes type arguments $[[@t]]$,
and expressions $[[ee]]$ include type abstraction $[[ /\ a . ee ]]$.
Programmers can now
explicitly abstract over type variables in both lambda and let expressions.

%Figure~\ref{fig:MTmg} shows the new typing rules for type abstraction.
When synthesising a type for an explicit type abstraction \( [[ /\ a . ee ]] \)
(\rref{ETm-InfTyAbs}), the expression \( [[ ee ]] \) is typed under an
extended environment, and the resulting forall type is instantiated under eager
instantiation. Type checking (\rref{ETm-CheckTyAbs}) skolemises any top level
inferred binders, and recursively checks \( [[ee]] \) under an extended environment.
Note that in order to support explicit type abstraction inside a lambda binder
\( [[ \ x . /\ a . ee ]] \), \rref{ETm-CheckAbs} has been slightly altered to
never skolemise after the arrow (even under deep instantiation).

%Similarly, Figure~\ref{fig:MTme} presents the updated pattern typing rules.
Type abstraction $[[ @ a ]]$ in both synthesis and checking mode
(\rref{Pat-InfTyVar} and \rref{Pat-CheckTyVar} respectively) produces a
type argument descriptor $[[ @ a ]]$ and extends the typing environment.
In data constructor patterns (\rref{Pat-InfCon} and \rref{Pat-CheckCon}),
full type schemes $[[ss1]]$ are allowed in patterns, where they
are used to instantiate the variables \([[as0]]\)
(possibly extended with guessed monotypes \([[ts0]]\), if there are not enough $[[ss1]]$).
Consider, for example, $[[ f (Just @ Int {,} x ) = x + 1 ]]$,
where the $[[ @ Int ]]$ refines the type of $[[Just]]$, which in turn assigns
$[[ x ]]$ the type $[[ Int ]]$. Note that pattern checking allows skolemising
bound type variables (\rref{Pat-CheckInfForall}), but only when the patterns
are not empty in order not to lose syntax-directedness of the rules.
The same holds for \rref{Pat-CheckForall}, which only applies when no
other rules match.

%% \paragraph{User-Defined Provenance}
%% We allow programmers to manually write type variables and mark them as compiler
%% generated. In other words, this feature allows the programmer to specify which type
%% variables can be manually instantiated and which can not. This feature has
%% recently been implemented in GHC.
%% \gertjan{Is this the place to point to the addition of { a } in the rules?}
%% \gertjan{Explain that the basic system does not need this distinction, as it
%%   does not have explicit type instantiation.}



==> tex/sections/Named.tex <==
%if style == newcode
\begin{code}
module Named where
\end{code}
%endif

\section{Named Arguments}
\label{sec:named}

\begin{figure}[h!]
  \input{tex/figures/LabSyntax.mng}
  \caption{Syntax Extended with Named Type Variables}
  \label{fig:Lsyn}
\end{figure}

\begin{figure}[h!]
  \input{tex/figures/LabTyping.mng}
  \caption{Typing Rules for Named Type Variables}
  \label{fig:LTma}
\end{figure}
\begin{figure}[h!]
  \input{tex/figures/LabTypingB.mng}
  \caption{Typing Rules for Named Type Variables}
  \label{fig:LTmb}
\end{figure}


==> tex/sections/Proofs.tex <==
%if style == newcode
\begin{code}
module Proofs where
\end{code}
%endif

\section{Evaluation Reasonings}
\label{app:proofs}

This section provides the reasonings behind the analysis of
Section~\ref{sec:evaluation}, laying the groundwork for more formal proofs in the
future.

\paragraph{Property~\ref{prop:let_inlining}: Let Inlining is Type Preserving}\ \\
Repeated case analysis on the given derivation (\rref{ETm-InfLet} or
\rref{ETm-CheckLet}, followed by \rref{EDecl-NoAnnSingle}) results in
\( [[ G |-E x = ee1 => G , x : forall ias . ne1 ~> x : s = ef ]] \), 
\( [[ G |-E ee1  => ne1 ~> ef ]] \), and either
\( [[ G , x : forall ias . ne1 |-E ee2 => ne ~> ef ]] \) or
\( [[ G , x : forall ias . ne1 |-E ee2 <= r ~> ef ]] \).
It is not hard to see that the result follows from
this, as typing the variable \( [[ x ]] \) (through \rref{ETm-InfApp}) or the
expression \( [[ ee1 ]] \) directly, results in an identical typing.

\paragraph{Property~\ref{prop:let_extraction}: Let Extraction is Type Preserving}\ \\
Unlike Property~\ref{prop:let_inlining}, Property~\ref{prop:let_extraction} only
holds under lazy instantiation. The reason is that type inference under eager
instantiation, produces an instantiated type for \( [[ ee1 ]] \) before
generalising and placing it in the context. This means that while explicit type
application could be possible for \( [[ ee1 ]] \) directly, it gets rejected for
\( [[ x ]] \).

\paragraph{Property~\ref{prop:let_inlining_dyn}: Let Inlining is Dynamic Semantics Preserving}\ \\
Repeated case analysis on the first premise (\rref{ETm-InfLet} or
\rref{ETm-CheckLet}, followed by \rref{EDecl-NoAnnSingle}) tells us that
\( [[ ef1 = ( \ x : s . ef3 ) ef4 ]] \), where
\( [[ G |-E ee1 => ne1 ~> ef4 ]] \), \( [[ s =n forall ias . ne1 ]] \), and
\( [[ G , x : s |-E ee2 => ne ~> ef3 ]] \) or \( [[ G , x : s |-E ee2 <= r ~> ef3 ]] \).
Typing \( [[ ee2 ]] \) using the variable \( [[ x ]] \) (and substituting
afterwards) or using the inlined expression \( [[ ee1 ]] \) results in a
different translation.
When typing the variable directly, the type gets instantiated in
\rref{ETm-InfApp} (under eager instantiation) or \rref{ETm-CheckInf} (under
lazy instantiation). Under shallow instantiation, this results in additional type
applications to the translated expression, which are erased during evaluation.
Under deep instantiation, however, eta expansion is performed on the translated
expression, potentially altering the evaluation outcome.

\paragraph{Property~\ref{prop:let_extraction_dyn}: Let Extraction is Dynamic Semantics Preserving}\ \\
Analogous to Property~\ref{prop:let_inlining_dyn}.

\paragraph{Property~\ref{prop:signature_type}: Signature Property is Type Preserving}\ \\
Before proving Property~\ref{prop:signature_type}, we first introduce two helper
properties.

\begin{property}[Pattern Checking is Type Preserving]\ \\
  \( \mathit{If}~[[ G |-P ps => psigs ; Del ~> fps : fpsigs ]]~\mathit{then}~[[ G |-P ps <= s => s' ; Del ~> fps : fpsigs ]]~\mathit{where}~[[ type ( psigs ; s' ~ s ) ]] \)
  \label{prop:pattern_checking_type}
\end{property}

Property~\ref{prop:pattern_checking_type} follows by structural induction on the
pattern typing derivation.

\begin{property}[Expression Checking is Type Preserving]\ \\
  \( \mathit{If}~[[ G |-E ee => ne ~> ef ]]~\mathit{then}~[[ G |-E ee <= r ~> ewf [ ef ] ]]~\mathit{where}~[[ G |- ne inst _ d r ~> ewf ]] \)
  \label{prop:expr_checking_type}
\end{property}

Under lazy instantiation,
Properties~\ref{prop:signature_type} and~\ref{prop:expr_checking_type} are
proven straightforwardly through mutual induction, using
Property~\ref{prop:pattern_checking_type}.
Neither property holds under eager instantiation, however.
The problem lies in the explicit type abstraction case: \rref{ETm-InfTyAbs}
eagerly instantiates the type, which is then generalised in
\rref{EDecl-NoAnnMulti}, resulting in an inferred forall type. The expression
is not accepted by \rref{ETm-CheckTyAbs} under this same inferred type,
though. As the type gets skolemised, the inferred variable is placed in the
typing environment, but this does not match the specified type variable in
\rref{ETm-CheckTyAbs}.

\paragraph{Property~\ref{prop:signature_dyn}: Signature Property is Dynamic Semantics Preserving}\ \\
Similarly to Property~\ref{prop:signature_type}, we first introduce two helper
properties.

\begin{property}[Pattern Checking is Dynamic Semantics Preserving]\ \\
  \( \mathit{If}~[[ G |-P ps => psigs ; Del ~> fps1 : fpsigs1 ]]~\mathit{and}~[[ G |-P ps <= s => s' ; Del ~> fps2 : fpsigs2 ]]~\mathit{and}~[[ type ( psigs ; s' ~ s ) ]]~\mathit{then}~[[ fps1 = fps2 ]]~\mathit{and}~[[ fpsigs1 = fpsigs2 ]] \)
  \label{prop:pattern_checking_dyn}
\end{property}

Property~\ref{prop:pattern_checking_dyn} follows by structural induction on the
pattern typing derivation.

\begin{property}[Expression Checking is Dynamic Semantics Preserving]\ \\
  \( \mathit{If}~[[ G |-E ee => ne ~> ef1 ]]~\mathit{and}~[[ G |-E ee <= r ~> ef2 ]]~\mathit{and}~[[ G |- ne inst _ d r ~> ewf ]]~\mathit{then}~[[ ef1 =ctx ewf [ ef2 ] ]] \)
  \label{prop:expr_checking_dyn}
\end{property}

Under shallow instantiation, properties~\ref{prop:signature_dyn}
and~\ref{prop:expr_checking_dyn} are proven straightforwardly using mutual
induction. Note that while \rref{ETm-InfTyAbs} instantiates the type eagerly,
while \rref{ETm-CheckTyAbs} does not. Under shallow instantiation, this
results in additional type applications, which are erased during evaluation
(\rref{FEval-TyApp}).
However, under deep instantiation, neither property holds, as
\rref{ETm-InfTyAbs} performs eta expansion on the translated expression,
altering its behaviour.

\paragraph{Property~\ref{prop:type_sig}: Type Signatures are Dynamic Semantics Preserving}\ \\
Similarly to before, we first introduce a new helper property.

\begin{property}[Expression Signatures are Dynamic Semantics Preserving]\ \\
  \( \mathit{If}~[[ G |-E ee <= r1 ~> ef1 ]]~\mathit{and}~[[ G |-E ee <= r2 ~> ef2 ]]~\mathit{then}~[[ ef1 =ctx ef2 ]] \)
  \label{prop:expr_sig}
\end{property}

Under shallow instantiation, Properties~\ref{prop:type_sig}
and~\ref{prop:expr_sig} are proven through straightforwardly mutual induction.
Neither property holds under deep instantiation, though, as the skolemisation
step in \rref{EDecl-Ann} performs eta expansion on the translated expression,
altering its behaviour depending on the provided type signature. 

\paragraph{Property~\ref{prop:pat_inlining_typ}: Pattern Inlining is Type Preserving}\ \\
Case analysis on the given derivation (\rref{EDecl-NoAnnMulti}) tells us that
\( [[ </ G |-P psi => psigs ; Del ~> fpsi : fpsigs // i /> ]] \), 
\( [[ </ G , Del |-E eei1 => nei1 ~> efi1 // i /> ]] \),
\( [[ </ G , Del |- nei1 inst _ d r1 ~> ewfi1 // i /> ]] \) and
\( [[ type ( psigs ; r1 ~ s ) ]] \).
Proving the goal (\rref{EDecl-NoAnnMulti}) requires us to show
\( [[ </ G |-E eei2 => nei2 ~> efi2 // i /> ]] \) and
\( [[ </ G |- nei2 inst _ d r2 ~> ewfi2 // i /> ]] \), where
\( [[ s = r2 ]] \).
Under lazy instantiation, this results follows straightforwardly from
\rref{ETm-InfAbs} and \rref{ETm-InfTyAbs}, as the patterns have simply been
moved to the righthandside, and are typed in the exact same way.
However, under eager instantiation, this fails as \rref{ETm-InfTyAbs} performs
an additional instantiation. Concretely, this means that while explicit type
abstractions on the left hand side remain uninstantiated, they are instantiated
eagerly under a lambda binder.

\paragraph{Property~\ref{prop:pat_extraction_typ}: Pattern Extraction is Type Preserving}\ \\
Analogous to Property~\ref{prop:pat_inlining_typ}.

\paragraph{Property~\ref{prop:pat_inlining_dyn}: Pattern Inlining / Extraction is Dynamic Semantics Preserving}\ \\
Case analysis on both typing derivations (\rref{EDecl-NoAnnMulti}) tells us that

\noindent
\( [[ ef1 = case </ fpsi : fpsigs -> ewfi1 [ efi1 ] // i /> ]] \) and
\( [[ ef2 = case </ empty : empty -> ewfi2 [ efi2 ] // i /> ]] \), where
\( [[ </ G |-P psi => psigs ; Del ~> fpsi : fpsigs // i /> ]] \),
\( [[ </ G , Del |-E eei1 => nei1 ~> efi1 // i /> ]] \), and
\( [[ </ G |-E eei2 => nei2 ~> efi2 // i /> ]] \).
As we would expect, the patterns from \( [[ fpsi1 ]] \) have been
shifted into the expression \( [[ efi1 ]] \), resulting in \( [[ efi2 ]] \).
For expression variable patterns, the context equivalence follows trivially,
from the evaluation relations \rref{FMatch-Var} and \rref{FEval-AppAbs}.
Type variable patterns are a bit more involved, as they are eagerly instantiated
in a lambda binder (\rref{ETm-InfTyAbs}), but not inside of a declaration
(\rref{EDecl-NoAnnMulti}).
Under shallow instantiation, the goal follows through simple induction, as the
instantiation only results in additional type applications, which are erased
during evaluation. However, under deep instantiation, \rref{ETm-InfTyAbs}
results in an eta expansion of the translated expression, altering the dynamic
semantics in the process.


==> tex/sections/RelatedWork.tex <==
%if style == newcode
\begin{code}
module RelatedWork where
\end{code}
%endif

\section{Related Work}

The type systems in this paper build most directly from
\citet{practical-type-inference}, \citet{visible-type-application},
and \citet{quick-look}. Each of these papers adds new capabilities
to Haskell, and each also decreases the stability of the language.
While these papers do consider properties we would consider
to be components of stability, stability is not a key criterion in
those authors' evaluation. By contrast, our work focuses squarely
on stability as a believable proxy for the quality of the user experience.

Many other works on designing type inference algorithms also introduce
stability properties, but these properties exist among others---such as completeness---and
do not seem to guide the design of the algorithm. We do call out one
such work, that by \citet{cochis}, which revolves around implicit programming systems,
and describes a property they call \emph{stability}.
In the context of that work, stability is about
Haskell's class-instance selection mechanism: we would like the choice
of instance to remain stable under substitutions. That is, if |f :: C a => a -> Int|
is called at an argument of type |Maybe b| (for a type variable |b|), the instance
selected for |C (Maybe b)| should be the same as the one that would be selected if
|f| were called on an argument of type |Maybe Int|. After all |Maybe b| can be
substituted to become |Maybe Int|; perhaps a small change to the program would
indeed cause this substitution, and we would not want a change in runtime
behaviour. Accordingly, the stability property, as used by \citet{cochis}, is
what we would also call a stability property, but it is much narrower than
the definition we give the term.

In comparison to these other papers on type systems and
type inference, the angle of this paper is somewhat different: we are not introducing a
new language or type system feature, proving a language type safe, or proving an
inference algorithm sound and complete to its declarative specification. Instead, we
introduce the concept of \emph{stability} as a new metric for evaluating (new or
existing) type systems, and then apply this metric to a system
 featuring both implicit and explicit instantiation.
Because of this novel, and somewhat unconventional topic, we are unable
to find further related work.


==> tex/sections/Stability.tex <==
%if style == newcode
\begin{code}
module Stability where
\end{code}
%endif

\newcommand{\squeezed}[2]{\begin{tabular}{@@{}l@@{}}\multicolumn{1}{@@{}l@@{\;\;\;\;}}{#1}\\\multicolumn{1}{@@{\;\;\;\;}r@@{}}{#2}\end{tabular}}

\section{Stability}
\label{sec:stability}

We have described stability as a measure of how small trans\-for\-ma\-tions---call them
\emph{similarities}---in user-written code might drastically change the behaviour of a program.
This section lays out the specific similarities we will consider with
respect to our instantiation flavours.
There are naturally \emph{many} transformations one might think of applying
to a source program. We have chosen ones that relate best to instantiation; others
(e.g. does a function behave differently in curried form as opposed to uncurried form?)
do not distinguish among our flavours and are thus less interesting in our concrete
context.
We include examples demonstrating each of these, showing how instantiation can
become muddled.
While these examples are described in
terms of types inferred for definitions that have no top-level signature, many of
the examples can easily be adapted to include a signature.
After presenting our formal model of Haskell instantiation,
we check our instantiation flavours against
these similarities in Section~\ref{sec:evaluation}, with proofs in
Appendix~\ref{app:formalproofs}.

We must first define what we mean by the ``behaviour'' of a program.
We consider two different notions of behaviour, both the
\emph{compile time} semantics of a program (that is, whether the program is
accepted and what types are assigned to its variables)
and its \emph{runtime} semantics (that is, what the program executes to,
assuming it is still well typed). We write, for example,
$ \transBCR $ to denote a similarity that we expect to respect
both compile and runtime semantics, whereas $ \transBR $ is one that
we expect only to respect runtime semantics, but may change compile time
semantics.
Similarly, $ \transCR $ denotes a one-directional similarity that we expect to
respect both compile and runtime semantics.

\subsection*{Similarity 1: Let-Inlining and Extraction}

A key concern for us is around $[[let]]$-inlining and -extraction. That is,
if we bind an expression to a new variable and use that variable instead of
the original expression, does our program change meaning? Or if we inline
a definition, does our program change meaning? These notions are captured
in Similarity 1:\footnote{A language with a strict $[[let]]$ construct
will observe a runtime difference between a let binding and its expansion, but 
this similarity would still hold with respect to type-checking.}
\begin{equation*}
  [[ let x = ee1 in ee2 ]] \transBCR [[ [ ee1 / x ] ee2 ]] 
\end{equation*}

%% \begin{similarity}\label{sim:let}
%%   \[ [[ let x = ee1 in ee2 ]] \transBCR [[ [ ee1 / x ] ee2 ]] \]
%% \end{similarity}

\paragraph{Example 1: |myId|}

The Haskell standard library defines |id :: forall a. a -> a| as the identity function.
Suppose we made a synonym of this (using the implicit top-level |let| of Haskell files),
with the following:
%
\begin{code}
myId = id
\end{code}
%
Note that there is no type signature. Even in this simple example, our choice of instantiation
eagerness changes the type we infer:
%
\begin{center}
\begin{tabular}{l||l||l}
|myId| & eager & lazy \\ \hline
deep or shallow & |forall {a}. a -> a| & |forall a. a -> a| \\
\end{tabular}
\end{center}
%
Under eager instantiation, the mention of |id| is immediately instantiated, and thus
we must re-generalise in order to get a polymorphic type for |myId|. Generalising
always produces inferred variables, and so the inferred type for |myId| starts
with |forall {a}|, meaning that |myId| cannot be a drop-in replacement for |id|,
which might be used with explicit type instantiation. On the other hand, lazy
instantiation faithfully replicates the type of |id| and uses it as the type
of |myId|.

\paragraph{Example 2: |myPair|}

This problem gets even worse if the original function has a non-prenex type, like
our |pair|, above. Our definition is now:
%
\begin{code}
myPair = pair
\end{code}
%
With this example, both design axes around instantiation matter:
\begin{center}
\begin{tabular}{l||l||l}
|myPair| & eager & lazy \\ \hline
deep & |forall {a} {b}. a -> b -> (a, b)| & \squeezed{|forall a. a ->|}{|forall b. b -> (a, b)|} \\
shallow & |forall {a}. a -> forall b. b -> (a, b)| & \squeezed{|forall a. a ->|}{|forall b. b -> (a, b)|} \\
\end{tabular}
\end{center}
%
All we want is to define a simple synonym, and yet reasoning about the types requires us to
consider both depth and eagerness of instantiation.

\paragraph{Example 3: |myPairX|}

The |myPairX| example above acquires a new entanglement once we account for specificity.
We define |myPairX| with this:
%
\begin{spec}
myPairX x = pair x
\end{spec}
%
We infer these types:
\begin{center}
\begin{tabular}{l||l||l}
|myPairX| & eager & lazy \\ \hline
\squeezed{deep or}{shallow} & \squeezed{|forall {a} {b}.|}{|a -> b -> (a, b)|} & \squeezed{|forall {a}. a ->|}{|forall b. b -> (a, b)|} \\
\end{tabular}
\end{center}
%
Unsurprisingly, the generalised variables end up as inferred, instead of specified.

\subsection*{Similarity 2: Signature Property}

The second similarity annotates a let binding with the inferred type
\( [[s]] \) of the bound expression \( [[ee1]] \). We expect this
similarity to be one-directional, as dropping a type annotation may
indeed change the compile time semantics of a program, as we hope programmers
expect.
\begin{equation*}
  [[ </ f psi = eei // i /> ]] \transCR [[ f : s; </ f psi = eei // i /> ]],~\text{where}~[[ s ]]~\text{is the inferred type of}~[[ f ]] 
\end{equation*}

\paragraph{Example 4: |infer|}

Though not yet implemented, we consider a version of Haskell that includes the ability
to abstract over type variables, the subject of an approved proposal for GHC~\cite{proposal-155}.
With this addition, we can imagine writing |infer|:
%
\begin{spec}
infer = \ @a (x :: a) -> x
\end{spec}
%
We would infer these types:
\begin{center}
\begin{tabular}{l||l||l}
|infer| & eager & lazy \\ \hline
deep or shallow & |forall {a}. a -> a| & |forall a. a -> a|
\end{tabular}
\end{center}
Note that the eager variant will infer a type containing an inferred quantified variable
|{a}|. this is because the expression |\ @a (x :: a) -> x| is instantly instantiated; it
is then |let|-generalised to get the type in the table above.

If we change our program to include these types as annotations, the eager type, with its
inferred variable, will be rejected. The problem is that we cannot check an abstraction
|\ @a -> ...| against an expected type |forall {a}. ...|: the whole point of having
an inferred specificity is to prevent such behaviour, as an inferred variable should not
correspond to either abstractions or applications in the term.

\subsection*{Similarity 3: Type Signatures}

Changing a type signature should not affect runtime semantics---except in the case of type classes
(or other feature that interrupts parametricity). Because our paper elides type classes, we can
state this similarity quite generally; more fleshed-out settings would require a caveat around
the lack of type-class constraints.
\begin{equation*}
  [[ f : s1; </ f psi = eei // i /> ]] \transBR [[ f : s2; </ f psi = eei // i /> ]] 
\end{equation*}

%% \begin{similarity}[Type signature for undefined]
%%   \[ | let BANG x = undefined in () | \transBCR | let x :: ty ; BANG x = undefined in () | \]
%% \end{similarity}

\paragraph{Example 5: |swizzle|}

Suppose we have this function defined\footnote{This example is inspired by
\citet{proposal-287}.}:
%
\begin{code}
undef :: forall a. Int -> a -> a
undef = undefined
\end{code}
%
Now, we write a synonym but with a slightly different type:
\begin{code}
swizzle :: Int -> forall a. a -> a
swizzle = undef
\end{code}
%
Shockingly, |undef| and |swizzle| have different runtime behaviour: forcing |undef| diverges
(unsurprisingly), but forcing |swizzle| has no effect. The reason is that the definition
of |swizzle| is not as simple as it looks. In the System-F-based core language used
within GHC, we have |swizzle = \ (n :: Int) -> /\ (a :: Type) -> undef @a n|. Accordingly,
|swizzle| is a function, which is already a value\footnote{Similarly to |swizzle|,
the definition of |undef| gets translated into
| /\ (a :: Type) -> undefined @(Int -> a -> a)|.
However, this is not a value as GHC evaluates underneath the | /\ | binder.
The evaluation relation can be found in Appendix~\ref{app:systemf}.}.

Under shallow instantiation, |swizzle| would simply be rejected, as its type is different
than |undef|'s. The only way |swizzle| can be accepted is if it is deeply skolemised
(see \emph{Application} in Section~\ref{sec:calculus}), a necessary consequence
of deep instantiation.

\begin{center}
\begin{tabular}{l||l}
|swizzle| & eager or lazy \\ \hline
deep & converges \\
shallow & rejected \\
\end{tabular}
\end{center}

\subsection*{Similarity 4: Pattern-Inlining and Extraction}

The fourth similarity represents changing variable patterns (written to the left of the
|=| in a function definition) into $\lambda$-binders (written on the right of the |=|),
and vice versa.
Here, we assume the patterns \( [[ ps ]] \) contain only (expression and type) variables.
The three-place \( [[ wrap ]] \) relation is unsurprising. It
denotes that wrapping the patterns $[[ps]]$ around the expression $[[ee1]]$
in lambda binders results in $[[ee1']]$.
Its definition can be found in \pref{app:addrel}.
\begin{equation*}
  [[ let x ps = ee1 in ee2 ]] \transBCR [[ let x = ee1' in ee2 ]],~\text{where}~[[ wrap ( ps ; ee1 ~ ee1' ) ]]
\end{equation*}

\paragraph{Example 6: |infer2|, again}

Returning to the |infer| example, we might imagine moving the
abstraction to the left of the |=|, yielding:
%
\begin{spec}
infer2 @a (x :: a) = x
\end{spec}
%
Under all instantiation schemes, |infer2| will be assigned the type |forall a. a -> a|.
Accordingly, under eager instantiation, the choice of whether to bind the variables
before the |=| or afterwards matters.

%% Here, though, we encounter another complication: we might imagine using these inferred
%% types to write a type signature in our program; an IDE might also do this automatically.
%% If we have eager instantiation, though, adding the type signature would lead to trouble.

%% Imagine checking the expression |\ @a (x :: a) -> x| against the type |forall {a}. a -> a|.
%% The quantified type variable |a| is marked as inferred, and so it is not available for
%% explicit instantiation or abstraction---indeed, the \emph{raison d'\^etre} of inferred
%% variables is that their presence or ordering cannot impact the typability of a program.
%% The expression thus fails to type-check. This is very disappointing; the language
%% implementation rejects the very type it has itself inferred.

\subsection*{Similarity 5: Single vs. Multiple Equations}

Our language model includes the ability to define a function by specifying multiple
equations. 
The type inference algorithm in GHC differentiates between single and multiple
equation declarations (see Section~\ref{sec:evaluation}),
and we do not want this distinction to affect types.
While normally new equations for a function would vary
the patterns compared to existing equations, we simply repeat the existing equation
twice; after all, the particular choice of (well-typed) pattern should not affect
compile time semantics at all.
\begin{equation*}
   [[ f ps = ee ]] \transBC [[ f ps = ee, f ps = ee ]]
\end{equation*}

\paragraph{Example 7: |unitId1| and |unitId2|}

Consider these two definitions:
%
\begin{code}
unitId1 () = id

unitId2 () = id
unitId2 () = id
\end{code}
%
Both of these functions ignore their input and return the polymorphic identity
function. Let us look at their types:
%
\begin{center}
\begin{tabular}{@@{}l@@{\quad}l||l||l}
  && eager & lazy \\ \cline{2-4}
|unitId1| & \squeezed{deep or}{shallow} & \squeezed{|forall {a}. () -> |}{|a -> a|} & \squeezed{|() ->|}{|forall a. a -> a|} \\ 
|unitId2| & \squeezed{deep or}{shallow} & \squeezed{|forall {a}. () -> |}{|a -> a|} & \squeezed{|forall {a}.() -> |}{|a -> a|} \\
\end{tabular}
\end{center}
%
The lazy case for |UnitId1| is the odd one out: we see that the definition of |unitId1|
has type |forall a. a -> a|, do not instantiate it, and then prepend the |()| parameter.
In the eager case, we see that both definitions instantiate |id| and then re-generalise.

However, the most interesting case is the treatment of |unitId2| under lazy instantiation.
The reason the type of |unitId2| here differs from that of |unitId1| is that the pattern-match
forces the instantiation of |id|.
As each branch of a multiple-branch pattern-match must result in the same type,
we have to seek the most general type that is still less general than each branch's type.
Pattern matching thus performs an instantiation step (regardless of eagerness),
in order to find this common type.

In the scenario of |unitId2|, however, this causes trouble: the match instantiates |id|,
and then the type of |unitId2| is re-generalised. This causes |unitId2| to have a
different inferred type than |unitId1|, leading to an instability.

\subsection*{Similarity 6: $\eta$-Expansion}

And lastly, we want $\eta$-expansion not to affect types. (This change \emph{can}
reasonably affect runtime behaviour, so we would never want to assert that $\eta$-expansion maintains
runtime semantics.)
\begin{equation*}
    [[ ee ]] \transBC [[ \ x . ee x ]],~\text{where}~[[ee]]~\text{has a function type} 
\end{equation*}

\paragraph{Example 8: |eta|}

Consider these two definitions, where |id :: forall a. a -> a|:
%
\begin{code}
noEta  =  id
eta    =  \x -> id x
\end{code}
%
The two right-hand sides should have identical meaning, as |eta| is simply
the $\eta$-expansion of |noEta|. Yet, under lazy instantiation, these
two will have different types:

\begin{center}
\begin{tabular}{l@@{\quad}l||l||l}
  && eager & lazy \\ \cline{2-4}
  |noEta| & deep or shallow & |forall {a}. a -> a| & |forall a. a -> a| \\
  |eta|   & deep or shallow & |forall {a}. a -> a| & |forall {a}. a -> a| \\
\end{tabular}
\end{center}
%
The problem is that the $\eta$-expansion instantiates the occurrence of |id| in
|eta|, despite the lazy instantiation strategy. Under eager instantiation, the
instantiation happens regardless.

\subsection{Stability}

The examples in this section show that the choice of instantiation scheme matters---and
that no individual choice is clearly the best. To summarise, each of our possible
schemes runs into trouble with some example; this table lists the numbers of the examples
that witness a problem:
%
\begin{center}
\begin{tabular}{l||l||l}
        & eager & lazy \\ \hline
deep    & 1, 2, 3, 4, 5, 6  & 5, 7, 8 \\
shallow & 1, 2, 3, 4, 6     & 7, 8 \\
\end{tabular}
\end{center}
%
At this point, the best choice is unclear. Indeed, these examples are essentially
where we started our exploration of this issue---with failures in each quadrant
of this table, how should we design instantiation in GHC?

To understand this better, Section~\ref{sec:calculus} presents a formalisation
of GHC's type-checking algorithm,
parameterised over the choice of depth and eagerness. \Pref{sec:evaluation} then
presents properties derived from the similarities of this section and checks
which variants of our type system uphold which properties. The conclusion becomes
clear: lazy, shallow instantiation respects the most similarities.

We now fix the definition of stability we will work toward in this paper:

\begin{definition*}[Stability]
  A language is considered stable when all of the program similarities above
  are respected.
\end{definition*}

We note here that the idea of judging a language by its robustness in the face of
small transformations is not new; see, for example, \citet{recasting-mlf} or \citet{cochis},
who also consider a similar property. However, we believe ours is the first work
% to give this property a name---stability---and
to focus on it as the primary criterion of evaluation.
%%  It is our hope that this attention to stability will
%% inspire others to use it more explicitly as a design goal and metric.

Our goal in this paper is not to eliminate instability, which would likely be too limiting, leaving
us potentially with either the Hindley-Milner implicit type system or a System F explicit one. Both
are unsatisfactory. Instead, our goal is to make the consideration of stability a key
guiding principle in language design. The rest of this paper uses the lens of stability
to examine design choices around ordered explicit type instantiation. We hope
that this treatment serves as an exemplar for other language design tasks and provides
a way to translate vague notions of an ``intuitive'' design into concrete language
properties that can be proved or disproved. Furthermore, we believe that instantiation
is an interesting subject of study, as any language with polymorphism must consider
these issues, making them less esoteric than they might first appear. 



==> tex/sections/SystemF.tex <==
%if style == newcode
\begin{code}
module SystemF where
\end{code}
%endif

\section{Core Language}
\label{app:systemf}

The dynamic semantics of the languages in Section~\ref{sec:calculus}
are defined through a translation to System F. While
the target language is largely standard, a few interesting remarks can be made.
The language supports nested pattern matching through case lambdas
\( [[ </ case fpsi : fpsigs -> efi // i /> ]] \), where patterns \( [[ fp ]] \)
include both term and type variables, as well as nested constructor patterns.
Note that while we reuse our type \([[s]]\) grammar for the core language,
System~F does not distinguish between inferred and specified binders.

We also define two meta-language features to simplify the elaboration, and the
proofs:
Firstly, in order to support eta-expansion (for translating deep instantiation
to System F), we define expression wrappers \([[ ewf ]]\),
essentially a limited form of expressions with a hole \( [[ [] ]] \) in them.
An expression \( [[ ef ]] \) can be filled in for the hole to get a
new expression \( [[ ewf [ ef ] ]] \). One especially noteworthy wrapper
construct is \( [[ \ ef1 . ef2 ]] \), explicitly abstracting over and handling
the expression to be filled in.
Note that, as expression wrappers are only designed to alter the type of expressions
through eta-expansion, there is no need to support the full System~F syntax.

Secondly, in order to define contextual equivalence, we introduce contexts \([[ fctx ]]\).
These are again expressions with a hole \([[ [] ]]\) in them, but unlike
expression wrappers, contexts do cover the entire System~F syntax.
Typing contexts is performed by the \([[ fctx : G1 ; s1 |-> G2 ; s2 ]]\) relation:
``Given an expression \([[ef]]\) that has type \([[s1]]\) under typing environment \([[G1]]\),
then the resulting expression \([[ fctx [ ef ] ]]\) has type \([[s2]]\) under
typing environment \([[G2]]\)''.
We will elaborate further on contextual equivalence in Appendix~\ref{app:ctx_equiv}.

%\begin{figure}[h!]
  \input{tex/figures/FSyntax.mng}
%  \caption{System F Syntax}
%  \label{fig:FSyntax}
%\end{figure}

  \input{tex/figures/FTypingC.mng}

Evaluation for our System F target language is largely standard and defined
below.
Note that, following GHC, our target language evaluates inside type abstractions
(\rref{FEval-TyAbs}). Because of this, a type abstraction $[[ /\ a . ef ]]$
is a value if and only if $[[ ef ]]$ is a value. A more extensive discussion
can be found in \citet[Appendix~A.3]{zerocost}.

%\begin{figure}[h!]
  \input{tex/figures/FEval.mng}
%  \caption{System F Small Step Semantics}
%  \label{fig:FEval}
%\end{figure}

%% \subsection{Translation from Implicit Polymorphic $\lambda$-Calculus}

%% \begin{figure}[h!]
%%   \input{tex/figures/SimpleTypingAF.mng}
%%   \caption{Term Typing for Implicit Polymorphic $\lambda$-Calculus with Translation}
%%   \label{fig:STmF}
%% \end{figure}

%% \begin{figure}[h!]
%%   \input{tex/figures/SimpleTypingCF.mng}
%%   \caption{Declaration Checking for Implicit Polymorphic $\lambda$-Calculus with Translation}
%%   \label{fig:STmcF}
%% \end{figure}

%% \begin{figure}[h!]
%%   \input{tex/figures/SimpleTypingDF.mng}
%%   \caption{Pattern Typing for Implicit Polymorphic $\lambda$-Calculus with Translation}
%%   \label{fig:STmdF}
%% \end{figure}

%% \begin{figure}[h!]
%%   \input{tex/figures/AltTypingBF.mng}
%%   \caption{Argument Type Checking for Implicit Polymorphic $\lambda$-Calculus with Translation}
%%   \label{fig:ATmbF}
%% \end{figure}

\subsection{Translation from the Mixed Polymorphic $\lambda$-calculus}
\label{app:elab}

%\begin{figure}[h!]
  \input{tex/figures/AltTypingAF.mng}
%  \caption{Term Typing for Mixed Polymorphic System F with Translation}
%  \label{fig:ATmF}
%\end{figure}

%\begin{figure}[h!]
  \input{tex/figures/ModTypingBF.mng}
%  \caption{Argument Type Checking for Mixed Polymorphic System F with Translation}
%  \label{fig:MTmbF}
%\end{figure}

%\begin{figure}[h!]
  \input{tex/figures/FTypingA.mng}
%  \caption{Type Instantiation for Mixed Polymorphic System F with Translation}
%  \label{fig:FTmA}
%\end{figure}

%\begin{figure}[h!]
  \input{tex/figures/ModTypingCF.mng}
%  \caption{Declaration typing for Mixed Polymorphic System F with Translation}
%  \label{fig:MTmcF}
%\end{figure}

%\begin{figure}[h!]
  \input{tex/figures/ModTypingEF.mng}
%  \caption{Pattern Typing for Mixed Polymorphic System F with Translation}
%  \label{fig:MTmeF}
%\end{figure}


